Techniques for Shared Resource Management in Systems with Throughput Processors

The continued growth of the computational capability of throughput processors has made throughput processors the platform of choice for a wide variety of high performance computing applications. Graphics Processing Units (GPUs) are a prime example of throughput processors that can deliver high performance for applications ranging from typical graphics applications to general-purpose data parallel (GPGPU) applications. However, this success has been accompanied by new performance bottlenecks throughout the memory hierarchy of GPU-based systems. We identify and eliminate performance bottlenecks caused by major sources of interference throughout the memory hierarchy. We introduce changes to the memory hierarchy for systems with GPUs that allow the memory hierarchy to be aware of both CPU and GPU applications' characteristics. We introduce mechanisms to dynamically analyze different applications' characteristics and propose four major changes throughout the memory hierarchy. We propose changes to the cache management and memory scheduling mechanisms to mitigate intra-application interference in GPGPU applications. We propose changes to the memory controller design and its scheduling policy to mitigate inter-application interference in heterogeneous CPU-GPU systems. We redesign the MMU and the memory hierarchy in GPUs to be aware of ddress-translation data in order to mitigate the inter-address-space interference. We introduce a hardware-software cooperative technique that modifies the memory allocation policy to enable large page support in order to further reduce the inter-address-space interference at the shared Translation Lookaside Buffer (TLB). Our evaluations show that the GPU-aware cache and memory management techniques proposed in this dissertation are effective at mitigating the interference caused by GPUs on current and future GPU-based systems.

==> Makefile <==
NAME = paper

.PHONY: paper clean
all: paper

paper: $(NAME).tex
	latexmk -xelatex -bibtex $(NAME).tex
	mv *.blg ./log
	mv *.bbl ./log
	mv *.fls ./log
	mv *.aux ./log
	mv *.log ./log
	mv *.fd* ./log
	mv *.toc ./log

rolling: $(NAME).tex
	latexmk -xelatex -pvc -bibtex -interaction=nonstopmode $(NAME).tex

clean:
	\rm ./log/* paper.pdf



==> font.tex <==
\usepackage[T1]{fontenc}
\usepackage{libertine}
\renewcommand*\oldstylenums[1]{{\fontfamily{fxlj}\selectfont #1}}


==> secs/abstract-short.tex <==
\chapter*{Abstract}
%\vspace{-0.3in}

The continued growth of the computational capability of throughput processors
has made throughput processors the platform of choice for a wide variety of
high performance computing applications. Graphics Processing Units (GPUs) are
a prime example of throughput processors that can deliver high performance for
%a prime example of throughput processors that is capable of providing high performance for
applications ranging from typical graphics applications to general-purpose data
parallel (GPGPU) applications. However, this success has been accompanied by
new performance bottlenecks throughout the memory hierarchy of GPU-based
systems. This dissertation identifies and eliminates performance bottlenecks
caused by major sources of interference throughout the memory hierarchy. 



%The continued growth of the computational capability, along with considerable
%improvements in the programmability of Graphics Processing Units (GPUs), have
%made GPUs the platform of choice for a wide variety of applications, ranging
%from typical graphics applications to general purpose data parallel (GPGPU)
%applications.  However, this success has been accompanied by new performance
%bottlenecks throughout the memory hierarchy of GPU-based systems. This
%dissertation identifies and eliminates performance bottlenecks caused by major
%sources of interference throughout the memory hierarchy. 

Specifically, we provide an in-depth analysis of inter- and intra-application
as well as inter-address-space interference that % have become a significant performance bottleneck.
significantly degrade the performance and efficiency of GPU-based systems.
% in any systems with GPUs. 
%These interferences not only 
%leading to poor GPU performance but also cause %memory divergence and %This is not defined yet so it is not a good idea to use it here
%This interference also causes unfairness to other applications that are sharing resources % such as the shared
%cache, shared main memory and shared TLB, 
%with the GPU.
% Addressing these emerging performance bottlenecks are largely impossible 
%unless the design of memory hierarchy are aware of GPU applications'
%characteristics.

%This dissertation develops shared resource management mechanisms throughout the main
%memory hierarchy that reduce interference in current and future systems with
%GPUs. We first analyze GPU characteristics and the source of interference
%throughout the memory hierarchy including the memory management unit (MMU). 

To minimize such interference, we introduce changes to the memory
hierarchy for systems with GPUs that allow the memory hierarchy to be aware of
both CPU and GPU applications' characteristics. We introduce
mechanisms to dynamically analyze different applications'
characteristics and propose four major changes throughout the memory
hierarchy. 

We propose changes to the cache management and memory scheduling mechanisms to
mitigate intra-application interference in GPGPU applications. We propose
changes to the memory controller design and its scheduling policy to mitigate
inter-application interference in heterogeneous CPU-GPU systems.  We redesign
the memory management unit and the memory hierarchy in GPUs to be aware of
address-translation-related data in order to mitigate the inter-address-space interference that
originates from the address translation process. We introduce a
hardware-software cooperative technique that modifies the memory allocation
policy to enable large page support in order to further reduce the
inter-address-space interference at the shared Translation Lookaside Buffer (TLB). Our evaluations show that
the GPU-aware cache and memory management techniques proposed in this
dissertation are effective at mitigating the interference caused by GPUs on
current and future GPU-based systems.



%First, we introduce \titleLongMeDiC
%(\titleShortMeDiC), a cache management mechanism that mitigates
%intra-application interference in GPGPU applications by allowing the shared L2
%cache and the memory controller to be aware of the GPU's warp-level memory divergence characteristics.
%\titleShortMeDiC uses this warp-level memory divergence information to give
%more cache space and more memory bandwidth to warps that benefit most from utilizing such resources.
%Our evaluations show that \titleShortMeDiC significantly outperforms multiple
%state-of-the-art caching policies proposed for GPUs.
%
%Second, we introduce the \titleLongSMS (\titleShortSMS), an
%application-aware CPU-GPU memory request scheduler that mitigates inter-application
%interference in heterogeneous CPU-GPU systems.  \titleShortSMS creates a
%fundamentally new approach to memory controller design that decouples
%% the three primary tasks of 
%the memory controller into three significantly simpler structures, each of
%which has a separate task, These structures operate together to greatly improve both system
%performance and fairness. Our three-stage memory controller first groups
%requests based on row-buffer locality. This grouping allows the second stage to
%focus on inter-application scheduling decisions. These two stages enforce
%high-level policies regarding performance and fairness. As a result, the last
%stage is simple logic that deals only with the low-level DRAM
%commands and timing. SMS is also configurable: it allows the system software
%to trade off between the quality of service provided to the CPU versus GPU applications.
%%\rachata{This stuff below is too long according to Onur's comment}
%%Our three-stage memory controller first groups
%%requests based on row-buffer locality. This grouping allows the second stage to
%%focus only on inter-application scheduling decisions. These two stages enforce
%%high-level policies regarding performance and fairness, and therefore the last
%%stage can employ simple per-bank FIFO queues and straight-forward logic that
%%only deals with the low-level DRAM commands and timing. 
%Our evaluations show that \titleShortSMS not only reduces inter-application
%interference caused by the GPU, thereby improving heterogeneous system
%performance, but also provides better scalability and power efficiency compared
%to multiple state-of-the-art memory schedulers.
%
%
%%This dissertation introduces changes in order to make memory hierarchy aware of differing
%%GPU applications' characteristics. This dissertation introduces MeDiC, a cache management 
%%mechanism, that mitigates intra-application interference in GPGPU applications by
%%allowing the shared L2 cache to be aware of GPU's warp-level memory divergence characteristics
%%and give cache resources to warps that benefit most from utilizing the cache.
%%
%%This dissertation introduces SMS, an application aware CPU-GPU memory scheduler that
%%mitigates inter-application interference in heterogeneous CPU-GPU systems. SMS
%%allows the shared memory scheduler to be aware of both CPU and GPU applications.
%%The design of SMS not only reduce inter-application interference caused by the GPU,
%%but also is more scalable than other state-of-the-art memory scheduler.
%
%
%Third, we redesign the GPU memory management unit to efficiently handle new
%problems caused by the massive address translation parallelism present in GPU
%computation units in multi-GPU-application environments. Running multiple GPGPU
%applications concurrently induces significant inter-core thrashing on the
%shared address translation/protection units; e.g., the shared Translation
%Lookaside Buffer (TLB), a new phenomenon that we call \emph{inter-address-space
%interference}. To reduce this interference, we introduce \emph{\titleLongMASK}
%(\titleShortMASK).  \titleShortMASK introduces TLB-awareness throughout the GPU
%memory hierarchy and introduces TLB- and cache-bypassing techniques to increase
%the effectiveness of a shared TLB. 
%
%Finally, we introduce \titleShortMOSAIC, a hardware-software cooperative
%technique that further increases the effectiveness of TLB by modifying the
%memory allocation policy in the system software. \titleShortMOSAIC introduces a
%high-throughput method to support large pages in multi-GPU-application
%environments. \yellow{The key idea is to ensure memory allocation preserve address space
%contiguity to allow pages to be coalesced without any data movements.} Our
%evaluations show that the \titleShortMASK-\titleShortMOSAIC combination
%provides a simple mechanism that eliminates the performance overhead of address
%translation in GPUs without significant changes to GPU hardware, thereby
%greatly improving GPU system performance. 

%Finally, we propose two techniques that redesign the GPU memory
%management unit to efficiently handle new problem caused by the massive parallelism present in GPU computation units in multi-GPU-application
%scenarios. We find that even with state-of-the-art GPU memory management and TLB designs,
%a single TLB miss during address translation can frequently stall multiple 
%GPU warps, defeating the GPU's fundamental
%techniques for tolerating memory latency. Furthermore, running multiple GPGPU
%applications concurrently induces significant inter-core thrashing on the
%shared TLB, a new phenomenon that we call \emph{inter-address-space interference}. We
%discover that inter-address-space interference between TLB misses and
%data requests throughout the memory hierarchy is a first-order performance
%concern. To reduce this interference, we introduce two new mechanisms: \titleLongMASK (\titleShortMASK) and \titleShortMOSAIC.
%\titleShortMASK introduces TLB-awareness throughout the memory hierarchy and
%introduces TLB- and cache-bypassing techniques to increase the effectiveness of a
%shared TLB. \titleShortMOSAIC provides a hardware-software cooperative
%technique that modifies the memory allocation policy in the system software and
%introduces high throughput method to support large pages in
%multi-GPU-application environments. We show that the
%\titleShortMASK-\titleShortMOSAIC combination provides a simple mechanism to eliminate
%the performance overhead of address translation in GPUs without significant
%changes in GPU hardware.

The key conclusion of this dissertation is that a combination of GPU-aware
cache and memory management techniques can effectively mitigate the memory
interference on current and future GPU-based systems as well as other types
of throughput processors.

\rachata{KevinC: The last sentence might not be enough. Might want to add another sentence to say something.}
\rachata{KevinC: Might want to break the MASK and MOSAIC.}

%\rachata{The para above, after mosaic and mask are introduces. Need fix because
%it still is not clear what mask and mosaic brings.}




==> secs/contrib.tex <==
\section{Expected Contributions}

We expect this thesis to make the following key contributions:

\begin{itemize}

\item This thesis provides a thorough design across the entire memory hierarchy
that improves quality of service (QoS), without affecting the performance, when
multiple GPGPU applications are concurrently running.

\item \titleShortMeDiC is the first work that observes that the different warps
within a GPGPU application exhibit heterogeneity in their memory divergence
behavior at the shared L2 cache, and that some warps do not benefit from the
few cache hits that they have. This memory divergence behavior tends to remain
consistent throughout long periods of execution for a warp, allowing for fast,
online warp divergence characterization and prediction.

\item \titleShortMeDiC identifies a new performance bottleneck in GPGPU
application execution that can contribute significantly to memory divergence:
due to the very large number of memory requests issued by warps in GPGPU
applications that contend at the shared L2 cache, many of these requests
experience \emph{high cache queuing latencies}.

\item \titleShortSMS is the first to observe the key difference between CPU and
GPU traffic that causes existing memory schedulers to perform poorly due to
interference from the GPU. 

\item \titleShortSMS is the first to observe a possible scalability problem in
existing memory schedulers when scheduling for high bandwidth applications. 

\item To our knowledge, this thesis will be the first work that incorporates
the knowledge of the Graphics pipeline to a GPU throttling mechanism.

\item To our knowledge, this thesis is the first work that takes an exhausive
look at how to provide a method to share GPU resources that can provide memory
protection and performance isolation for kernels concurrently executing in
separate address spaces.

\end{itemize}



==> secs/future.tex <==
\chapter{Future Research Directions}
%\section{Future Research Directions}


\section{Additional QoS Issues in Systems with GPUs}

While this thesis addressed interference problems in various systems with GPUs.
There are additional Quality-of-Service (QoS) issues that are out of the scope
of this thesis. These issues generally arises when multiple GPU applications
are spatially sharing the GPU and are running concurrently. 

The first issues that arises is that the introduction of multiple GPU introduces
resource contention at the scratchpad memory, which is usually software managed.
When multiple applications are sharing the GPUs, it is possible for one application
allocate all of scratchpad memory. In this scenario, other applications are unable
to utilize any of these scratchpad space until the original application release
their allocated memory. 

With the techniques and hardware changes that allows applications to share the GPU
more effectively, it is possible to solve this QoS problem using through modifications
in the hypervisor. For example, additional kernel scheduling techniques can be applied
to 1) probe the scratchpad requirement by each application and 2) enforce a proper QoS
policy, which only grants each application a portion of the scratchpad memory. Because
this involves changes in both the hypervisor as well as the original GPGPU applications,
which now has to be able to adapt to differing resource restriction, it is out of the
scope of this thesis.


\section{Interference Management in GPUs for Real-time Applications}

The emergence of new type of Internet-of-things (IoT) brings introduces another
type of application. Traditionally, these applications runs on an embedded device
that handles all the computations. However, the rise of better cloud infrastructures
allows these applications to off-load their computation over to a centralized
servers. While the GPU can provide good throughput due to its parallelism, it
also needs to provide a good response time for these emerging real-time application
as well.

Even though mechanisms proposed in this thesis aim to minimize the slowdown caused
by interference, these mechanisms are unable to provide an actual performance
guarantee, which is required when a hard real-time application is executing.



%\section{Proposed Future Research}
%
%Our preliminary works provide mechanisms to reduce interference of GPUs on
%shared cache (Section~\ref{sec:prelim-medic}) and main memory
%(Section~\ref{sec:prelim-sms}). In this section, we investigate other parts of
%the memory hierarchy and propose mechanisms to mitigate GPU interference. First,
%we take further look at the generation of GPU requests onto the memory
%hierarchy. Our proposal plans to further reduce the interference of GPU on the
%memory hierarchy by selectively throttling the GPU, as explained in
%Section~\ref{sec:sms-plus}.
%
%Second, to fully provide performance isolation and reduce interference in
%system with GPUs across all parts of the memory hierarchy, we plan to
%investigate interference of GPU on the remaining component in the memory
%hierarchy, which is the memory management units (MMU) and translation lookaside
%buffers (TLB). Section~\ref{sec:tlb} provides our research plan on how to
%design the MMU and TLB not only to be aware of the GPU applications, but also
%aware of interference cased by multiple concurrent GPU applications sharing the
%GPU.
%
%\section{Eliminating Interference in Heterogeneous Systems with GPU-aware Source Throttling}
%\label{sec:sms-plus}
%
%While our preliminary work, \titleLongSMS~\cite{sms}, provides an
%application-aware memory scheduling design for a CPU-GPU heterogeneous system,
%GPU applications can still saturate the available memory bandwidth.  The amount
%of parallelism of the Graphics applications causes burst of memory requests
%over a short period of time. The observation from our preliminary work,
%SMS~\cite{sms}, shows memory requests from Graphics applications flood the memory controller during
%these burst. As a result, other applications that share the off-chip memory stall. The
%solution provided by our preliminary work, SMS, can mitigate the interference
%from these Graphics applications in heterogeneous CPU-GPU systems. However, in
%multiple SoCs, the amount of the available off-chip bandwidth is shared across
%multiple IPs. As a result, it is desirable to lower the amount of peak
%bandwidth created by the GPU, reducing the pressure from the Graphics
%applications at the memory controller.
%
%%GPU applications can still saturated the available memory bandwidth.
%%Figures~\ref{peak-memory-bandwidth}a shows bandwidth consumption of a Graphic
%%application over time. As can be observed from
%%Figure~\ref{peak-memory-bandwidth}a, Graphic application generally send burst
%%of requests following by a period of small memory activity. Similar to the
%%observation from the previous work, SMS~\cite{sms}, memory requests from
%%Graphic flood the memory controller during these burst, stalling other
%%application that share the off-chip memory. While the solution provided by our
%%preliminary work, SMS, can mitigate the interference from these Graphic
%%application in heterogeneous CPU-GPU systems, it is still desirable to lower
%%the amount of peak bandwidth, reducing the pressure from the Graphic
%%application at the memory controller.
%
%To address this problem, we plan to further analyze the source of these
%GPU bursts by breaking down the memory request stream from Graphics applications
%into multiple separate streams, each of which comes from different buffers in
%GPUs (texture, color, shader, etc.). Then, we plan to redesign these buffers to
%be aware of the Graphics pipeline and manipulate the memory request stream from
%these buffers to lower the peak GPU bandwidth. This would reduce contention in the
%memory system and, if done right, improve the QoS and performance.
%%if they are not critical to the progress of the GPU (i.e., throttling
%%requests from this buffer should not affect the framerate of the Graphic application).
%%Figure~\ref{peak-memory-bandwidth-break}b
%%provides this breakdown of memory request burst from each buffer in the GPU. We
%%make an observation that during each burst, not all buffer but only a subset of
%%them are the sources of such memory request burst.
%
%%TODO: Add this plot
%
%\subsection{Our Goal}
%
%As previously mentioned, our goal in this direction of study is to design a
%mechanism that can selectively throttle different buffers in GPU, eliminating
%the source of the high peak GPU bandwidth at the source without affecting the
%framerate performance of Graphics applications. To achieve this result, we
%propose to map how Graphics pipeline renders a frame to each of the buffers and caches
%that is utilizing the memory. Then, we categorize memory requests into critical and
%non-critical requests. An example of critical requests is a request for data
%used by an earlier stage of the Graphics pipeline. An example of a
%non-critical requests is a request for data further in the
%Graphics pipeline. For example, a write to frame buffer, which is the final
%step in the rendering process, is less important compared to other requests in
%the Graphics pipeline and can be delayed until the end of the rendering process.
%With this categorization, we propose to provide a Graphics-pipeline-aware
%throttling mechanism. This mechanism throttles requests that are in
%the non-critical category, delaying injection of these memory requests.
%We plan to throttle these requests until the main memory have available bandwidth to service these
%memory requests. At the same time, we propose to use the knowledge of the
%Graphics pipeline to accelerate memory requests that are in the critical category to
%meeting the framerate target.
%
%
%In summary, we plan to answer the following questions:
%
%\begin{enumerate}
%
%\item How can we design a GPU throttling mechanism that can utilize the knowledge
%of the Graphics pipeline?
%
%\item Is it possible to model dependencies between differing GPU memory requests and
%identify the critical memory requests during execution in hardware?
%
%\item How can we design a mechanism that can accelerate critical memory requests to make
%effective use of the available memory bandwidth?
%
%\item What is the performance improvement of the combined throttling mechanism
%and various memory scheduling mechanism, including SMS~\cite{sms} and recent
%memory schedulers~\cite{bliss}?
%
%\end{enumerate}
%
%
%\section{Interference from GPU in Future Systems Containing Multiple GPU Applications}
%\label{sec:tlb}
%
%
%While many applications can benefit from GPU acceleration, not all of them can
%fully utilize the resources available on a GPU. For example, an application may
%exhibit abundant parallelism but fail to utilize \emph{entire} GPU memory.  Similarly,
%irregular parallel applications might occupy fewer cores while consuming more
%off-chip memory. Heterogeneity with respect to resource consumption represents
%an opportunity for the GPU to concurrently schedule kernels from multiple applications. 
%The \emph{de facto} standard approach to scheduling for GPUs
%time-slices all resources, unnecessarily serializing work that could be
%co-scheduled to improve throughput. 
%
%As pointed out in Section~\ref{sec:virt-back}, the current implementations of
%TLB and MMU~\cite{markhill-tlb,abhishek-tlb,grid,gdev,gpuvm} strictly limit
%all GPGPU applications to have one virtual address space. Restriction to a
%single address-space is a severe limitation because it disables kernels from
%different GPGPU applications to run concurrently. This does not only lead to
%sub-optimal performance, but also causes system-level pathologies like priority
%inversion~\cite{ptask}. NVIDIA GRID~\cite{grid} and AMD Multi-user GPU~\cite{firepro} provide
%hardware supports that allow multiple applications on multiple
%virtual machines to share a single physical GPU. However, these solutions
%impose hard bounds on the actual level concurrency, e.g. GRID supports up to
%four concurrent VMs. As a result, resources are statically partitioned across virtual
%machines. Statically partition resources reduces efficiency and limits the ability of the system to
%respond to load imbalance and to enforce performance isolation.
%
%Although enabling multiple address spaces increases GPU efficiency, it can also cause
%interference between different GPU applications. Specifically, one
%application might cause TLB flushes and occupy the majority of the main memory,
%resulting in slowdown of other applications sharing the system. In this thesis proposal,
%we plan to mitigate interference problem when multiple GPU applications are concurrently running on the GPU.
%
%
%%However, previous work has observed that claiming all the GPU resources is not
%%always beneficial~\cite{onur-pact}. Recently, a newer set of analytic GPGPU
%%applications, such as the Netflix movie recommendation system~\cite{netflix}
%%and a stock market analyzer~\cite{tobias-stock}, require a closely connected,
%%highly virtualized, shared environment. These applications, which benefit from
%%the amount of parallelism that the GPUs provides, do not need to use all
%%resources in the GPU to maximize their performance. Instead, these emerging
%%applications benefit from concurrency - by running a few of these applications
%%together, each application claims some share of the resources on the GPU, without
%%incurring significant performance impact since every application only requires a
%%portion of GPU resources. However, to effectively run these applications
%%concurrently, an intelligent and dynamic resource management mechanism is
%%needed in order to provide better efficiency and high throughput.
%%
%%In order for these analytic GPGPU applications to be run effectively in a large
%%datacenter, recent works propose a mechanism that provides virtualization of GPU
%%resources, allowing the hypervisor to control resource allocation and make the GPU
%%available to all the virtual machines~\cite{grid,gpuvm}. While these approaches
%%allow GPGPU applications to be run on virtual machines with minimal performance
%%impact, GPU resources are either time-shared, allowing only one virtual machine
%%to utilize the entire GPU at time~\cite{pass-through}, or partitioned statically, where
%%each virtual machine will have access to statically partitioned GPU resources (GPU cores,
%%scratchpad and GPU main memory)~\cite{grid,gpuvm}. Both of these approaches limit
%%the viability of virtual machines to provide performance isolation and good
%%Quality-of-Serivce (QoS) to multiple GPGPU applications that run concurrently.
%%
%%Previous works have shown performance benefits on both graphics and GPGPU
%%applications by providing better scheduling and resource management in
%%GPUs~\cite{onur-pact,chatterjee14,chen-micro14,sms,onur-micro14,ccws,elastic-kernel}.
%%However, these approaches are done either purely from the hardware side with no
%%communication with the operating system and the applications
%%themselves~\cite{onur-pact,chatterjee14,chen-micro14,sms,onur-micro14,ccws} or
%%are designed purely from the GPGPU applications' side~\cite{elastic-kernel}.
%%Enabling communication between the hardware and software creates opportunities
%%for the management mechanism to partition GPU resources across multiple GPGPU
%%applications more efficiently.
%
%\subsection{Our Goal}
%
%Our goal in this research direction is to provide TLB and MMU
%designs that support fine-grain flexible spatial multi-plexing of GPU resource
%across kernels from mutually distrustful applications, e.g. processes running
%in different guest VMs on the same host. We argue that enabling such
%fine-grain sharing is not only beneficial, but required. Avoiding unnecessary
%serialization of kernels that could run concurrently improves resource
%utilization, end-to-end latency for individual applications, and system-wide
%throughput. More importantly, giving the hardware the ability to dynamically
%partition resources and disallow kernels from one process or VM to impede the
%progress of kernels from another, leading to better QoS and performance
%isolation.
%
%We plan to achieve our goal through two steps. First, we provide TLB and MMU
%designs that can support efficient TLB flush, demand paging. The TLB and MMU
%designs should be able to grant protections for GPGPU applications sharing the
%GPU. To achieve these goals, we plan to employ the assisted warp framework
%proposed in a previous work~\cite{caba}.  This assisted warp would perform
%tasks such as TLB flushes and demand paging while the TLB is implemented to
%contain bits for memory protection.
%
%Next, we plan to design a MMU that improves QoS and provides performance
%isolation. To achieve this goal, we plan to further modify the MMU in GPU with
%a page replacement policy that is aware of GPGPU applications and their
%characteristics. We plan to do this by adding a few additional PTX instructions. 
%Applications can add these PTX instructions to signal the GPU with basic mapping 
%between kernels and applications.
%
%In summary, we plan to answer the following questions:
%
%\begin{enumerate}
%
%\item How to design TLB and MMU that enable concurrent support for applications
%running on different virtual address space?
%
%\item How to efficiently design a mechanism that allows over-provision of GPU resources?
%The mechanism should provide supports for efficient TLB flushes and demand paging.
%
%\item Would it be possible to virtualize GPU resources intelligently in order
%to provide 1) performance isolation across different virtual machines and 2)
%quality of service (QoS) guarantees for each virtual machine?
%
%\item How can we add PTX instructions that enable applications to specify
%resource requirements?
%
%\end{enumerate}
%
%%\subsection{Novelty over Previous Work}
%%
%%Several previous works have explored potential benefits of providing
%%concurrency in GPUs~\cite{elastic-kernel} as well as benefits of better
%%resource management in simulation~\cite{onur-pact,sms,onur-micro14}.  Unlike
%%GRID~\cite{grid}, where all GPU resources are utilized by one virtual machine
%%at a time, we plan to develop a framework that allows GPGPU applications to be
%%run concurrently.  While there exist frameworks that allow multiple GPGPU
%%applications to run concurrently on a single system (Gdev~\cite{gdev}) and
%%on multiple virtual machines through a hypervisor (GPUVm~\cite{gpuvm}), both Gdev and GPUVm
%%do not provide a dynamic resource allocation scheme that can adapt to changes
%%in program behaviour and interference when multiple GPGPU applications are running
%%concurrently. Additionally, none of the previous works provides a
%%hardware-software cooperative scheduler and resource manager.
%%
%%In contrast to previous works, we aim to provide a GPU manager that supports
%%concurrency and can provide dynamic resource allocation of GPU resources. The
%%goal of this GPU manager is to improve system performance and QoS for GPGPU
%%applications that are sharing the GPU resources.
%
%%\subsection{Research Plan} 
%%
%%We propose to first analyze the behaviour and potential bottlenecks of recent GPGPU
%%applications~\cite{netflix,tobias-stock}. Toward this end, we propose to create
%%a framework that can intelligently schedule groups of GPGPU applications to
%%efficiently run together on a GPU, and design a resource allocator that
%%will accurately allocate different resources for each application based on application's
%%requirements. 
%%
%%In order to achieve our goal, we propose the following steps:
%%
%%\begin{itemize}
%%
%%\item Modify the Gdev framework~\cite{gdev} and create a resource manager that
%%allows dynamic allocation of GPU resources. This resource manager will keep track
%%of current GPU resources and provide the scheduling and resource allocation decisions
%%to all GPGPU applications.
%%
%%\item Developing a dynamic resource manager that can adapt to different GPGPU
%%applications' behaviour, as well as handling cases where multiple GPGPU
%%applications are running concurrently. Additionally, this resource manager will
%%group multiple GPU kernels that should be executed together into a single
%%CUDA context and schedule different CUDA contexts based on a QoS scheme to 
%%ensure concurrency and fairness.
%%
%%\item Integrating our software-based framework to the CUDA frontend of an
%%execution driven GPU simulator~\cite{gpgpusim}. Then, we plan to modify the GPU
%%architecture to expose simple GPU statistics from the hardware to the software
%%manager. Exposing simple hardware counters to the resource manager dynamically
%%should allow the scheduler and resource manager to schedule and allocate GPU
%%resources more efficiently.
%%
%%\item Lastly, in order to provide performance isolation and QoS across different virtual
%%machines, we propose to combine our infrastructure with GPUVm
%%framework~\cite{gpuvm} and design a mechanism that improve QoS of all virtual
%%machines. 
%%
%%\end{itemize}
%
%
%\section{Proposed Extensions to \titleShortMeDiC and \titleShortSMS}
%
%Our preliminary works, \titleShortMeDiC and \titleShortSMS, have mitigated
%interference in shared cache as well as the main memory. However, there are
%several design explorations and related research questions that we would like
%to further investigate. Section~\ref{sec:medic-plus} lists additional steps we
%plan for \titleShortMeDiC and Section~\ref{sec:sms-plusplus} lists additional
%steps we plan for \titleShortSMS.
%
%
%
%
%


==> secs/mask-micro17/secs/abstract.tex <==
%!TEX root=../mask.tex

\begin{abstract}

\changesIV{Graphics Processing Units (GPUs)} exploit \changesI{large \changesII{amounts} of} thread-level parallelism to \changesI{provide high \changesIII{instruction} throughput and} \changesIII{to} efficiently
hide long-latency stalls. The resulting high throughput, 
along with continued programmability improvements,
have made GPUs an essential \changesIII{computational} resource in many domains.
\changesI{Applications from different domains can have \changesII{vastly} different \changesII{compute
and memory demands on the GPU}. 
\changesII{In a large-scale computing environment, to efficiently accommodate such 
wide-ranging demands without leaving GPU resources underutilized, multiple
applications can \emph{share} a single GPU, akin to how multiple applications
execute concurrently on a CPU.}
Multi-application concurrency requires several support mechanisms in \changesIII{both} hardware
and software. \changesIII{One such key mechanism is} \emph{virtual memory}, which manages and protects
the address space of each application.}
% Hence, in a large-scale computing environment, \emph{sharing} the
% GPUs across multiple applications can further increase GPU resource utilization.}
%Due to the heterogeneous compute requirements of different
%applications, there is a growing need to \emph{share} the GPU across multiple
%applications in large-scale computing environments.
However, \changesIII{modern GPUs lack the extensive support for 
multi-application concurrency available \changesIV{in} CPUs, and as a result suffer
from high performance overheads when shared by multiple applications,
as we \changesVIII{demonstrate}.}
% \changesIII{unlike CPUs, which have extensive
% support for multi-application concurrency, modern GPUs have only primitive
% support, which introduces high performance
% %support.  This primitive support introduces high performance
% overheads as we demonstrate in this paper.}
% unlike CPUs, which offer seamless multi-application concurrency 
% \changesII{by providing} hardware support 
% for multitasking and virtualization, GPUs currently \changesII{provide} only 
% primitive support for \changesII{such multi-application concurrency
% features.  As a result, it is cumbersome to share a contemporary GPU across
% multiple applications.}
% % multi-application concurrency.

% In contemporary GPUs, 
\changesII{We perform a detailed analysis of which \changesI{multi-application} concurrency support limitations 
hurt GPU performance the most.}
% \changesII{The} limited support for multi-application concurrency \changesII{in GPUs}} 
% is largely due to limitations within the memory system. 
% \changesII{In this work, we perform} a detailed analysis of challenges
% in state-of-the-art GPU virtual memory management that \changesII{hinder} multi-application 
% concurrency. 
\changesII{We find that the poor performance is largely a result of the 
virtual memory mechanisms \changesIV{employed in} modern GPUs.
In particular, poor address translation performance
is a key obstacle to efficient GPU sharing.}
% While existing 
% address translation mechanisms in GPU perform well when the GPU executes a
% single application, these mechanisms suffer greatly in the presence of multiple
% concurrently-executing applications.}
% \changesII{While} GPUs are designed to share memory between the CPU and GPU,
% \changesII{the existing mechanisms mechanisms do not work well when sharing memory}
% % but do not handle multi-application concurrency 
%  \emph{within the GPU}.
% %   well.  
\changesII{State-of-the-art address translation mechanisms, which were
designed for \changesIV{single-application} execution, experience} 
% when
% multiple applications spatially share the GPU, \changesII{due to} 
significant 
\changesII{\emph{inter-application \changesIII{interference}} when multiple applications spatially
share the GPU}. 
% \changesII{for the shared translation lookaside buffer (TLB)} 
% \changesI{a large amount of thrashing}.
\changesII{This contention leads to frequent misses in the shared translation
lookaside buffer (TLB), where a single miss can
induce long-latency stalls for hundreds of threads.}
% We found that TLB contention introduces long-latency stalls
% that hundred of threads must wait for. As a result of these TLB stalls, the
\changesI{\changesII{As a result, the GPU often cannot schedule enough threads}
% often do not have enough threads
to successfully hide the \changesII{stalls}, which
diminishes \changesIV{system} throughput and becomes a first-order performance concern.}
%TLB contention is high enough to prevent the GPU from successfully hiding
%stall latencies, becoming a first-order performance concern.

%This analysis forms the bases for 
\changesI{Based on our analysis, we propose} \titleShort{}, 
a \changesI{new GPU} \changesII{framework that provides} low-overhead virtual memory
support for the concurrent execution of multiple applications.
\changesII{\titleShort{} consists of three novel \changesIII{address-translation-aware} cache and memory management
mechanisms that work together to \changesIII{largely} reduce the overhead of address translation:}
% \titleShort{} extends the GPU 
% memory hierarchy to efficiently support address translation
% %with multi-level TLBs, 
% using translation-aware memory and
% cache management \changesII{mechanisms, which to maximize throughput in the presence of 
% cross-application contention. \changesI{\titleShort{} consists
% of three synergistic mechanisms.} \titleShort{} uses 
\changesI{(1)~a} token-based technique to reduce TLB \changesI{contention, (2)~a} %miss overheads.  
\changesII{bypassing mechanism to improve the effectiveness of cached address
translations, and (3)~an} application-aware memory 
scheduling \changesIII{scheme} to reduce the interference between address translation and 
data requests. \changesIII{Our evaluations show} that
\titleShort{} restores much of the \changesI{throughput} %thread-level parallelism previously
lost to \changesI{TLB contention.} %address translation. 
Relative to a state-of-the-art GPU TLB, 
% in the presence of contention,
\titleShort{} improves system throughput by 57.8\%, 
improves IPC throughput by 43.4\%, and reduces \changesIII{application-level} unfairness by 22.4\%. \titleShort{}'s
\changesI{system throughput} is within 23.2\% of \changesII{an} ideal \changesIII{GPU system} with 
no \changesIII{address} translation overhead. 

\end{abstract}

% \sloppypar{Compute density growth and advances in front-end programmability have made
% GPUs a compelling choice for many performance-hungry data-parallel applications.
% However, exposing GPUs to applications running in virtualized settings such 
% as Infrastructure-as-a-Service (IaaS) clouds remains problematic due to the lack of architectural support 
% for flexible fine-grained sharing. Although GPUs can be time-shared, the lack of software 
% control over preemption and memory protection leaves 
% system software bereft of the primitives needed to implement flexible QoS-based 
% resource management policies expected by cloud infrastructure users. Consequently,
% IaaS providers typically offer only restricted GPU support or no GPU support at all.}
% %Architectural support for fine-grain sharing of GPUs under a flexible policy
% %is urgently needed to make GPUs more accessible and usable in the 
% %cloud---support for multi-address-space concurrency can best address this need. }
% 
% By employing \emph{spatial multiplexing} instead of time-sharing, GPUs can
% concurrently execute kernels from multiple address spaces, and
% system software can  allocate GPU resources and enforce policies across contending 
% VMs, with or without support for preemption. 
% However, GPU spatial multiplexing relies on memory protection, 
% %and while
% %well-understood memory virtualization techniques are applicable in this setting, 
% and cross address space concurrency stresses the GPU memory subsystem in ways that 
% current memory hierarchies are not optimized for. In this work, we provide detailed
% analyses showing the huge overhead of address translation on GPUs and how 
% address translation become a major bottleneck of GPGPU applications despite GPU's
% inherent latency hiding capability. 
% %New techniques to 
% %reduce virtualization (i.e., address translation) overheads are required.


==> secs/mask-micro17/secs/ack.tex <==
\section*{Acknowledgments}

We thank the anonymous reviewers \changesIV{from ASPLOS 2017/2018, MICRO 2016/2017, and ISCA 2017.} 
\changesIV{We gratefully acknowledge SAFARI and SCEA 
group members} for their feedback. We acknowledge the support of 
our industrial partners, especially Google, Intel,
Microsoft, NVIDIA, and VMware. This research was
partially supported by the NSF (grants 1409723, 1618563, 1657336, and 1750667)
%(grants 0953246, 1065112, 1147397, 1205618, 1212962,
%1213052, 1302225, 1302557, 1317560, 1320478, 1320531, 1409095, 1409723,
%1423172, 1439021, 1439057, and 1618563), 
and the Semiconductor Research Corporation. \changesIX{An earlier version of this
paper was placed on arXiv.org in August 2017~\cite{mask-arxiv}.}



==> secs/mask-micro17/secs/component-eval.tex <==
\subsection{Component-by-Component Analysis}
\label{sec:component-analysis}


\para{Effectiveness of \tlbtokenname.} 
%To understand \titleShort{}'s efficacy at reducing thrashing,
Table~\ref{fig:tlb-baseline} compares the TLB hit rates of GPU-MMU and
\titleShort-TLB. We show only GPU-MMU results for TLB hit rate experiments, as the
TLB hit behavior for Static and GPU-MMU are similar. \titleShort-TLB increases
TLB hit rates by 49.9\% on average, which we attribute to \tlbtokenname. First,
\tlbtokenname reduces the number of warps utilizing the shared TLB entries,
which in turn reduces the miss rate. Second, the bypass cache can store
frequently-used TLB entries that cannot be filled in the traditional TLB.
Table~\ref{fig:tlb-bypass-hit} confirms this, showing the hit rate of the
bypass cache for \titleShort-TLB. From Table~\ref{fig:tlb-baseline}
and Table~\ref{fig:tlb-bypass-hit}, we conclude that the TLB-fill bypassing component
of \titleShort successfully reduces thrashing and ensures that frequently-used
TLB entries stay cached. 

%\begin{figure}[h!]
%     \centering
%     \subfloat[Aggregate TLB Hit Rates]{\includegraphics[width=0.49\columnwidth]{results/multi-tlb-hit-mask-tlb.pdf}}%
%     \subfloat[Hit Rate of the bypass cache]{\includegraphics[width=0.49\columnwidth]{results/bypass-cache-tall.pdf}}%
%     \caption{Effectiveness of \tlbtokenname.} 
%     \label{fig:tlb-baseline}
%\end{figure}



%\begin{figure}[h!]
%\centering
%\includegraphics[width=\columnwidth]{results/multi-tlb-hit-new.pdf}%
%\caption{Aggregate Shared TLB hit rates.} 
%\label{fig:tlb-baseline}
%\end{figure}



\begin{table}[h!]
%\begin{scriptsize}
\centering
\begin{tabular}{|c|c|c|c|c|}
        \hline
\textbf{Shared TLB} & \textbf{0 HMR}   & \textbf{1 HMR} & \textbf{2 HMR} & \textbf{Average} \\
\textbf{Hit Rate} & & & & \\
        \hline
        \hline
GPU-MMU & 47.8\% & 45.6\% & 55.8\% & 49.3\% \\
        \hline
\titleShort-TLB & 68.1\% & 75.2\% & 76.1\% & 73.9\% \\
        \hline
\end{tabular}%
\vspace{1em}
\caption{Aggregate Shared TLB hit rates.} 
\label{fig:tlb-baseline}
%\end{scriptsize}%
\end{table}%



%\begin{figure}[h!]
%\centering
%\includegraphics[width=\columnwidth]{results/bypass-cache-new.pdf}%
%\caption{TLB hit rate for bypassed cache.} 
%\label{fig:tlb-bypass-hit}
%\end{figure}

\begin{table}[h!]
%\begin{scriptsize}
\centering
\begin{tabular}{|c|c|c|c|c|}
        \hline
\textbf{Bypass Cache} & \textbf{0 HMR}   & \textbf{1 HMR} & \textbf{2 HMR} & \textbf{Average} \\
\textbf{Hit Rate} & & & & \\
        \hline
        \hline
\titleShort-TLB & 63.9\% & 66.6\% & 68.8\% & 66.7\% \\
        \hline
\end{tabular}%
\vspace{1em}
\caption{TLB hit rate for bypassed cache.}
\label{fig:tlb-bypass-hit}%
%\end{scriptsize}%
\end{table}%


\para{Effectiveness of \cachebypass.}
%To evaluate \cachebypass, 
Table~\ref{fig:tlb-data-hit} shows the average L2 data cache hit rate for
TLB requests. For requests that fill into the shared L2 data cache, \cachebypass is
effective in selecting which blocks to cache, resulting in a TLB request hit rate
that is higher than 99\% for all of our workloads.
%~\cjr{That's kind of astounding. Really? This strikes me as a potential red flag. 
%If every single application gets that much improvement there's probably something wrong.}  
%\rachata{This is only the hit rate for TLB-requests.}
At the same time, \cachebypass minimizes the
impact of bypassed TLB requests, leading to 17.6\% better
performance on average compared to GPU-MMU, as shown in Figure~\ref{fig:multi-ws}.

%\begin{figure}[h]
%\centering
%\includegraphics[width=\columnwidth]{results/multi-cache-hit.pdf}%
%\caption{L2 data cache hit rate for TLB requests.\cjr{change Y axis label, which is correct, but invites confusion!}} 
%\label{fig:tlb-bypass-hit}
%\end{figure}

\begin{table}[h!]
%\begin{scriptsize}
\centering
\begin{tabular}{|c|c|c|c|c|}
        \hline
\textbf{L2 Data Cache} & \textbf{0 HMR}   & \textbf{1 HMR} & \textbf{2 HMR} & \textbf{Average} \\
\textbf{Hit Rate} & & & & \\
        \hline
        \hline
GPU-MMU & 71.7\% & 71.6\% & 68.7\% & 70.7\% \\
        \hline
\titleShort-Cache & 97.9\% & 98.1\% & 98.8\% & 98.3\% \\
        \hline
\end{tabular}%
\vspace{1em}
\caption{L2 data cache hit rate for TLB requests.\cjr{change Y axis label, which is correct, but invites confusion!}} 
\label{fig:tlb-data-hit}
%\end{scriptsize}%
\end{table}%



\rachata{See if there are any changes in L2 nonTLB hit rate. Might improve due to lower contention.}

\para{Effectiveness of \dramsched.}
While the impact of the DRAM scheduler we propose is minimal for many applications,
(the average improvement across \emph{all} workloads is just 0.83\% in
Figure~\ref{fig:multi-ws}), we observe that a few applications that suffered more severely from
interference (see Figures~\ref{fig:dram-util}
and~\ref{fig:dram-latency})
can significantly benefit from our scheduler, since it prioritizes TLB-related
requests. Figures~\ref{fig:multi-dram-util}
and~\ref{fig:multi-dram-lat} compare the DRAM bandwidth utilization and
DRAM latency of GPU-MMU and \titleShort-DRAM for workloads that benefit
from \dramsched.  When our DRAM scheduler policy is employed,
SRAD from the SCAN-SRAD pair sees a 18.7\% performance improvement, while both
SCAN and CONS from SCAN-CONS have performance gains of 8.9\% and 30.2\%, 
respectively. In cases where the DRAM latency is high, the DRAM scheduler policy 
reduces the latency of TLB requests by up to 10.6\% (SCAN-SAD),
while increasing DRAM bandwidth utilization by up to 5.6\%
(SCAN-HISTO). 

\begin{figure}[h]
\centering
\resizebox{\columnwidth}{!}{%
\subfloat[DRAM Bandwidth Utilization]{{
	\includegraphics[height=80pt]{results/multi-dram-util.pdf}%
	\label{fig:multi-dram-util}
}}%
%\qquad
\subfloat[DRAM Latency]{{
	\includegraphics[height=80pt]{results/multi-dram-lat.pdf}%
	\label{fig:multi-dram-lat}
}}%
}
%\vspace{-1em}
\caption{DRAM bandwidth utilization and latency.\cjr{We could save space by 
		combining legends for all these graphs.}}

%\caption{DRAM bandwidth utilization (higher is better) and DRAM latency (lower is better).\cjr{We could save space by 
%		combining legends for all these graphs.}}
\label{fig:multi-dram}
\end{figure}


==> secs/mask-micro17/secs/eval.tex <==
\section{Evaluation}

\cjr{
\begin{compactitem}
\item Do GPU-MMU and Static enjoy the same oracular schedule? Would be more accurate at least for 
	Static to partition based on the available schemes for GRID. I'll bet that would leave some cores
	unused. \rachata{Yes. All of them enjoys the oracle. Note that we detach ourselves from GRID because
        of comments from MICRO reviewers. Essentially it is hard to claim what we model represents GRID due to
        limited informations.}
\item Might want to group plots by their category to save space.
\item We need to find a way to make plots bigger... \rachata{Grouping them by category might do the trick}
\item When using figure Xa, Xb, etc, we need to use the subcaption command instead of adding letters by hand--the colors aren't coming out right.
\item Of course, the real baseline that neither we nor our competitors include is a design with no memory protection, or one where address translation and TLBs are in the memory controller. Too late for ISCA probably, given that we have another paper to deal with as well.
\end{compactitem}
}

%To evaluate \titleShortMASK{}, we compare its performance against three designs.  The
We compare the performance of \titleShortMASK against three designs.  The
first, called \emph{Static}, uses a static spatial partitioning of resources, where an
oracle is used to partition GPU cores, but the shared L2 cache and memory
channels are partitioned equally to each application. This design is intended
to capture key design aspects of NVIDIA GRID and AMD FirePro---however,
insufficient information is publicly available to enable us to build a higher
fidelity model. The second design, called \emph{GPU-MMU}, models the flexible spatial
partitioning GPU MMU design proposed by Power et al.~\cite{powers-hpca14}.\footnote{Note that we
use the design in Figure~\ref{fig:tlb-mask-baseline} instead of the one in
Figure~\ref{fig:tlb-powers-hpca14}, as it provides better performance for the
workloads that we evaluate.} The third design we compare to is an \emph{ideal} scenario,
where every single TLB access is a TLB hit. We also report performance impact for individual
components of \titleShortMASK{}: \tlbtokenname(\titleShortMASK{}-TLB),
\cachebypass(\titleShortMASK{}-Cache), and \dramsched(\titleShortMASK{}-DRAM).

\subsection{Multiprogrammed Performance}
\label{sec:eval-multi-mask}

\begin{figure*}[ht!!!]
\centering
\vspace{-2em}
\includegraphics[width=\columnwidth]{secs/mask-micro17/results/ws-main-new-detail.pdf}%
\caption{System-wide weighted speedup for multiprogrammed workloads.} 
\vspace{-1em}
\label{fig:multi-ws-detail}
\end{figure*}



Figures~\ref{fig:multi-ws} and~\ref{fig:multi-ws-detail} compare the weighted speedup of multiprogrammed
workloads for \titleShortMASK{}, as well as each of the components of
\titleShortMASK{}, against Static and GPU-MMU. Each group of bars in the figure
represents a pair of co-scheduled benchmarks. Compared to GPU-MMU,
\titleShortMASK{} provides 45.7\% additional speedup. We also found that
\titleShortMASK performs only 23\% worse than the ideal scenario where the TLB always
hits. We observe that \titleShortMASK{} provides 43.4\% better aggregate throughput
(system wide IPC) compared to GPU-MMU. Compared to the Static baseline, where
resources are statically partitioned, both GPU-MMU and \titleShortMASK provide
better performance, because when an application stalls for concurrent TLB
misses, it does not use other shared resources such as DRAM bandwidth. During
such stalls, other applications can utilize these resources. When multiple
GPGPU applications run concurrently, TLB misses from two or more applications
can be staggered, increasing the likelihood that there will be heterogeneous
and complementary resource demand. 


\begin{figure}[ht!!!]
\centering
\includegraphics[width=0.7\columnwidth]{secs/mask-micro17/results/ws-main-new.pdf}%
\caption{System-wide weighted speedup for multiprogrammed workloads.} 
\label{fig:multi-ws}
\end{figure}


Figure~\ref{fig:multi-unfair} compares unfairness in \titleShortMASK{} against the
GPU-MMU and Static baselines. On average, our mechanism reduces
unfairness by 22.4\% compared to GPU-MMU.  As the number of tokens for each
application changes based on the TLB miss rate, applications that benefit more
from the shared TLB are more likely to get more tokens, causing applications
that do not benefit from shared TLB space to yield that shared TLB space to
other applications. Our application-aware token distribution mechanism and TLB
fill bypassing mechanism can work in tandem to reduce the amount of
inter-application cache thrashing observed in
Section~\ref{sec:motiv-inter-thrashing}. Compared to statically partitioning
resources in Static, allowing both applications access to all of the shared
resources provides better fairness.  On average, \titleShortMASK{} reduces
unfairness by 30.7\%, and a handful of applications benefit by as much as
80.3\%.


\begin{figure}[h]
\centering
%\vspace{-1em}
\includegraphics[width=0.7\columnwidth]{secs/mask-micro17/results/unfair-new.pdf}%
\caption{Max unfairness of GPU-MMU and \titleShortMASK.} 
%\vspace{-1em}
\label{fig:multi-unfair}
\end{figure}


\para{Individual Application Analysis.} \titleShortMASK{} provides better
throughput on all applications sharing the GPU due to reduced TLB miss
rates for each application. The per-application L2 TLB miss rates are reduced
by over 50\% on average, which is in line with the system-wide miss rates observed
in Figure~\ref{fig:tlb-baseline}. Reducing the number of TLB misses through
the TLB fill bypassing policy (Section~\ref{sec:fill-bypassing}), and
reducing the latency of TLB misses through the shared L2 bypassing
(Section~\ref{sec:data-bypassing}) and the TLB- and application-aware DRAM
scheduling policy (Section~\ref{sec:dram-sched-mask}) enables significant
performance improvement.
%\cjr{Are our mechanism names in harmony with the earlier text here?} 

In some cases, running two applications concurrently provides better speedup
than running the application alone (e.g., RED-BP, RED-RAY, SC-FWT). We
attribute these cases to substantial improvements (more than 10\%) of two
factors: a lower L2 queuing latency for bypassed TLB requests, and a higher L1
hit rate when applications share the L2 and main memory with other
applications.


\subsection{Component-by-Component Analysis}
\label{sec:component-analysis}

\para{The Effectiveness of \tlbtokenname.} 
%To understand \titleShortMASK{}'s efficacy at reducing thrashing,
Table~\ref{fig:tlb-baseline} compares the TLB hit rates of GPU-MMU and
\titleShortMASK-TLB. We show only GPU-MMU results for TLB hit rate experiments, as the
TLB hit behavior for Static and GPU-MMU are similar. \titleShortMASK-TLB increases
TLB hit rates by 49.9\% on average, which we attribute to \tlbtokenname. First,
\tlbtokenname reduces the number of warps utilizing the shared TLB entries,
which in turn reduces the miss rate. Second, the bypass cache can store
frequently-used TLB entries that cannot be filled in the traditional TLB.
Table~\ref{fig:tlb-bypass-hit} confirms this, showing the hit rate of the
bypass cache for \titleShortMASK-TLB. From Table~\ref{fig:tlb-baseline}
and Table~\ref{fig:tlb-bypass-hit}, we conclude that the TLB-fill bypassing component
of \titleShortMASK successfully reduces thrashing and ensures that frequently-used
TLB entries stay cached. 

%\begin{figure}[h!]
%     \centering
%     \subfloat[Aggregate TLB Hit Rates]{\includegraphics[width=0.49\columnwidth]{secs/mask-micro17/results/multi-tlb-hit-mask-tlb.pdf}}%
%     \subfloat[Hit Rate of the bypass cache]{\includegraphics[width=0.49\columnwidth]{secs/mask-micro17/results/bypass-cache-tall.pdf}}%
%     \caption{Effectiveness of \tlbtokenname.} 
%     \label{fig:tlb-baseline}
%\end{figure}



%\begin{figure}[h!]
%\centering
%\includegraphics[width=\columnwidth]{secs/mask-micro17/results/multi-tlb-hit-new.pdf}%
%\caption{Aggregate Shared TLB hit rates.} 
%\label{fig:tlb-baseline}
%\end{figure}



\begin{table}[h!]
%\begin{scriptsize}
\centering
\begin{tabular}{|c|c|c|c|c|}
        \hline
\textbf{Shared TLB} & \textbf{0 HMR}   & \textbf{1 HMR} & \textbf{2 HMR} & \textbf{Average} \\
\textbf{Hit Rate} & & & & \\
        \hline
        \hline
GPU-MMU & 47.8\% & 45.6\% & 55.8\% & 49.3\% \\
        \hline
\titleShortMASK-TLB & 68.1\% & 75.2\% & 76.1\% & 73.9\% \\
        \hline
\end{tabular}%
\vspace{1em}
\caption{Aggregate Shared TLB hit rates.} 
\label{fig:tlb-baseline}
%\end{scriptsize}%
\end{table}%



%\begin{figure}[h!]
%\centering
%\includegraphics[width=\columnwidth]{secs/mask-micro17/results/bypass-cache-new.pdf}%
%\caption{TLB hit rate for bypassed cache.} 
%\label{fig:tlb-bypass-hit}
%\end{figure}

\begin{table}[h!]
%\begin{scriptsize}
\centering
\begin{tabular}{|c|c|c|c|c|}
        \hline
\textbf{Bypass Cache} & \textbf{0 HMR}   & \textbf{1 HMR} & \textbf{2 HMR} & \textbf{Average} \\
\textbf{Hit Rate} & & & & \\
        \hline
        \hline
\titleShortMASK-TLB & 63.9\% & 66.6\% & 68.8\% & 66.7\% \\
        \hline
\end{tabular}%
\vspace{1em}
\caption{TLB hit rate for bypassed cache.}
\label{fig:tlb-bypass-hit}%
%\end{scriptsize}%
\end{table}%


\para{The Effectiveness of \cachebypass.}
%To evaluate \cachebypass, 
Table~\ref{fig:tlb-data-hit} shows the average L2 data cache hit rate for
TLB requests. For requests that fill into the shared L2 data cache, \cachebypass is
effective in selecting which blocks to cache, resulting in a TLB request hit rate
that is higher than 99\% for all of our workloads.
%~\cjr{That's kind of astounding. Really? This strikes me as a potential red flag. 
%If every single application gets that much improvement there's probably something wrong.}  
%\rachata{This is only the hit rate for TLB-requests.}
At the same time, \cachebypass minimizes the
impact of bypassed TLB requests, leading to 17.6\% better
performance on average compared to GPU-MMU, as shown in Figure~\ref{fig:multi-ws}.

%\begin{figure}[h]
%\centering
%\includegraphics[width=\columnwidth]{secs/mask-micro17/results/multi-cache-hit.pdf}%
%\caption{L2 data cache hit rate for TLB requests.\cjr{change Y axis label, which is correct, but invites confusion!}} 
%\label{fig:tlb-bypass-hit}
%\end{figure}

\begin{table}[h!]
%\begin{scriptsize}
\centering
\begin{tabular}{|c|c|c|c|c|}
        \hline
\textbf{L2 Data Cache} & \textbf{0 HMR}   & \textbf{1 HMR} & \textbf{2 HMR} & \textbf{Average} \\
\textbf{Hit Rate} & & & & \\
        \hline
        \hline
GPU-MMU & 71.7\% & 71.6\% & 68.7\% & 70.7\% \\
        \hline
\titleShortMASK-Cache & 97.9\% & 98.1\% & 98.8\% & 98.3\% \\
        \hline
\end{tabular}%
\vspace{1em}
\caption{L2 data cache hit rate for TLB requests.\cjr{change Y axis label, which is correct, but invites confusion!}} 
\label{fig:tlb-data-hit}
%\end{scriptsize}%
\end{table}%



\rachata{See if there are any changes in L2 nonTLB hit rate. Might improve due to lower contention.}

\para{Effectiveness of \dramsched.}
While the impact of the DRAM scheduler we propose is minimal for many applications,
(the average improvement across \emph{all} workloads is just 0.83\% in
Figure~\ref{fig:multi-ws}), we observe that a few applications that suffered more severely from
interference (see Figures~\ref{fig:dram-util}
and~\ref{fig:dram-latency})
can significantly benefit from our scheduler, since it prioritizes TLB-related
requests. Figures~\ref{fig:multi-dram-util}
and~\ref{fig:multi-dram-lat} compare the DRAM bandwidth utilization and
DRAM latency of GPU-MMU and \titleShortMASK-DRAM for workloads that benefit
from \dramsched.  When our DRAM scheduler policy is employed,
SRAD from the SCAN-SRAD pair sees an 18.7\% performance improvement, while both
SCAN and CONS from SCAN-CONS have performance gains of 8.9\% and 30.2\%, 
respectively. In cases where the DRAM latency is high, the DRAM scheduler policy 
reduces the latency of TLB requests by up to 10.6\% (SCAN-SAD),
while increasing DRAM bandwidth utilization by up to 5.6\%
(SCAN-HISTO). 

\begin{figure}[h]
\centering
%\resizebox{\columnwidth}{!}
{%
\subfloat[DRAM Bandwidth Utilization]{{
	\includegraphics[height=160pt]{secs/mask-micro17/results/multi-dram-util.pdf}%
	\label{fig:multi-dram-util}
}}%
%\qquad
\subfloat[DRAM Latency]{{
	\includegraphics[height=160pt]{secs/mask-micro17/results/multi-dram-lat.pdf}%
	\label{fig:multi-dram-lat}
}}%
}
%\vspace{-1em}
\caption{DRAM bandwidth utilization and latency.\cjr{We could save space by 
		combining legends for all these graphs.}}

%\caption{DRAM bandwidth utilization (higher is better) and DRAM latency (lower is better).\cjr{We could save space by 
%		combining legends for all these graphs.}}
\label{fig:multi-dram}
\end{figure}

\subsection{Scalability and Performance on Other Architectures}
\label{sec:750-eval}


Figure~\ref{fig:eval-scaling} shows the performance of GPU-MMU and \titleShortMASK,
normalized to the ideal performance with no translation overhead, as we vary the
number of applications executing concurrently on the GPU. We observe that
as the application count increases, the performance of both GPU-MMU and \titleShortMASK
are further from the ideal baseline, due to contention for shared
resources (e.g., shared TLB, shared data cache). However, \titleShortMASK provides
increasingly better performance compared to GPU-MMU (35.5\% for one
application, 45.7\% for two concurrent applications, and 47.3\% for three
concurrent applications). We conclude that \titleShortMASK provides better
scalability with application count over the state-of-the-art designs.

\begin{figure}[h]
\centering
\resizebox{\columnwidth}{!}
{%
\subfloat[Scalability analysis]{{
%\subfloat[Performance on different number of applications]{{
	\includegraphics[width=0.4\columnwidth,valign=t]{secs/mask-micro17/results/scaling-core.pdf}%
	\vphantom{\includegraphics[width=0.4\columnwidth,valign=t]{secs/mask-micro17/results/perf-arch.pdf}}%
	\label{fig:eval-scaling}
}}%

\subfloat[Performance on Fermi]{{
%\subfloat[Performance on different architectures.]{{
\includegraphics[width=0.4\columnwidth,valign=t]{secs/mask-micro17/results/perf-arch.pdf}%
\label{fig:eval-maxwell}
}}%
%\qquad
}
%\vspace{-1em}
\caption{Scalability (a) and portability (b) studies for \titleShortMASK.}
\label{fig:mask-scaling-and-arch}
\end{figure}

%While the evaluation presented in Section~\ref{sec:eval-multi} focuses on a GTX
%750 Ti GPU, which uses the Maxwell architecture, 
The analyses and designs of \titleShortMASK{} are architecture independent and
should be applicable to any SIMD machine. To demonstrate this, we evaluate
\titleShortMASK on the GTX 480, which uses the Fermi architecture~\cite{fermi}.
%\footnote{We tuned the pipeline configuration using
%configurations from the developmental branch of GPGPU-Sim. In addition, we configure the SIMD width to 64
%SIMD threads, with 8 memory controllers and a 1.5MB shared cache.}
Figure~\ref{fig:eval-maxwell} shows the performance of GPU-MMU and
\titleShortMASK{}, normalized to the ideal performance with no translation
overhead, for the GTX 480 and the GTX 750 Ti. We make three observations.
First, address translation incurs significant performance overhead in both
architectures for the baseline GPU-MMU design.  Second, \titleShortMASK{} provides
a 29.1\% performance improvement over the GPU-MMU design in the Fermi
architecture.  Third, compared to the ideal performance, \titleShortMASK{} performs
only 22\% worse in the Fermi architecture. On top of the data shown in
Figure~\ref{fig:eval-maxwell}, we find that \titleShortMASK{} reduces unfairness
by 26.4\% and increases the TLB hit rates by 64.7\% on average the in Fermi
architecture. We conclude that \titleShortMASK{} delivers significant benefits
regardless of GPU architecture.

%While the evaluation presented in Section~\ref{sec:eval-multi} focuses on a
%GTX 480 GPU, which uses the
%Fermi architecture, the analyses and designs of \titleShortMASK{} are architecture
%independent and should be applicable to any SIMD machine. To demonstrate this,
%we evaluate \titleShortMASK on the GTX 750 Ti, which uses the Maxwell
%architecture~\cite{maxwell}.\footnote{We tuned the pipeline configuration using
%configurations from the developmental branch of GPGPU-Sim. In addition, we configure the SIMD width to 64
%SIMD threads, with 8 memory controllers and a 1.5MB shared cache.}
%Figure~\ref{fig:eval-maxwell} shows the performance of
%GPU-MMU and \titleShortMASK{}, normalized to the ideal performance with
%no translation overhead, for the GTX 480 and the GTX 750 Ti. We make three observations.  First, address translation incurs significant
%performance overhead in both architectures for the baseline GPU-MMU design.
%Second, \titleShortMASK{} provides a 43.4\% performance
%improvement over the GPU-MMU design in the Maxwell architecture.
%Third, compared to the ideal performance, \titleShortMASK{} performs only 22\% worse in the
%Fermi architecture, and 24\% worse in the Maxwell architecture, both of which
%are significantly better than GPU-MMU's performance.
%We conclude that \titleShortMASK{} delivers significant benefits regardless of the
%specific GPU architecture.

\subsection{Hardware Overheads}
\label{sec:overhead-mask}

To support memory protection, each L2 TLB cache line adds an address space identifier (ASID).
In our evaluation, we added one byte per TLB entry for ASID bits, which translates to 7\% of the L2 TLB size. 

To support \tlbtokenname, we add two 16-bit counters at each shader core.
In the shared cache, we add a
32-entry fully-associative content addressable memory (CAM) for the bypass
cache, and 30 15-bit token counts with 30 1-bit token direction entries to support
the token distribution for 30 concurrent applications. In total, we add 436
bytes of extra space (4 bytes per core on the L1 TLB, and 316 bytes in the
shared L2 TLB). This additional overhead translates to 0.5\% growth of the L1 TLB and
3.8\% of the L2 TLB.

\cachebypass support adds ten 8-byte counters per core to track
cache hits and cache accesses per level, including the data cache
hit and accesses. This is 80 bytes total and is less than 0.1\%
of the shared L2 cache. Each cache and memory request contains an
additional 3 bits % of information 
specifying the page walk level, as discussed in
Section~\ref{sec:data-bypassing}.

\dramsched adds a 16-entry FIFO queue in each memory channel for TLB-related
requests, and a 64-entry memory request buffer per memory channel for the
\silverQ, while reducing the size of the \normalQ by 64 entries down to 192
entries. This adds an extra 6\% of storage overhead to the DRAM request queue per
memory controller.




==> secs/mask-micro17/secs/isca-abstract.tex <==
%!TEX root=../paper.tex

\begin{abstract}

\sloppypar{Compute density growth and advances in front-end programmability have made
GPUs a compelling choice for many performance-hungry data-parallel applications.
However, exposing GPUs to applications running in virtualized settings such 
as Infrastructure-as-a-Service (IaaS) clouds remains problematic due to the lack of architectural support 
for flexible fine-grained sharing. Although GPUs can be time-shared, the lack of software 
control over preemption and memory protection leaves 
system software bereft of the primitives needed to implement flexible QoS-based 
resource management policies expected by cloud infrastructure users. Consequently,
IaaS providers typically offer only restricted GPU support or no GPU support at all.}
%Architectural support for fine-grain sharing of GPUs under a flexible policy
%is urgently needed to make GPUs more accessible and usable in the 
%cloud---support for multi-address-space concurrency can best address this need. }

By employing \emph{spatial multiplexing} instead of time-sharing, GPUs can
concurrently execute kernels from multiple address spaces, and
system software can 
allocate GPU resources and enforce policies across contending 
VMs, with or without support for preemption. 
However, GPU spatial multiplexing relies on memory protection, 
%and while
%well-understood memory virtualization techniques are applicable in this setting, 
and cross address space concurrency stresses the GPU memory subsystem in ways that 
current memory hierarchies are not optimized for. 
%New techniques to 
%reduce virtualization (i.e., address translation) overheads are required.

\titleShort{} is a memory hierarchy design optimized for
spatial multiplexing across concurrently-running 
kernels from different address spaces. \titleShort{} extends the GPU 
memory hierarchy with address translation support,
including multi-level TLBs, and uses memory and
cache management to maximize throughput in the presence of 
cross-context contention. \titleShort{} uses a novel 
token-based approach to reduce TLB miss overheads.
L2 cache bypassing mechanisms and application-aware memory 
%We apply TLB-request-aware L2 cache bypassing policies and application-aware memory 
scheduling reduce interference between page-walk and 
data requests. Relative to a state-of-the-art GPU TLB,
\titleShort{} improves system throughput by 29.1\%, improves IPC throughput
by 27.2\%, and reduces unfairness by 23.3\%.~\cjr{update numbers?}

\end{abstract}


==> secs/mask-micro17/secs/obsolete-abstract.tex <==
\begin{abstract}

The compute density of GPUs makes them an attractive platform for
general purpose (GPGPU) applications with abundant
parallelism. Programmability advances in front-end tools such as CUDA
have made GPUs applicable in an increasingly broad set of application
domains. However, their applicability remains limited in virtualized 
settings---lack of fine grain software control over memory protection 
or preemption leaves system software such as OSes and hypervisors 
without the mechanisms required to provide QoS guarantees. 
We argue that support for cross-application concurrency on GPUs, or {\em
spatial multiplexing}, is a compelling approach to addressing these
shortcomings. 
%Eliding such support simplifies the hardware, but risks poor utilization and
%exposes applications to QoS pathologies such as starvation and
%unfairness, for example when processes with long-running kernels
%contend for the GPU against processes with short kernels. 
%\adwait{Last sentence is not required.}
%In cloud environments, where users pay for and expect a clearly-defined 
%quality-of-service, the inability to avoid resource allocation pathologies
%is anathema.
Spatial multiplexing can improve utilization and aggregate
throughput by co-scheduling applications with complementary resource demands.
%enabling meaningful QoS and isolation guarantees. 
Spatial multiplexing is effective with or without support for 
preemption. 
%Rachata: This part below is new
However, flexible spatial multiplexing also requires memory protection in form of
virtual address translation. We discover that the addition of the necessary
protection support through address translation of multiple applications creates
a new bottleneck: \emph{cross-application interference between
address-translation requests and data requests}, resulting in significant
negative impact on system performance.

%Rachata: This part was in the earlier version
%We argue that support for cross-application concurrency on GPUs, or {\em
%spatial multiplexing}, is a compelling approach to addressing these
%shortcomings. Spatial multiplexing can improve utilization and aggregate
%throughput by co-scheduling applications with complementary resource demands,
%enabling meaningful QoS and isolation guarantees. Spatial multiplexing is
%effective with or without support for preemption. However, cross-application
%concurrency requires memory protection. We find that with the addition of
%the necessary protection support, existing latency
%tolerance mechanisms are insufficient to hide the overheads of address 
%translation because of cross-application interference between 
%address-translation requests and data requests, resulting in significant 
%negative impact on system performance.

This paper presents \titleShort{}, a memory hierarchy design that enables
fine-grained, flexible, and {\em safe} spatial multiplexing of GPU resources
across kernels from different address spaces. \titleShort{} reduces cross-application
interference through three components:
%We focus on mechanisms to enable
%TLBs, page-walkers, and memory schedulers to better tolerate overheads from
%address translation and interference across protection domains. 
%\titleShort consists of three components: 
a novel token-based approach for mediating TLB access to the shared TLB that
ameliorates TLB miss burst overheads, an L2 cache bypassing mechanism that
reduces interference between page-walk requests and application data requests,
and an application-aware memory scheduler that is able to distinguish between
page-walk and data requests. \titleShort improves system throughput by
29.11\%, improves IPC throughput by 27.19\% and reduces unfairness by 23.3\%.
%\adwait{We should mention where is token based scheme employed? We should also
%say briefly  -- why the proposed mechanisms are GPU-specific or tie to the above
%observations.}

%\adwait{general comment -- abstract is too long. I fixed some small grammar/spelling
%issues. Rachata: can you take one more pass?}


% and reduce overall TLB miss rate by 61.3\%.}

%We find that
%a memory scheduling policy that is aware of TLB fill and page-walk
%operations can improve performance by XX\%, and that the degree of
%parallelism in page table walks has a first order impact on
%performance. \titleShort{} relies on a novel token-based approach to
%mediating TLB access that ameliorates TLB miss burst overheads,
%improving performance by YY\%.

%~\cjr{page table walk finding needs
%  update, along with nugget numbers for XX, YY.}
 
%~\aj{can we add 1-2 lines on why and how token-based scheme works}
 



% Comments:
% - Should we discuss how TLB affect concurrent apps, performance and fairness (QoS)
% - This work focuses on management of resources in the memory hierarchy (tlb, cache, main memory)
% under parallel GPU applications.

\end{abstract}




==> secs/mask-micro17/secs/obsolete.tex <==
\section{Old commented stuff moved from other sections to make editing less confusing}
 
 %A key components that is shared across multiple virtual machines is memory.
%Specifically, the memory management units (MMU) and the translation lookaside
%buffers (TLB) must be able to handle the unified address commonly used in
%recent GPUs, not only for a single GPGPU application but
%also for multiple GPGPU applications that are running on different virtual
%machines.  


%Lastly, kernels from different VMs must be isolated from each
%other not only in terms of performance (one VM's kernels
%shouldn't have perceptible impact on the performance of
%another's), but also data accessibility (kernels from different
%VMs should not be able to read or write eachother's memory). In
%this work, we provide an exhausive look at how the introduction
%of these components affect applications concurrently running on
%the GPU in terms of performance and fairness.  Then, we design
%an architecture that mitigate the performance overhead from the
%introduction of TLB and MMU in GPU systems.


%Not all kernels can fully utilize the resources available on a
%GPU. Some may exhibit abundant parallelism but under-utilize memory.
%Irregular parallel kernels may occupy fewer cores but consume more
%off-chip memory. Such heterogeneity with respect to resource
%consumption represents an opportunity to schedule kernels concurrently
%to improve utilization, and NVIDIA's support for concurrent
%kernels~\cite{Sanders:2010:CEI:1891996} (or {\it streams}), which enables kernels from a {\it
%  single application} to execute concurrently demonstrates that
%potential performance benefits are significant. However, while kernels
%from different applications could be co-scheduled to achieve similar
%gains, modern hardware cannot take advantage of this due to a lack of support
%for address translation and memory protection in upper layers of the
%memory hierarchy.
%\cjr{I think this paragraph is a distraction. Yes, we care about improving
%utilization, but that's a positive side-effect of what we're doing, not the 
%first-order goal.}


%As can be seen from Figure~\ref{fig:speedup-scale}, when more number of GPU cores
%are used to execute GPGPU applications, the additional speedup does not always
%scale linearly. In fact, we observe that several applications run into a plateau
%due to either their inherent limited amount of instruction level parallelism, which
%is defined as how many instructions can be executed in parallel or limited amount
%of memory level parallelism, which is how much off-chip memory can an application
%utilize in parallel.



%The introduction of TLBs and address translation caches entail fundamental
%overheads, particularly at the L2 level where such structures are shared. We
%explore this impact in single- and multiple-application settings to inform our
%design. We evaluated the TLB design both with and without the page walk cache,
%which is introduced in previous work to reduce the penalty of a TLB
%miss~\cite{powers-hpca14}, as well as with and without the shared TLB. For the
%workload we evaluated, we found that a design with a shared TLB and without the
%page walk cache yield comparable performance to a design with both a shared TLB
%and a page walk cache, and outperform an original design proposed by Powers et
%al.~\cite{powers-hpca14} by 9.1\%.  As a result, we choose to incorporate a
%shared TLB into the baseline design in this work.



%~\cjr{Is ``going to the memory partition'' 
%standard language that all reviewers are going to understand?}

%\rachata{Discuss other design issues here}
%\cjr{Umm...yes. Seems like actually, there's nothing yet that is specific to multiple
%apps...maybe the story needs to change?}
%



%\subsection{Performance between Designs}
%
%
%
%To illustrate tradeoffs between these three designs, we perform execute two
%concurrent GPGPU applications on MAFIA framework~\cite{mafia} with three
%different configurations: time-multiplexing, non-flexible spatial-multiplexing
%where each applications can access half of the available memory channels and
%flexible spatial-multiplexing where two applications can utilizing every memory
%channels. For both spatial-multiplexing designs, we configure the partitioning
%of GPU cores such that it yields the most weighted speedup (See
%Section~\ref{sec:meth}. Figure~\ref{fig:time-vs-space-vs-flex}a shows the
%performance, measured in weighted IPC speedup of two
%applications~\cite{harmonic_speedup,ws-metric2}, and
%Figure~\ref{fig:time-vs-space-vs-flex}b shows bandwidth utilization between
%these three designs. Several observations are in order. First, while the
%time-multiplexing design provide good individual performance for applications
%that get launched first, it is unfair toward applications that has to wait and
%execute later, leading to lower performance. Second, the non-flexible
%spatial-multiplexing design provides lower performance compared to the flexible
%spatial-multiplexing design as they has lower bandwidth utilization, which
%leads to lower throughput on both applications. Third, both time-multiplexing
%and non-flexible spatial multiplexing designs leads to lower DRAM utilization.

%\begin{itemize}
%\item No overprovisioning -- Every application has to make sure it does not exceed the GPU resources
%\item Limit parititioning
%\item Need programmer involvement
%\item No support for Security
%\item No demand paging --> Someone need to handle TLB flush. Previous paper addressed this.
%\end{itemize}
%\cjr{Rachata, I'm leaving this list in, to remind us to discuss in case you feel strongly we should talk about overcommit and paging. I think
%we should just point to related work on these.}
%

%\noindent\textbf{Design Considerations}
%We consider the implications of cross-address-space
%concurrency on GPU design. We explore the performance impact of adding address
%translation hardware throughout the entire memory hierarchy to motivate the
%design of \titleShort{} presented in Section~\ref{sec:design}.
%cjr{repetitive--not sure what this text is doing...}


%: address
%translation based on page tables. We assume an x86-like page-table
%structure with a register-based mechanism for setting the page-table
%root (a CR3-like register set by privileged software)
%per shader core.
%When a virtual address points to a
%physical location in DRAM not accessible from the application's
%virtual address space, the memory management unit detects and handles
%the violation by evicting the offending application from the shader
%core. 
%We do not consider demand paging in this work;
%our design is easily extended to adopt techniques described
%in~\cite{tianhao-hpca16}.  
%~\cjr{Rachata, is the L2 physically indexed
%  in your design? If so, no ASID-based eviction is necessary. If not,
%  then we need to put this text back: ``and invalidating all shared
%  TLB entries owned by it, which we detect with an added ASID in L2
%  cache lines.'' --> Rachata's answer: L2 is physically indexed in our design.}

%%to this end, we extend a design proposed by previous work on tlb
%\noindent\textbf{page walk cache and shared tlb.}
%%we begin from a tlb design proposed in~\cite{powers-hpca14} to support memory protection, shown in
%%figure~\ref{fig:tlb-baseline-design}a and~\ref{fig:tlb-baseline-design}b. 
%%each core has a private l1 cache. all cores share a highly-threaded 
%%page table walker (\mycirc{1}).  on a tlb miss, the shared
%%page table walker first probes the page walk cache (\mycirc{2})\footnote{in our evaluation,
%%we configure the page walk cache to 16-way 1024 entries}, then shared l2
%%cache and main memory. 
%figure~\ref{fig:tlb-baseline-design}b shows an alternative design suggested 
%in~\cite{powers-hpca14}. we eliminate the page walk cache,
%and dedicate the same chip area to the shared tlb. this design features
%two-level tlbs, with l2 tlb lines are extended with address space identifiers,
%and a parallel page table walker \mycirc{1}. tlb accesses from multiple threads
%to the same page are coalesced to reduce the number of active tlb-related
%requests and reduce interference in the memory system. on a tlb miss, 
%a page table walker starts walking the page directory \mycirc{2},
%then probes the shared l2 cache and main memory respectively \mycirc{4}. we
%compare the performance of the two designs using the parameters laid out in
%section~\ref{sec:meth}. for the workload we evaluated, we found that design b
%(shown in figure~\ref{fig:tlb-baseline-design}b) provide better performance
%across all except two workloads, and \emph{provides 10.9\% better average
%performance}. 
%\cjr{``only one workload? really?''}
%\rachata{two, to be exact. the reason because l2 cache (as seen in fig 8 and later on in fig 18) is pretty effectively at
%doing the job page walk cache suppose to be doing.}
%we find that the shared data cache enables a hit rate for the page table 
%walker that is competitive with a dedicated page walk cache.
%%(when used to cache content of page table walks).
%%because we found that shared tlb up to 82\% hit rate. 
%given the same chip area, it is more
%beneficial to dedicate the area to a shared tlb. consequently, we selected 
%design b as our baseline tlb design in this work, as it \emph{provides better
%performance with similar chip area}.


%GPU throughput relies heavily on \emph{fine-grained 
%multithreading}~\cite{cdc6600,smith-hep} to hide memory latency.
%However, we find that the introducing address
%translation hardware limits the GPU's ability to effectively hide
%latency. 

%Rachata: Moved up to Section 3-new
%\subsection{Bottlenecks Caused By Address Translation}
%\label{sec:tlb-bottleneck}
%
%
%
%%\adwait{this sub-section does not have any results for multiple-application.
%%Should we change the sub-title?}
%%
%%\adwait{If we decide to move 3.1 to section 2, we should open this section
%%with clear goal of this section. As I understand, we are trying to show that
%%multiple application interference can severely hamper TLB misses leading to
%%very poor performance/latency tolerance. Am I correct?}
%%\rachata{Moved old 3.1 to the end of Section 2}
%%
%%%\subsection{Slowdowns due to TLB Misses: Single Application}
%%%\subsection{TLB Misses: Single Application}
%%%\label{sec:tlb-miss}
%%
%%To understand this effect of address translation, we In this subsection, we
%%first analyze the effect of TLB miss latency on GPGPU applications'
%%performance. To perform this analysis, we eliminate the interference between
%%page-table-walk-related data and non-page-table-walk-related data throughout
%%the memory hierarchy by tying TLB miss to a fixed latency instead of the usual
%%page table walking routine.  This eliminates page table walker to probe L2 as
%%well as main memory and prevent the page table data to trash L2 and DRAM.
%%Figure~\ref{fig:tlb-latency-sweep} shows the performance of GPGPU applications
%%under various TLB miss latency. 
%%%In this experiment, we intentionally eliminate any interference from TLB-related data
%%%at both the shared L2 cache as well as the DRAM main memory by setting a TLB
%%%miss to a fixed latency, and prevent the page table walker from probing L2
%%%cache and DRAM. 
%%From~\ref{fig:tlb-latency-sweep}, we observe that there is a
%%significant slowdown even though 1) the TLB miss latency is set to a value
%%close to a roundtrip latency of a single DRAM requests 2) TLB miss does not
%%cause interference to the shared L2 data cache and 3) TLB miss does not consume
%%additional bandwidth at the main memory, the performance of GPGPU applications
%%degrade significantly in most GPGPU applications.
%%
%%\adwait{I am not sure if reviewers will be convinced with these latency sweep
%%results. Can we show this particular problem with real multiple-application 
%%interference data?}
%%
%%
%%\begin{figure}[h!]
%%     \vspace{3pt}
%%	\centering
%%	\includegraphics[width=0.9\columnwidth]{figs/ipc_vs_tlb.pdf}%
%%        \vspace{-1pt}
%%	\caption{Performance slowdown under different TLB miss latency.} 
%%        \vspace{-10pt}
%%	\label{fig:tlb-latency-sweep}
%%\end{figure}
%%
%%
%%\rachata{This might be a good place to argue why Powers et al.'s design is lacking
%%(hit rate compared to using L2 data cache is not significantly higher. Any subsequent
%%misses still incur high latency. Hence, it is better to reduce tlb miss altogether instead.)}
%
%Despite parallelization of page table walks, we observe that GPGPU applications
%slow down significantly. To understand the reason behind this significant
%slowdown, Figure~\ref{fig:stall-tlb} illustrates an example during the
%execution of a GPGPU application where all warps want to access data from
%memory%, with and without virtual-to-physical address translation. 
%Without virtual-to-physical address translation
%(Figure~\ref{fig:stall-tlb}a), when a GPU core executes one of its long latency
%memory instruction (shown as the grey box labeled Warp A), shown as instruction
%for warp A in Figure~\ref{fig:stall-tlb}a, the core does not stall as long as
%there are other warps to schedule from. In this case, the GPU core will select
%one of the remaining warps (warp B-H) to execute the next cycle (\mycirc{1}).
%This way, the core can keep executing useful instructions while waiting for
%memory requests generated by warp A. As a result, after executing all these
%warps, the core sends all necessary data requests to DRAM. However, with the
%introduction of the virtual-to-physical address translation, shown in
%Figure~\ref{fig:stall-tlb}b, suppose that now warp A runs into a TLB miss. In
%this case, any other threads that need the data from the same page as warp A
%also has to stall (as shown in the example where warp B-D, shown as lighter red
%block, now also has to stall waiting for warp A's page walk), neither fetching
%their data, nor executing useful instructions (\mycirc{2}). Similar problem
%happens to where a TLB miss caused by Warp E stalls Warps E-G (\mycirc{3}). During
%this time when GPU core is stalling, the only warp that is fetching an actual 
%data is Warp H (\mycirc{4}), while Warps A-G has to wait until the two page table
%walk (\mycirc{2} and \mycirc{3}) finish. In
%this example, we have shown two phenomenon. First, there are significantly
%fewer number of available warps the core can schedule from due to stalled
%induced by a TLB miss. Second, during this TLB-induced stall, warps (A through
%G) are not able to send necessary DRAM requests until TLB-miss is resolved.
%Thus, reducing the chance that GPU can hide latency. 
%%\rachata{Need to figure out how to make this
%%paragraph stronger. Essentially what I want to say is that 1) Fewer warps are
%%available and 2) For those warps that get stalled due to a TLB miss, they are
%%not making use of DRAM bandwidth.} Because a TLB miss can stall multiple warps,
%%the GPU's latency-hiding capability is reduced: fewer warps are available to be
%%scheduled at any given time. 
%
%%To understand the impact of this on GPU performance, 
%%Figure~\ref{fig:stall-tlb}c shows an example of GPU stalls caused by a single TLB miss
%
%
%%In the worst case, a TLB miss can stall {\em all} threads across multiple warps
%%that access data on a page, leading to much lower latency hiding capability as
%%shown in Figure~\ref{fig:stall-tlb}. 
%
%%In this example, there are in total
%%four warps in a shader core: $A$, $B$, $C$, $D$. Each warp has four threads,
%%and all threads are executing a series of load instructions.
%%Five of the threads want to access addresses on a page mapped by 
%%the same TLB entry, but the translation is out of the TLB cache, causing a TLB miss, as shown in Figure~\ref{fig:stall-tlb}a. 
%%Because the GPU executes instructions in lockstep, this causes high latency stalls for 
%%all threads on both warp $A$ and $B$. 
%%Additionally, because GPUs execute
%%instructions in lockstep, the entire warp containing these five stalled
%%threads is stalled, even if other threads are hitting in both the TLB
%%and the data cache.
%%% as shown in Figure~\ref{fig:stall-tlb}a.
%
%\begin{figure}[h!]
%     \vspace{-5pt}
%	\centering
%	\includegraphics[width=0.9\columnwidth]{figs/tlb-stall.pdf}%
%        \vspace{-5pt}
%	\caption{An example of bottleneck created by TLB misses.} 
%        \vspace{-5pt}
%	\label{fig:stall-tlb}
%\end{figure}
%
%To further understand the impact of TLB miss latency to the performance of
%GPGPU applications, 
%%Figure~\ref{fig:schedulable-warp}a shows the average number
%%of concurrent TLB for each application, with brackets showing the standard
%%variation, and 
%Figure~\ref{fig:schedulable-warp} shows the number of warps being stalled per
%active TLB misses (misses that are going through the page table walking
%process) as well as the average number of concurrent page walks across
%different GPGPU applications. From this figure, we conclude that GPGPU
%applications' large number of concurrent TLB misses cause significant number of
%warps to stall, without fetching its needed data to DRAM, leading to
%significant slowdown for various GPGPU applications.
%
%
%\begin{figure}[h!]
%     \vspace{-5pt}
%	\centering
%	\includegraphics[width=0.9\columnwidth]{figs/stalled_per_miss.pdf}%
%        \vspace{-5pt}
%	\caption{Average number of stalled warp per active TLB miss and number of concurrent page walks.} 
%        \vspace{-5pt}
%	\label{fig:schedulable-warp}
%\end{figure}
%
%According to this data, it is crucial to minimize the number of TLB misses
%as well as minimize the latency of page table walk. While the page walk cache
%and the shared L2 cache can be utilized to reduce the penalty of TLB misses.
%In the next section, we provide further analyses on how page-walk-related
%data interfere with different components throughout the memory hierarchy.
%
%%TODO: Check this part
%%With the reduction in the number of schedulable warp, we also observe severe
%%reduction in DRAM bandwidth utilization when the latency of TLB miss gets
%%higher as shown in Figure~\ref{fig:dram-util-drop}. This reduction in DRAM
%%utilization occur due to the drop in the number of schedulable warp as the
%%majority of GPU warps are stalled due to TLB miss rather than concurrent memory
%%requests, as we discussed in a high level in Figure~\ref{fig:stall-tlb}b.
%%
%%\adwait{I did not understand the importance of Figure~\ref{fig:dram-util-drop} in this
%%section. I think there are significant flow issues.}
%%
%%\rachata{Now that I reread it, I agree that the above paragraph breaks the flow...}
%%
%%\begin{figure}[ht!]
%%     \vspace{3pt}
%%	\centering
%%	\includegraphics[width=0.9\columnwidth]{figs/bw_vs_tlb.pdf}%
%%        \vspace{-1pt}
%%	\caption{Decrease in DRAM bandwidth utilization as TLB miss latency increases.} 
%%        \vspace{-10pt}
%%	\label{fig:dram-util-drop}
%%\end{figure}
%
%
%
%
%%Because a TLB miss can stall multiple warps, the GPU's
%%latency-hiding capability is reduced: fewer warps are available to be
%%scheduled at any given time. 
%%%To understand the impact of this on GPU performance, 
%%Figure~\ref{fig:stall-tlb}b shows an example of GPU stalls caused by a single TLB miss
%%that stalls warps $A$ and $B$. 
%%In this example, while warps $A$ and $B$ stall and wait
%%for address translation, the shader core only has warp $C$ and $D$ available for scheduling.
%%Because each load instructions in $C$ and $D$ takes 4 cycles, and there are no other available
%%warps, the entire GPU core stalls. 
%%%This example shows how
%%%a single TLB miss can significantly effect latency hiding capability of the GPU.
%
%%In this example, 8 warps are in the
%%GPU cores (warp $A$ to $H$, all currently executing an 8-cycle load instruction).
%%%Figure~\ref{fig:stall-tlb}a shows that when none of
%%%these 8 warp are stalled due to TLB, in this case, by the time warp $A$ gets
%%%its data back 8 cycles later, the warp is available and the GPU can execute
%%%warp A again. In this case, GPU core never stalls. 
%%Figure~\ref{fig:stall-tlb}b shows a case in which three warps, $A$, $B$ and $C$, 
%%are waiting for a single TLB miss () and therefore cannot issue the load instruction. 
%%%%In this case, warps  cannot issue to load instruction due to a
%%%%TLB miss. 
%%As a result, the GPU cores can only schedule instructions
%%from the remaining warps, leading to GPU stall.
%%%% as shown in Figure~\ref{fig:stall-tlb}b.
%%\cjr{This is not clear. I've tried to clean it up, but I think it needs
%%some more attention. Where is Warp C in the figure? We need to be very 
%%explicit why we can't schedule from D-H: the warps occupying the cores
%%appear to have misses, which looks like precisely the case GPU multi-threading
%%is designed for. 
%%}
%
%
%
%%\begin{figure}[ht!]
%%     \vspace{3pt}
%%	\centering
%%	\includegraphics[width=0.9\columnwidth]{figs/tlb-stall-sample.pdf}%
%%        \vspace{-1pt}
%%	\caption{Reduction in GPU latency hiding capability due to TLB misses.} 
%%        %\vspace{-10pt}
%%	\label{fig:stall-tlb-sample}
%%\end{figure}
%
%
%
%%To illustrate the effect of TLB misses on GPGPU applications,
%%Figure~\ref{fig:ideal-baseline} shows the performance of the TLB design
%%described above with different TLB miss latency compared to an ideal design
%%with zero TLB latency. We run these experiments on Mafia
%%framework~\cite{mafia} using a previously proposed GPU-MMU
%%design~\cite{powers-hpca14} as described in Section~\ref{sec:meth} and
%%Figure~\ref{fig:tlb-baseline-design}.
%%%Rachata: New
%%%While the GPU-MMU design~\cite{powers-hpca14} do not have the shared TLB as the
%%%authors observed that a page walk cache outperforms a shared TLB in
%%%applications evaluated in GPU-MMU, in this work, we evaluate a TLB design with
%%%a shared TLB but no page walk cache and compared it against a design without a
%%%shared TLB but has a page walk cache. For the workload we evaluated, we
%%%observed that a design with a shared TLB but without a page walk cache
%%%outperforms the other design by roughly 9\% on average on multi-programmed
%%%scenario.  Additionally, we found that for the applications we evaluated,
%%%adding a page walk cache with a shared TLB does not make a significant
%%%performance improvement.  Hence, we choose to replace the page walk cache with
%%%a shared TLB. 
%%In the ideal case, we fill the TLB miss to the TLB entry right
%%away, so that subsequent requests to the same page incur a TLB hit. The results
%%show that while the GPU can tolerate long memory latencies for data requests,
%%it is more susceptible to long TLB miss requests, as any threads that need to
%%access pages covered by pending TLB misses are stalled. 
%
%%To illustrate the effect of TLB misses on GPGPU applications,
%%Figure~\ref{fig:ideal-baseline} shows the performance of the TLB
%%design described above compared to an ideal design with zero TLB latency.  We run
%%these experiments on Mafia framework~\cite{mafia} using a previously proposed
%%GPU-MMU design~\cite{powers-hpca14} as described in Section~\ref{sec:meth} and Figure~\ref{fig:tlb-baseline-design}.
%%%Rachata: New
%%While the GPU-MMU design~\cite{powers-hpca14} do not have the shared TLB as the
%%authors observed that a page walk cache outperforms a shared TLB in
%%applications evaluated in GPU-MMU, in this work, we evaluate a TLB design with
%%a shared TLB but no page walk cache and compared it against a design without a
%%shared TLB but has a page walk cache. For the workload we evaluated, we
%%observed that a design with a shared TLB but without a page walk cache
%%outperforms the other design by roughly 9\% on average on multi-programmed scenario.
%%Additionally, we found that for the applications we evaluated, adding a page
%%walk cache with a shared TLB does not make a significant performance improvement.
%%Hence, we choose to replace the page walk cache with a shared TLB. In the ideal
%%case, we fill the TLB miss to the TLB entry right away, so that subsequent
%%requests to the same page incur a TLB hit. The results show that while the GPU
%%can tolerate long memory latencies for data requests, it is more susceptible to
%%long TLB miss requests, as any threads that need to access pages covered by
%%pending TLB misses are stalled. 
%
%
%
%%This slowdown increases with
%%memory size because the depth of page table walks increases. We conclude that
%%minimizing the number  of TLB misses as well as reducing their latency is
%%critical to GPU performance.
%
%%~\cjr{This is kind of an obvious conclusion. It would
%%be more convincing if we arguing that the effect is somehow worse than we predicted or
%%worse than others have predicted.}
%
%%\begin{figure}[h]
%%     \vspace{3pt}
%%	\centering
%%	\includegraphics[width=0.8\columnwidth]{results/level_sweep.pdf}
%%        \vspace{-1pt}
%%	\caption{Performance comparison between an ideal result to different TLB miss latency. TODO: Change the plot once data are parsed} 
%%        \vspace{-10pt}
%%	\label{fig:ideal-baseline}
%%\end{figure}


%\subsection{Overhead of Address Translation on Multiple GPGPU Applications}

% in this Section, we
%evaluated the impact of TLB shootdowns on system performance.

%To understand the effect of TLB shootdowns on performance, we synthetically
%inject TLB flush request periodically. During the shootdown, affected TLB
%entries are invalidated. During the invalidation, all TLB entries are blocked
%and any subsequent TLB accesses has to walk the entire page table. We modeled
%the time needed for the invalidation using CACTI 6.5~\cite{cacti} and then rounded
%to the closest number of cycles. Figure~\ref{fig:flush} shows the effect of
%TLB flush on GPGPU application's performance base on various flush frequency.

%\rachata{It might be useful to do a brief summary of this section here}

%
%Figure~\ref{fig:tlb-miss-breakdown} shows that the TLB is the bottleneck for
%these applications. We observe two trends. First, for applications with
%significant L1 and L2 TLB misses, the miss rate is highly correlated with
%application performance. The resulting slowdowns can be severe, also observed
%by previous works on GPU TLB designs~\cite{powers-hpca14, abhishek-tlb,
%abhishek-ispass16}. Second, significant thrashing occurs in the shared L2 TLB
%due to the large number of parallel TLB requests even with one application
%utilizing the shared TLB.  
%Moved this discussion up GPGPU applications generally have high locality
%within a page (as can be seen through the high row buffer hit
%rate~\cite{gpgpu-sim,demystify,sms}, where the row buffer is at the same
%granularity as a page), so multiple concurrent TLB misses are likely to stall
%the progress of many warps in a shader core. The GPU is unable to hide all
%this latency, and degraded performance is the result. 





%\noindent\textbf{Minimizing TLB Misses is Critical.} One primary source of
%application slowdown comes from interference from one applications' to a
%TLB-related requests to shared resources (shared cache and main memory) of
%another application. Figure%TODO: A figure show one application TLB requests,
%where many threads are waiting, get blocked shows an example of potential stall
%time due to an interference to a TLB requests.  While a typical memory stall
%can stall a warp, TLB-miss takes longer to be serviced and likely to stall
%multiple warps that has to access data in the page. While GPU can generally
%tolerate long latency memory request, GPU are less likely to be able to
%tolerate long TLB-miss latency.

%This is repeated of above material
%\textbf{Interference at the Shared TLB.} As illustrated in
%Section~\ref{sec:tlb-miss}, TLB misses can harm GPU performance, despite the
%GPU's latency-tolerant design.  When multiple applications are sharing the GPU,
%the interference to the shared TLB can further degrade performance, as the
%likelihood of entries being shared across shader cores decreases. 

%\rachata{Move the discussion on the page walk cache here?}

%\rachata{Note: What I want to say here is along the
%line of GPU cache is there to filter out excess off-chip bandwidth, not for its
%low latency. Unless every thread hits in the cache, the whole warp stalls for
%the entire DRAM latency.  However, with TLB-related data, this is different as
%it operates in threads granularity (page table walker), not in warp
%granularity.}

%With the introduction of the address translation, shared L2 data cache can
%also
%be used to cache page-table-walk-related data. However, this introduce another
%source of interference is the shared cache. Both TLB-related data as well as
%applications' data contend for the space in the shared cache, causing
%additional interference as well as long queueing latency~\cite{medic-pact}. 

%Address translation incurs memory references
%(page-table walks) to handle TLB misses, so adding TLBs to a GPU
%memory hierarchy introduces the possibility of interference between
%TLB-miss activity and normal data operations, even within a single
%application. 
%Figure~\ref{fig:tlb-miss-interference-example} shows an
%example of this interference.  

%These two plots provide the evidence that,
%even though there are significantly smaller number of page-walk-related data,
%the latency of these page-walk-related requests are still as high, or sometimes
%even higher than normal data requests due to memory interference.  Depending on
%how many times page table walker have to access the main memory, the latency
%penalty of a TLB miss gets increasingly higher. Thus, it is increasingly harder
%for GPU to hide the latency TLB miss as discussed in Section~\ref{sec:tlb-bottleneck}.
%
%When page table walks handles TLB miss at all levels of the hierarchy, accesses
%to main memory are necessary. 
%GPU applications typically have high row buffer
%hit rates. Previous work on memory scheduling, such as the
%FR-FCFS~\cite{fr-fcfs,frfcfs-patent} scheduler takes advantage of that fact by
%prioritizing accesses that hit in the current row buffer. We find that this
%policy often ends up prioritizing non-TLB-related memory request over
%TLB-related memory requests. As a result, TLB-related requests, particular
%those accessing leaf nodes of the page table, can queue up at the memory
%controller, harming performance by increasing queueing delay.





%When page table walks handles TLB miss at all levels of the hierarchy, accesses
%to main memory are necessary. GPU applications typically have high row buffer
%hit rates. Previous work on memory scheduling, such as the
%FR-FCFS~\cite{fr-fcfs,frfcfs-patent} scheduler takes advantage of that fact by
%prioritizing accesses that hit in the current row buffer. We find that this
%policy often ends up prioritizing non-TLB-related memory request over
%TLB-related memory requests. As a result, TLB-related requests, particular
%those accessing leaf nodes of the page table, can queue up at the memory
%controller, harming performance by increasing queueing delay.
%
%Figure~\ref{fig:dram-util} shows the breakdown of DRAM bandwidth utilization
%(measure as the fraction of the total DRAM bandwidth) while
%Figure~\ref{fig:dram-latency} compare the latency of a normal data request with
%page-walk-related data requests. These two plots provide the evidence that,
%even though there are significantly smaller number of page-walk-related data,
%the latency of these page-walk-related requests are still as high, or sometimes
%even higher than normal data requests due to memory interference.  Depending on
%how many times page table walker have to access the main memory, the latency
%penalty of a TLB miss gets increasingly higher. Thus, it is increasingly harder
%for GPU to hide the latency TLB miss as discussed in Section~\ref{sec:tlb-bottleneck}.


%From these data, we make the following
%observations on page-table-walk-related data. First, the
%page-table-walk-related data make up only a small fraction of the total
%off-chip bandwidth of each application. Second, even though there are
%significantly smaller number of page-table-walk-related data, the latency of
%these requests are still as high, or sometimes even higher than normal data
%requests. As a result, depending on how many times page table walker have to
%access the main memory, the latency penalty of a TLB miss gets increasingly
%higher and it become increasingly harder for GPU to hide these long latency TLB
%miss as discussed in Section~\ref{sec:tlb-bottleneck}.

%\adwait{Figure~\ref{fig:dram-util} seems interesting. Do we evaluate the 
%effect of always prioritizing TLB misses in the memory controller? I think
%it can significantly improve the performance.}
%
%\rachata{I did, I also evaluated a new DRAM policy to prevent one application
%to starve the other application. I will add this part to the mechanism}




% This turn out too small
%
%
%\begin{figure}[h!]
%    \centering
%    \begin{subfigure}[t]{0.45\textwidth}
%        \centering
%	\includegraphics[width=\columnwidth]{figs/dram_util_2apps.pdf}%
%	\caption{Bandwidth breakdown of two applications.} 
%    \end{subfigure}%
%    ~
%    \begin{subfigure}[t]{0.45\textwidth}
%        \centering
%	\includegraphics[width=\columnwidth]{figs/dram_latency.pdf}%
%	\caption{Latency breakdown of two applications.} 
%    \end{subfigure}
%\end{figure}
%



%Aside from the effect of page translation on the effective DRAM bandwidth, when
%multiple GPGPU applications are concurrently running. It is possible that one
%GPGPU application occupies most, if not all, GPU resources at any given time.
%This results in severe slowdown for other GPGPU applications that are
%concurrently running. Figure~\ref{fig:slowdown-example} shows a case of two
%GPGPU applications, both of which enter the memory-bound episode at the same
%time. As shown, the first GPGPU application enters the memory bound episode
%slightly before the second GPGPU application. Three observation are in order.
%First, because the first application gets to send most of it memory request
%before the second application, when the second application enters its memory
%episode, the shared cache are being filled by data from the first applications,
%causing the initial slowdown for the second application. Second, after the
%second application enters it memory episode for a while, interference from both
%applications causes severe slowdown to both application. 


%When multiple GPGPU applications are concurrently running. It is possible that
%one GPGPU application occupies most, if not all, GPU resources at any given
%time. This results in severe slowdown for other GPGPU applications that are
%concurrently running. Figure~\ref{fig:slowdown-example} shows a case of two
%GPGPU applications, both of which enter the memory-bound episode at the same
%time. As shown, the first GPGPU application enters the memory bound episode
%slightly before the second GPGPU application. Three observation are in order. First,
%because the first application gets to send most of it memory request before
%the second application, when the second application enters its memory episode,
%the shared cache are being filled by data from the first applications, causing
%the initial slowdown for the second application. Second, after the second application
%enters it memory episode for a while, interference from both applications causes
%severe slowdown to both application. 
%
%To mitigate both problems, it is important to 1) identify the critical request,
%and prioritize them throughout the entire memory hierarchy and 2) minimize
%applications interference across applications. Sections~\ref{sec:mech-interfere}
%described our design.

%% cjr: moved this from intro, where it seemed too detailed. 
%% can't find the figure?
%Figure~\ref{fig:tlb-miss-interference-example} illustrates this interference.
%While it is desirable to minimize the TLB miss latency by allowing data
%generated by the page table walk routing to probe the shared cache. These
%TLB-related data can interfere and thrash data cache entries and lower the
%performance of the GPU. This create an interesting trade-off between
%prioritizing TLB related request and a typical data request in GPU memory
%hierarchy. As we pointed out in Section~\ref{sec:way-part}, \rachata{Continue here}
%\cjr{Not sure why this is here...would delete it but there's a Rachata note...}

%TODO: Explain the result from way partitioning in L2. Interfererence from TLB to L2 data cache

%Figure~\ref{fig:impact-fault} shows the performance impact of a system with two
%GPGPU applications running and one GPGPU application causing multiple TLB
%flushes in a row compared to the case when both applications are running alone.
%In this case, the performance of the GPGPU application is heavily affected by
%the aggressor GPGPU application that causes multiple TLB flushes. In this case,
%we propose a TLB design that prevent both access violation as well as performance
%impact due to faults from other GPGPU applications.

%
%% Data stored in the root and levels closer to root node generally has more
%% sharers across multiple threads in GPU programs while data stored in
%% close-to-leaf nodes is less likely to be shared across threads. As a result, it
%% is much more likely for memory requests closer to the root nodes to hit in the
%% shared L2 cache, significantly minimizing the latency of TLB-miss.

%while it is not as destructive to completely bypass the shared L2 cache for data closer to
%the leaf node of a page table walking routine as by the time TLB miss to the same entry
%happens again, the data is more than likely to be evicted from the shared cache.
%%TODO: Plot showing cache hit rate of each TLB-related accesses

%Aside from the cache bypassing to eliminate interference in the shared L2
%cache, 
\rachata{We can probably cut this if needed}
We also explored cache partitioning between page-walk- and non-page-walk-related data to
further reduce TLB miss overheads. However, partitioning the shared L2 cache
ways for TLB-related data comes with two downsides. First, cache partitioning
reduces the effective L2 cache for non-TLB-related data. Second, cache
partitioning do not decrease the queuing latency accessing the cache. We find
that with just one way per set dedicated to address translations, GPGPU
applications incur a 3\%-5\% increase in L2 cache miss rate relative to the
design with no way partitioning, so our design elides this technique.


%\begin{table*}[t!]
%\begin{scriptsize}
%  \centering
%\vspace{3pt}
%    \begin{tabular}{ll}
%        \toprule
%%        \hline
%\textbf{System Overview}           &  30 cores, 6 memory partitions\\
%        \cmidrule(rl){1-2}
%\textbf{Shader Core Config}           &  1400 MHz, 9-stage pipeline, GTO scheduler~\cite{ccws}\\
%        \cmidrule(rl){1-2}
%\textbf{Private L1 Cache}    &  16KB, 4-way associative, LRU, L1 misses are coalesced before accessing L2, 1 cycle latency \\
%        \cmidrule(rl){1-2} 
%\textbf{Shared L2 Cache}   &  768KB total, 16-way associative, LRU, 2 cache banks/2 interconnect ports per memory partition, 10 cycle latency \\
%        \cmidrule(rl){1-2} 
%\textbf{Private L1 TLB}    &  64 entries per core, fully associative, LRU, 1 cycle latency \\
%        \cmidrule(rl){1-2} 
%\textbf{Shared L2 TLB}   &  1024 entries total, 16-way associative, LRU, 2 ports per memory partition (12 ports total), 10 cycle latency \\
%        \cmidrule(rl){1-2} 
%\textbf{DRAM}   & GDDR5 1674 MHz, 6 channels (one channel per memory partition), FR-FCFS scheduler~\cite{fr-fcfs,frfcfs-patent}, 8 banks per rank\\
% & burst length 8\\
%        \cmidrule(rl){1-2} 
%\textbf{Page Table Walker}   & 32 threads shared page table walker, traversing 4-level tree structure similar to previous work~\cite{powers-hpca14}\\
%%        \hline
%        \bottomrule
%    \end{tabular}%
%%  \vspace{-5pt}
%  \caption{Configuration of the simulated system.}
%  \vspace{-5pt}
%%  \vspace{-10pt}
%  \label{table:config}%
%\end{scriptsize}%
%\end{table*}%


==> secs/mask-micro17/secs/related.tex <==
% !TEX root=../mask.tex

\section{Related Work}

\changesI{To our knowledge, this \changesIV{paper} is the first to (1)~provide a thorough
analysis of GPU memory virtualization under \changesII{multi-application} concurrency, and
(2)~redesign the entire GPU memory hierarchy to be aware of \changesII{address translation}
requests. In this section, we discuss previous techniques that \changesV{aim to (1)~provide}~\changesVII{sharing and virtualization mechanisms for GPUs,}~\changesV{(2)~reduce} the overhead of address
translation in \changesVII{GPUs, and (3)~reduce inter-application interference}.}

\subsection{Techniques to Enable GPU Sharing}
%\subsection{Sharing and Memory Management in GPUs}

\para{Spatial Multiplexing and \changesII{Multi-Application} Concurrency.} 
Several works propose techniques to improve GPU utilization
with \changesII{multi-application} concurrency~\cite{mosaic,mafia,asplos-sree,
wang-hpca16,li2014symbiotic,pagoda-ppopp17},
but they do not support memory protection.
%The opportunity to improve utilization 
%with concurrency is well-recognized, but previous 
%proposals~\cite{asplos-sree,wang-hpca16,li2014symbiotic,pagoda-ppopp17}
%do not support memory protection.
\changesI{Jog et al.~\cite{mafia} propose an application-aware GPU memory 
scheduler to improve the performance of concurrently-running GPU applications.}
Adriaens et al.~\cite{gpu-multitasking} 
observe the need for spatial sharing across protection domains,
but do not propose or evaluate a design.
NVIDIA GRID~\cite{grid} and AMD Firepro~\cite{firepro} support static
partitioning of hardware to allow kernels from different VMs
to run concurrently, but the partitions are determined at startup,
which causes fragmentation and underutilization (see \changesI{the \emph{Static} configuration \changesV{evaluated} in} Section~\ref{sec:eval-multi}).
\titleShortMASK{}'s goal is \emph{flexible, dynamic} partitioning. 
NVIDIA's Multi Process Service (MPS)~\cite{mps} allows multiple processes to
launch kernels on the GPU, but the service provides no memory protection or
error containment. 
%Out-of-range reads/writes can happen without triggering errors,
%and exceptions cannot be attributed to the client causing the error. Such
%behaviors are contrary to our fundamental goal of providing isolation. As a
%result, MPS is not suitable for supporting multi-application in a
%multi-tenant cloud setting. 
Xu et al.~\cite{warp-slicer} propose Warped-Slicer,
which is a mechanism for multiple applications to spatially share a GPU core.
Warped-Slicer provides no memory protection, and is not suitable
for supporting multi-application execution. % in a cloud setting.
\changesI{Ausavarungnirun et al.~\cite{mosaic} propose Mosaic, 
\changesII{a mechanism that provides programmer-transparent
support for multiple page sizes in GPUs that provide memory protection for}
% a multi-page-size support for GPUs that provides memory protection for 
multi-application execution. The main goal of Mosaic is to increase 
the effective size of the TLB,
which is orthogonal \changesIV{to \titleShortMASK, and \changesIV{Mosaic} can be combined 
\changesVIII{with \titleShortMASK} to achieve even higher 
performance, as shown in~\cite{rachata-thesis}.}}


%HERE

\para{\changesVII{Time Multiplexing}.}
\changesIV{As discussed in Section~\ref{s:time-multiplex}, \changesVII{time multiplexing}}
% can allow multiple applications to time-share the GPU at
% finer granularity, enabling resource management policies less
% prone to QoS pathologies. Support for it 
is an active research area~\cite{isca-2014-preemptive, gebhart,wang-hpca16}, and 
architectural support~\cite{lindholm,pascal} will likely improve in future GPUs.
\changesIV{These techniques are complementary \changesVII{to} and can be combined with \titleShortMASK}.
%and we leave techniques to combine them for future work.

\para{GPU Virtualization.} 
\changesIV{Techniques to provide GPU virtualization can support concurrent execution of
GPGPU applications~\cite{gdev,gpuvm,gVirt}.} %Most current hypervisor-based full virtualization techniques for GPGPUs 
%must support a virtual device abstraction without the 
\changesIV{However, these GPU virtualization approaches require dedicated hardware support, such as 
\changesV{the} Virtual Desktop Infrastructure (VDI) found in NVIDIA GRID~\cite{grid} and AMD FirePro~\cite{firepro}.
As we discuss in Section~\ref{sec:spatial-multiplex}, 
%Key components missing from these
%proposals include support for the
these techniques do \changesV{\emph{not}} provide \changesV{\emph{dynamic}} partitioning of
hardware resources, and perform worse than \titleShortMASK (see Section~\ref{sec:eval}).}
%efficient techniques for handling over-subscription. 
%Performance overheads incurred by these designs argue strongly for hardware assistance.
%as we propose. By contrast, 
%API-remoting solutions such as 
vmCUDA~\cite{vmCUDA} and rCUDA~\cite{rcuda} provide \changesIV{close-to-ideal} 
performance, \changesIV{but they require significant modifications to 
GPGPU applications and the operating system, which sacrifice transparency to the application,
performance isolation, and compatibility across multiple GPU architectures.}
\changesIV{Vijaykumar et al.~\cite{zorua} propose a framework to virtualize
GPU \changesV{resources for a single application. This technique is \changesVII{complementary} to \titleShortMASK.}}

\para{Demand Paging.}
%In a program running on CPU-GPU systems, performing demand paging can be done
%through the OS on the CPU side. However, this is no longer possible when demand
%paging is done to support concurrent GPU applications. 
%Demand paging is an important primitive for memory virtualization that 
%is challenging for GPUs~\cite{abhishek-ispass16}. 
Recent works on CC-NUMA~\cite{cc-numa-gpu-hpca15}, AMD's hUMA~\cite{huma}, and
NVIDIA's PASCAL architecture~\cite{tianhao-hpca16,pascal}
support demand paging in GPUs. These techniques can be used in conjunction
with \titleShortMASK{}.
% to support paging.


%Lastly, when there is an interrupt or an exception, the GPU will have to be
%able to handle the long latency of the interrupt to resolve. These latency
%generally range in hundred thousand to million cycles. Generally, when these
%interrupt occurs in other systems, an interrupt handler from the Operating
%system will handle the interrupt while the processor perform a context switch
%and run other processes during this event in order to utilize the stalling
%cores. However, in GPU, two major components are missing.  First, preemption
%does not exist and the application current running on the GPU will stall.
%Second, there is no operating system to handle the interrupt. In this work, we
%address both problems by first introducing cross-cores task migration, which
%allows other concurrent applications from other cores to migrate, acting
%similar to a context switch. Second, we introduce [TODO: Continue]


\subsection{TLB Design}

\para{GPU TLB Designs.} Previous works\changesVIII{~\cite{mosaic,cong-hpca17,powers-hpca14,pichai-asplos14,abhishek-ispass16}} \changesV{explore} TLB designs in
heterogeneous systems with
GPUs. %, and the
%adaptation of x86-like TLBs in a heterogeneous CPU-GPU setting~\cite{powers-hpca14}.  
%Key elements in these designs include probing
%the TLB after L1 coalescing to reduce the amount of parallel TLB requests,
%shared concurrent page table walks, and translation caches to reduce main
%memory accesses. 
%\titleShortMASK{} owes much to these designs, but we show
%empirically that contention patterns at the shared L2 layer require additional
%support beyond these designs to accommodate contention from multiple address spaces. 
%Ausavarungnirun et al.~\cite{mosaic} propose a TLB design that supports
%multiple page sizes, which is orthogonal and can be combined with \titleShortMASK
%to achieve higher performance~\cite{rachata-thesis}.
Cong et al.~\cite{cong-hpca17} propose a TLB %support to accommodate cross-context contention. Cong et al. propose a TLB
design for accelerators. This design utilizes the host (CPU) MMU to perform page walks, which
\changesIV{secs/mask-micro17/results in high performance overhead} in the context of multi-application GPUs. Pichai et
al.~\cite{pichai-asplos14} explore a TLB design for heterogeneous CPU-GPU systems,
and add TLB awareness to the existing CCWS GPU warp scheduler~\cite{ccws}.
%which enables parallel TLB accesses on the L1 cache level,
%similar in concept to the Powers design~\cite{powers-hpca14}. 
Warp scheduling is orthogonal to our work, and 
%incorporating a TLB-aware CCWS warp scheduler with \titleShortMASK{} 
can be combined to further improve performance.

%\para{GPU TLB Designs.} Previous works have explored TLB designs in
%heterogeneous systems with
%GPUs~\cite{cong-hpca17,powers-hpca14,abhishek-tlb,abhishek-ispass16}, and the
%adaptation of x86-like TLBs in a heterogeneous CPU-GPU
%setting~\cite{powers-hpca14}.  Key elements in these designs include probing
%the TLB after L1 coalescing to reduce the amount of parallel TLB requests,
%shared concurrent page table walks, and translation caches to reduce main
%memory accesses. \titleShortMASK{} owes much to these designs, but we show
%empirically that contention patterns at the shared L2 layer require additional
%support beyond these designs to accommodate contention from multiple address spaces. Cong et al.\ propose a TLB
%%support to accommodate cross-context contention. Cong et al. propose a TLB
%design similar to our baseline GPU-MMU design~\cite{cong-hpca17}.  However,
%this design utilizes the host (CPU) MMU to perform page walks, which is
%inapplicable in the context of multi-application GPUs. Pichai et
%al.~\cite{abhishek-tlb} explore a TLB design for heterogeneous CPU-GPU systems,
%and add TLB awareness to the existing CCWS GPU warp scheduler~\cite{ccws}.
%%which enables parallel TLB accesses on the L1 cache level,
%%similar in concept to the Powers design~\cite{powers-hpca14}. 
%Warp scheduling is orthogonal to our work, and 
%%incorporating a TLB-aware CCWS warp scheduler with \titleShortMASK{} 
%can be combined to further improve performance.



Vesely et al.~\cite{abhishek-ispass16} analyze support for virtual memory in heterogeneous
systems, finding that the cost of address translation
in GPUs is an order of magnitude higher than \changesIV{that} in CPUs, and that \changesIV{high-latency}
address translations limit the GPU's latency hiding capability and \changesVIII{hurt}
performance. % (an observation in line with our own findings in Section~\ref{sec:tlb-bottleneck}). 
We show additionally that %thrashing due to
\changesIV{inter-address-space} interference further slows down applications sharing the GPU. \titleShortMASK is capable \changesV{of
not only} reducing interference between multiple applications
(Section~\ref{sec:eval-multi}), but \changesIV{also} reducing the TLB miss 
rate \changesV{during} single-application \changesV{execution} as well \changesIV{(as shown in our technical 
report~\cite{mask-tech-report}).}
% We expect that our techniques are applicable to CPU-GPU heterogeneous systems. 


%Instead of relying on hardware modifications, 
\changesIV{Lee et al.~\cite{vast} propose VAST,} \changesVII{a software runtime
that dynamically partitions GPU kernels to manage the memory available to each
kernel.  VAST does not provide any support
for memory protection.  In contrast, \titleShortMASK enables memory virtualization
in hardware, and offers memory protection.}
% a software-managed virtual memory space for GPUs. %They observe that
% %Data-parallel applications typically have a larger working set size compared to
% %the size of GPU memory, preventing these applications from utilizing GPUs.
% %To address this, 
% VAST creates the illusion of a large virtual memory.
% % (without concerns about the physical memory size), by providing an automatic memory
% %management system that partitions GPU programs into chunks that fit the physical
% %memory space. 
% %Even though recent GPUs now support demand paging~\cite{pascal},
% \changesV{Instead of a software-managed virtual memory, \titleShortMASK provides an application-transparent
% virtual memory support.}} \todo{This need to be fixed}
% %\changesVI{\changesV{\cite{vast}'s} observation regarding the large working set \changesV{sizes} of GPGPU programs
% %motivates} the need for better virtual memory support, which is what \titleShortMASK provides.} \todo{rewrite this last sentence.}

\para{TLB Designs in CPU Systems.}  Cox and Bhattacharjee~\cite{cox-asplos16} propose a %an efficient 
TLB design that allows entries corresponding to multiple
page sizes to share the same TLB structure, simplifying the design of
TLBs. %While this design can be applied to GPUs, 
This design \changesI{solves} a different problem \changesVIII(area and energy efficiency),} 
and is orthogonal to \titleShortMASK{}. \changesIV{\changesV{Other} works~\cite{inter-core-tlb, bhattacharjee11hpca, lustig13taco} examine} 
shared last-level TLB designs and page walk cache
designs~\cite{large-reach}, proposing \changesIV{mechanisms} that can accelerate
\changesIV{\emph{multithreaded}} applications by sharing translations between
cores. \changesIV{These} proposals are likely to be less effective for
\changesIV{\emph{multiple}} concurrent GPGPU applications, \changesI{for which} translations 
are \changesIV{\emph{not}} shared between virtual address spaces. Barr et al.~\cite{spectlb} propose
SpecTLB, which speculatively predicts address
translations to avoid the TLB miss latency.  
%Speculatively predicting address translation 
\changesIV{Doing so} can be \changesIV{costly} in GPUs, because
there can be multiple concurrent TLB misses to many different TLB
entries in the GPU.
%This proposal mainly target system with small pages, which generally increases
%the cost of translation upon a TLB miss, which can be common in GPUs.
%\cjr{Smaller than 4k?}

Direct segments~\cite{direct-segment} and redundant memory mappings~\cite{rmm}
reduce address translation overheads by mapping large contiguous virtual memory regions
to a contiguous physical region. These techniques increase
 the reach of each TLB entry, and are
complementary \changesIV{to \titleShortMASK{}.}
%, and may eventually become relevant in GPU settings as well.

%% However, this proposal does not work on GPU workloads as memory
%% allocations in GPU applications are more dynamic. 
%% CJR: the real thing here is that you don't need this stuff on
%% a card that can only address 5-10GB of memory. However, there's no 
%% reason our work can't use these ideas. 


% \pagebreak
\subsection{Techniques to Reduce \changesV{Inter-Application} Interference}


%\para{Token-based Shared Resource Management.} Multiple
%proposals rely on tokens to rate limit access to shared resources such
%as caches, interconnect, and memory. PCAL~\cite{donglihpca15} reduces cache 
%thrashing problem by throttling concurrent cache access using tokens. 
%In PCAL, only threads with tokens are able to fill into the shared cache, 
%and tokens are distributed to threads according to reuse. \titleShortMASK{} extends
%this idea to a GPU context by mediating warp-level rather than thread-level access, 
%and by finding a token distribution policy better suited to the TLB. 
%PCAL's purely reuse-based policy does not work in the TLB of
%the GPU due to the flat distribution of TLB miss rates across warps (see Section~\ref{sec:fill-bypassing}). 
%%%Second, PCAL statically assigns token counts, which works for a shared L2 cache in a single-application
%%scenario, but is ineffective for a shared cache as reuse profiles change with multiple applications. 
%%\cjr{I'm not sure I buy this second reason. However, the first reason is compelling enough. 
%%Heck, just adapting to a warp-based rather than thread-based policy is enough.}
%%applications' characteristics of concurrent applications
%%can changes.

\sloppypar{\para{GPU-Specific Resource Management.}
%Jog et al.~\cite{mafia} propose MAFIA, a main memory management
%scheme that improves performance of concurrently-running GPGPU
%applications. The design of MAFIA assumes that parallel applications
%operate under the same virtual address space, and does not model address
%translation overheads or accommodate {\em safe}, concurrent execution of kernels
%from different protection domains. 
%In contrast, we model and study 
%the impact of address translation and memory protection. 
Lee et al.~\cite{lee2012tap} propose TAP, a TLP-aware cache
management mechanism that modifies the \changesIV{utility-based} cache partitioning
policy~\cite{ucp-yale} and \changesIV{the baseline} cache insertion policy~\cite{rrip} to lower \changesIV{cache space \changesV{interference} between 
GPGPU and CPU applications}.  \changesVIII{TAP} does not consider address translation traffic.}

%However, TAP does not consider address translation and interference
%between different GPGPU applications.

\changesV{Various} memory scheduler designs target systems with
\changesVI{GPUs~\cite{complexity,chatterjee-sc14,sms,jeong-cpu-gpu,usui-squash,usui-dash,adwait-critical-memsched}.} Unlike
\titleShortMASK{}, these designs focus on a single GPGPU application, and are not
aware of \changesIV{address translation requests}. 
%page walk traffic. They focus on reducing the complexity of the memory
%scheduler for a single application~\cite{complexity}, reducing
%inter-warp interference~\cite{chatterjee-sc14}, or managing heterogeneous CPU-GPU
%applications~\cite{sms,jeong-cpu-gpu,usui-squash,usui-dash}. 
While some of these works propose
mechanisms that reduce \changesIV{inter-application} interference~\cite{sms,jeong-cpu-gpu,usui-squash,usui-dash}, they 
differ from \titleShortMASK because \changesV{they (1)~consider interference bewteen CPU applications and 
GPU applications, and (2)~are \emph{not} aware of address translation requests.}
%do not consider interference between page-walk-related
%and normal memory traffic. 


%Resource management in heterogeneous CPU-GPU systems has enjoyed considerable
%research attention. Lee et al. propose TAP~\cite{lee2012tap}, a TLP-aware cache
%management mechanism that modifies existing CPU cache partitioning
%policy~\cite{ucp-yale} and cache insertion policy~\cite{rrip} to lower GPGPU
%applications' interference with CPU applications on the shared cache.
%Ausavarungnirun et al. propose SMS~\cite{sms}, which is a low complexity memory
%controller design that reduces interference of Graphics applications with CPU
%applications at the main memory. Jeong et al. propose a QoS-aware memory
%scheduling policy that improves QoS of Graphics and CPU applications in
%heterogeneous systems~\cite{jeong-cpu-gpu}. Usui et al. propose SQUASH, a
%QoS-aware memory scheduler for heterogeneous systems~\cite{squash}. While these
%works propose mechanisms to reduce interference, they are different than
%\titleShortMASK because 1) they consider interference from applications with wildly
%different characteristics (CPU applications vs. GPU applications) and 2) do
%not consider interference between page-walk-related data and normal data. 

%HERE


\para{Cache Bypassing Policies in GPUs.} \changesVIII{There are
many techniques (e.g., \cite{medic,donglihpca15,li-ics15,xie-hpca15,chen-micro47,chen-mes14,xie-iccad13,mrpb})} to reduce
contention \changesV{in} shared GPU
caches.
% employ
%memory-divergence-based bypassing~\cite{medic}, reuse-based cache
%bypassing~\cite{donglihpca15,li-ics15,xie-hpca15,chen-micro47,chen-mes14}, and software-based
%cache bypassing~\cite{xie-iccad13}, and sometimes combine these works
%with throttling~\cite{chen-micro47,chen-mes14,mrpb} to reduce contention. 
\changesIV{Unlike \titleShortMASK, these works do \emph{not} differentiate address translation requests
from data demand requests,} and focus on \changesI{only 
\changesV{single-application} execution}. 
%These techniques are orthogonal to \titleShortMASK{}.

%Lee et al. proposes TAP, a TLP-aware cache management scheme that improves
%two CPU-based cache management scheme, TAP-UCP and TAP-RRIP for CPU-GPU heterogeneous
%systems. First, TAP-UCP modified utility based cache partitioning~\cite{ucp}
%by limiting the number of ways in the L2 cache GPGPU application can utilize
%based on the benefit of L2 cache to the GPGPU application. Second, TAP-RRIP
%proposes a modification to Re-Reference Interval Prediction~\cite{rrip} by
%limiting interference when GPGPU application do not need extra cache space.

\para{Cache and TLB Insertion Policies.} Cache insertion policies that 
account for cache thrashing~\cite{dip,rrip,bip}, future reuse~\cite{eaf-vivek,seshadri-taco2015}, \changesIV{or
inter-application interference~\cite{wu11ispass}} work well for CPU
applications, but \changesIV{previous works} have shown \changesI{that}~\changesIV{some of} these 
policies \changesV{can be} ineffective for GPU applications~\cite{lee2012tap,medic}. 
This observation holds for the shared L2 TLB in \changesIV{multi-address space execution.}
%\changesIV{Wu and Martonosi~\cite{wu11ispass} propose an insertion policy} that 
%mitigate interference from \changesIV{address translation requests~\cite{wu11ispass}} for CPUs
%are even more critical for GPUs, because outstanding TLB misses can 
%significantly limit parallelism by stalling a large number of threads.


% considered by \titleShortMASK{} as well.



%\adwait{this subsection seems incomplete..}

%%This work is
%%complementary to our work and leave extension of \titleShortMASK{} to support
%%it as future work. 
%% and can be combined to realize the full potential of
%% virtual address supports in systems with GPUs.
%%However, it is possible to further realize
%%additional potential of concurrent GPU applications if the paging becomes more
%%efficient.~\cjr{What do you mean by this? How?} 







==> secs/medic/section/abstract.tex <==
% !TeX root = ../paper.tex

\begin{abstract}

%Graphics Processing Units (GPUs) have enormous parallel processing power that
%can leverage thread-level parallelism. Traditionally, GPUs have been used to
%run graphics applications as they naturally exhibit high amounts of
%concurrency. In recent years, with programming languages such as CUDA and
%OpenCL, programmers have also been able to parallelize non-graphics,
%general-purpose (GPGPU) applications into thousands of threads to harness the
%power of GPUs.

In a GPU, all threads within a warp execute the same instruction in lockstep.
For a memory instruction, this can lead to \emph{memory divergence}: the memory
requests for some threads are serviced early, while the remaining requests
incur long latencies.  This divergence stalls the warp, as it cannot
execute the next instruction until \emph{all} requests from the current 
instruction complete.

In this work, we make three new observations.  First, GPGPU warps exhibit
heterogeneous memory divergence behavior at the shared cache: some warps have
most of their requests hit in the cache (high cache utility), while other warps
see most of their request miss (low cache utility).  Second, a warp retains the same divergence
behavior for long periods of execution.  Third, due to high memory level
parallelism, requests going to the shared cache can incur queuing delays as 
large as hundreds of cycles, exacerbating the effects of memory divergence.

We propose a set of techniques, collectively called \emph{\titleLongMeDiC{}}
(\titleShortMeDiC{}), that reduce the negative performance impact of memory divergence and cache queuing.
\titleShortMeDiC{} uses warp divergence characterization to guide three components:
(1)~a cache bypassing mechanism that exploits the latency tolerance of low cache
utility warps to both alleviate queuing delay and increase the hit rate for high
cache utility warps, (2)~a cache insertion policy that prevents data from high
cache utility warps from being prematurely evicted, and (3)~a memory controller
that prioritizes the few requests received from high cache utility warps to
minimize stall time.  We compare \titleShortMeDiC{} to four cache management 
techniques, and find that it delivers an average speedup of 21.8\%, and 20.1\%
higher energy efficiency, over a state-of-the-art GPU cache management
mechanism across 15 different GPGPU applications.
% We find that \titleShortMeDiC{} delivers an average speedup of
% 21.8\%, and 20.1\% higher energy efficiency, over \yellow{a state-of-the-art} GPU cache
% management mechanism across 15 different GPGPU applications.

% Warps from a GPGPU application can experience \emph{memory divergence:} 
% some of the requests generated by a single memory
% instruction can be serviced quickly, while the remaining requests incur long latencies.
% Memory divergence increases execution latency as the warp can continue executing
% only after all memory requests from an instruction completes.
% 
% In this work, we make three new key observations. First, we identify
% that GPGPU warps exhibit heterogeneity in their memory divergence behavior at
% the shared cache: some warps achieve high cache utility (i.e., most requests
% are hits) while others have low cache utility.
% % Some of these warps experience the full benefit of shared caching due
% % to their access patterns, while other warps have poor shared cache utility and
% % can even induce cache thrashing. This inter-warp heterogeneity results in
% % greatly varying latency tolerance across the warps.
% Second, a warp retains similar, predictable divergence behavior for long periods of execution.
% Third, shared cache requests can incur significant queuing delays (as large as 
% hundreds of cycles), as the high degree of memory level parallelism 
% allows applications to issue large amounts of L2 cache requests within a small number
% of cycles, exacerbating the effects of memory divergence.
% 
% To reduce the negative performance impact of memory divergence and cache queuing, we propose
% a set of techniques, collectively called
% \titleLongMeDiC{} (\titleShortMeDiC{}).  The key idea of \titleShortMeDiC{} is to identify
% and take advantage of the predictable warp memory divergence behavior
% to reduce application latency.  \titleShortMeDiC{} uses
% warp divergence characterization to guide three components:
% % The key idea of \titleShortMeDiC is to identify and take
% % advantage of the predictable warp memory characteristics to optimize cache
% % management and memory scheduling. \titleShortMeDiC consists of three components: 
% (1)~a cache bypassing mechanism that exploits the latency tolerance of warps with
% low cache utility to alleviate the queuing delay and increase the hit rate for warps
% with high cache utility,
% (2)~a cache insertion policy that prevents the cache
% blocks of warps with high cache utility from being prematurely evicted, and
% (3)~a memory controller that prioritizes requests from warps with high cache utility
% to minimize warp stall time due to occasional cache misses.  Our evaluation shows that \titleShortMeDiC{} provides a 21.8\%
% performance improvement and 20.1\% higher energy efficiency, on average across
% 15 different GPGPU applications, compared to the best previous state-of-the-art GPU cache
% management mechanism.




% Warps from a GPGPU application can experience \emph{memory divergence}, where 
% during a single load instruction, some of the requests from the warp are serviced
% quickly by the caches, while other requests incur long lookup latencies and may
% need to be retrieved from DRAM.  In this work, we focus on the causes of memory
% divergence that exist within the GPU \emph{memory partition} (i.e., the shared
% last-level cache and DRAM).  First, we identify that GPGPU warps exhibit
% heterogeneity in shared cache utilization --- some warps have most of their
% memory requests hit in the shared cache (\emph{mostly-hit warps}), while other
% warps see most memory requests become shared cache misses (\emph{mostly-miss
% warps}).  As we observe, a mostly-hit warp continues to be a mostly-hit warp
% throughout its lifetime, and a mostly-miss warp continues to be mostly-miss for
% its lifetime.

% In this work, we make two new key observations. First, we identify that queuing
% latency in the GPU's L2 cache is a significant source of the long memory
% latency in GPUs.  L2 cache accesses can take as many as several hundreds of
% cycles, due to the large amounts of memory level parallelism in GPUs and the
% limited number of read/write ports and L2 cache banks. Second, unlike graphics
% applications, warps in GPGPU applications utilize the shared cache differently
% and therefore have different latency tolerance. While cache accesses from some
% warps fully benefit from using the cache and generate many cache hits, accesses
% from other warps are not able to take advantage of the cache and can cause
% cache thrashing. This causes heterogeneity in latency tolerance between
% different warps within a GPGPU application.



\end{abstract}


==> secs/medic/section/qual-eval.tex <==
\section{Qualitative Evaluation}

\subsection{Bypassing Policies in both CPU and GPU systems}

\subsection{Caching Policies in CPU-based Systems}

Several works has been proposed to improve the cache utilization of a
multi-core CPU system~\cite{rrip,eaf-vivek}. These works are designed to
take advantage of cache utilization of each CPU thread. However, as we will
show in detail in Section~\ref{sec:reuse}, these previously proposed CPU-cache
management schemes are not aware of the heterogeneous characteristic of
different warps and fail to identify highly reused warps. In this work, we
propose a GPU-specific parallelism- and warp-aware policy that addresses these
drawbacks.



==> secs/medic/section/related.tex <==
% !TeX root = ../paper.tex

\subsection{Related Work}
\label{sec:related}
%There are several previous works that propose cache
%bypassing as their key mechanism. In this subsubsection, we will discuss and
%compare \titleShortMeDiC{} with these proposals. 

To our knowledge, this is the first work that identifies inter-warp memory divergence
heterogeneity and exploits it to achieve better system performance in GPGPU
applications. Our new mechanism consists of warp-type-aware components for
cache bypassing, cache insertion, and memory scheduling. We have already
provided extensive quantitative and qualitative comparisons to state-of-the-art
mechanisms in GPU cache bypassing~\cite{donglihpca15}, cache
insertion~\cite{eaf-vivek}, and memory scheduling~\cite{fr-fcfs,frfcfs-patent}. In
this section, we discuss other related work in these areas.

\vspace{5pt}
\noindent\textbf{Hardware-based Cache Bypassing.} \green{PCAL is a bypassing mechanism that
addresses the cache thrashing problem by throttling the
number of threads that time-share the cache at any given time~\cite{donglihpca15} (see Section~\ref{sec:methodology}). The key idea of
PCAL is to limit the number of threads that get to access the cache. 
%While this work and PCAL share the same goal of reduce cache thrashing, we directly
%address the bigger problem of increasing the utilization of shared resources of
%different warps. Additionally, this work also provides a mechanism that
%differentiates how each warp utilizes its shared resources and provide a
%prioritization scheme at various places, not only in the cache, to minimize the
%amount of time warps are stalled due to long latency memory instructions.
Concurrent work by Li et al.~\cite{li-ics15} proposes a cache bypassing
mechanism that allows only threads with high reuse to utilize the cache. The
key idea is to use locality filtering based on the reuse characteristics of GPGPU
applications, with only high reuse threads having access to the cache.
Xie et al.~\cite{xie-hpca15} propose a bypassing mechanism at the
thread block level. In their mechanism, the compiler statically marks whether thread blocks prefer caching or bypassing. 
At runtime, the mechanism dynamically selects a subset of thread blocks to use
the cache, to increase cache utilization.

Chen et al.~\cite{chen-micro47,chen-mes14} propose a combined warp throttling and
bypassing mechanism for the L1 cache based on the cache-conscious warp
scheduler~\cite{ccws}. The key idea is to bypass the cache when resource
contention is detected. This is done by embedding history information into the
L2 tag arrays. The L1 cache uses this information to perform bypassing
decisions, and only warps with high reuse are allowed to access the L1 cache. 
Jia et al. propose an L1 bypassing mechanism~\cite{mrpb}, whose
key idea is to bypass requests when there is an associativity stall.
%As we have shown in Section~\ref{sec:eval}, our mechanism is not only able to identify highly reused
%blocks implicitly, but our mechanism can also differentiate between warps with high reuse that
%are likely to benefit from the cache and warps with high reuse that are unable to benefit from
%the cache.} 

\titleShortMeDiC{} differs from these prior cache bypassing works because it
uses warp memory divergence heterogeneity for bypassing decisions. We also show
in Section~\ref{sec:eval} that our mechanism implicitly takes reuse information 
into account.}
%and that it correctly applies bypassing decisions
%appropriately based on warp type.
%the reuse based mechanism can be hard to
%implement at the shared L2 cache; 
%however, we use the Bloom filter based
%mechanism proposed for the Evicted Address Filter cache~\cite{eaf-vivek} to
%simplify the process of tracking reuse information.

\vspace{5pt}
\noindent\textbf{Software-based Cache Bypassing.} \green{Concurrent work by Li et
al.~\cite{li-sc15} proposes a compiler-based technique that performs cache
bypassing using a method similar to PCAL~\cite{donglihpca15}. Xie et
al.~\cite{xie-iccad13} propose a mechanism that allows the compiler to perform
cache bypassing for global load instructions. Both of these mechanisms are different from
\titleShortMeDiC{} in that \titleShortMeDiC{} applies bypassing to \emph{all} loads and stores that
utilize the shared cache, without requiring additional characterization at the
compiler level.} Mekkat et al.~\cite{mekkat-pact13} propose a bypassing mechanism for when
a CPU and a GPU share the last level cache. Their key idea is to
bypass GPU cache accesses when CPU applications are cache sensitive, which is
not applicable to GPU-only execution.

\vspace{5pt}
\noindent\textbf{CPU Cache Bypassing.} In addition to GPU cache bypassing, there is prior work that proposes cache
bypassing as a method of improving system performance for
CPUs~\cite{tyson-micro28,doung-micro45,gaur-isca11,piquet-acsac07,teresa-micro97,teresa-isca97}. 
As they do not operate on SIMD systems, these mechanisms do not (need to)
account for memory divergence heterogeneity when performing bypassing decisions.
%These mechanisms are only applicable to their
%targeted systems, and cannot be ported for GPGPU applications. 

\vspace{5pt}
\noindent\textbf{Cache Insertion and Replacement Policies.} Many works have
proposed different insertion policies for CPU
 systems (e.g.,~\cite{bip,eaf-vivek,dip,rrip}).  We compare our insertion policy against
the Evicted-Address Filter (EAF)~\cite{eaf-vivek} in Section~\ref{sec:eval}, and show
that our policy, which takes advantage of inter-warp divergence
heterogeneity, outperforms EAF. Dynamic Insertion Policy
(DIP)~\cite{dip} and Dynamic Re-Reference Interval Prediction
(DRRIP)~\cite{rrip} are insertion policies that account for cache
thrashing. The downside of these two policies is that they are unable to
distinguish between high-reuse and low-reuse blocks in the same
thread~\cite{eaf-vivek}. The Bi-modal Insertion Policy~\cite{bip}
dynamically characterizes the cache blocks being inserted. None of
these works take warp type 
characteristics or memory divergence behavior into account.
%our insertion mechanism will also impact the
%replacement policy, and that we track cache block characteristics at a warp-level
%granularity. 
%The replacement policy in \titleShortMeDiC{} also replaces blocks based
%on the hit ratio (where the mosly-miss category will be the prime candidate for
%replacement). 
%All these previously proposed policies does not take into
%account of the inter-warp heterogeneity in GPGPU applications.

\vspace{5pt}
\noindent\textbf{Memory Scheduling.} There are several memory scheduler designs that
target systems with CPUs~\cite{fr-fcfs,parbs,stfm,atlas,tcm,bliss,bliss-arxiv,mise},
GPUs~\cite{complexity,chatterjee-sc14}, and heterogeneous
compute elements~\cite{sms,jeong2012qos,squash}.  Memory schedulers for CPUs 
and heterogeneous systems generally aim
to reduce interference across different applications~\cite{fr-fcfs,parbs,stfm,atlas,tcm,bliss,bliss-arxiv,sms,squash,mise}.

\vspace{-4pt}
Chatterjee et al. propose a GPU memory
scheduler that allows requests from the same warp to be grouped
together, in order to reduce the memory divergence across different memory
requests within the same warp~\cite{chatterjee-sc14}. Our memory scheduling
mechanism is orthogonal, because we aim to reduce the interference
that mostly-hit warps, which are sensitive to high memory latency, 
experience due to mostly-miss warps.  It is possible to combine these two
scheduling algorithms, by batching requests (the key mechanism
from Chatterjee et al.~\cite{chatterjee-sc14}) for both the high and low priority queues (the
key mechanism of our memory scheduler). 
% and as shown
%by Ausavarungnirun et al., these CPU schedulers are not applicable to GPU
%applications~\cite{sms}. Additionally, the design in Ausavarungnirun et
%al.~\cite{sms} is not applicable to GPU-only applications because the scheduler
%will fall back to FR-FCFS~\cite{fr-fcfs} when running on GPU-only applications.

%\noindent\textbf{Thread Throttling:} \yellow{Previous works propose thread
%throttling as another alternative solution to cache thrashing
%problem~\cite{ccws, ccws-swl,nmnl-pact13,cpugpu-micro,kuo-throttling14}.
%Combining \titleShortMeDiC with such throttling mechanisms is an interesting
%direction for future work.}

\vspace{5pt}
\noindent\textbf{Other Ways to Handle Memory Divergence.} \green{In addition to cache
bypassing, cache insertion policy, and memory scheduling, other works have
proposed different methods of decreasing memory
divergence~\cite{ccws,nmnl-pact13,cpugpu-micro,kuo-throttling14,largewarps,warpsub,zheng-cal,caws-pact14,tor-micro13}.
These methods range from thread throttling~\cite{ccws,nmnl-pact13,cpugpu-micro,kuo-throttling14} to warp
scheduling~\cite{ccws,largewarps,warpsub,zheng-cal,caws-pact14,tor-micro13}.
While these methods share our goal of reducing memory divergence, none of them
exploit inter-warp heterogeneity and, as a result, are orthogonal or
complementary to our proposal.  Our work also makes new observations about 
memory divergence not covered by these works.}
% While these methods share our goal of reducing memory divergence, their
% solutions are orthogonal or complementary to our proposal and thus can be combined with our techniques.
% \yellow{Furthermore, we contribute new observations about memory divergence not
% covered by these works.}}






==> secs/mosaic/secs/abstract.tex <==
% !TEX root=../paper.tex


\begin{abstract}




Contemporary discrete GPUs support rich memory management features
such as virtual memory and demand paging. 
These features simplify GPU programming by providing
a virtual address space abstraction similar to CPUs and eliminating
manual memory management, 
but they introduce high performance \changesI{overheads} during
(1)~address translation and (2)~page faults.
A GPU relies on high degrees of \emph{thread-level parallelism} (TLP) to hide 
memory latency.
Address translation can undermine TLP, as a single miss in the translation
lookaside buffer (TLB) invokes an expensive serialized page table walk that 
often stalls \emph{multiple} threads.  
% Due to the limited TLB capacity,
% these TLB misses occur more frequently as application data sets grow, and as
% multiple applications interfere with each other.
\changesI{Demand paging} can also undermine TLP, as \changesI{multiple threads often stall while they wait for an}
expensive data transfer over the \changesI{system I/O (e.g., PCIe) bus} when the GPU demands a page.
%over the PCIe bus when the GPU demands a page.

% Unfortunately, the features introduce high
% overheads for (1)~address translation and (2)~page faults (which require 
% expensive data transfers over PCIe), which can cripple GPU performance.}
% % These features dramatically
% % simplify GPU programming by providing a familiar virtual address space
% % abstraction, and eliminating manual memory management, but they come at the
% % cost of additional overheads for address translation and
% % page-fault-driven PCIe transfers. The overheads can be crippling.

In \changesI{modern} GPUs, \changesI{we face} a trade-off \changesI{on how
the page size used for memory management affects address translation and demand paging.}
% \changesI{when we try to reduce} these two overheads.
\changesI{The address translation overhead is lower when we employ a \emph{larger} page size}
(e.g., 2MB \emph{large pages}, compared with
conventional 4KB \changesI{\emph{base pages}}), which \changesI{increases} TLB coverage and thus \changesIII{reduces}
TLB misses.
Conversely, \changesI{the} demand paging \changesI{overhead is lower when we
employ a \emph{smaller} page size}, which \changesI{\changesI{decreases} the \changesIII{system I/O bus} transfer latency}.
%and improve page prefetching.
% is dominated by transfer latencies,
% which are best mitigated by overlapping transfer with kernel execution,
% and by predictive prefetching; both strategies are better served
% by smaller page sizes.
% %GPU kernel threads, and avoided where possible using techniques
% %such as predictive prefetch. Larger pages magnify load-to-use
% %intervals with longer PCIe transfers, increasing the average number
% %of threads stalled by a given fault. Demand-paging for discrete
% %GPUs is best served by smaller pages; indeed previous work has
% %dismissed huge pages as a viable alternative for these reasons.
%We find that GPGPU applications present an opportunity to exploit this trade-off, 
\changesI{Support for \emph{multiple page sizes} can help relax the page size
trade-off so that address translation and demand paging optimizations work
together synergistically.  However, existing \changesIII{page} \emph{coalescing}
(i.e., merging base pages into \changesIIIII{a large page}) and \emph{splintering} (i.e., splitting a
large page into base pages) policies require costly base page migrations that
\changesIII{undermine the benefits multiple} page sizes provide.}
\changesI{In this paper, we observe} that GPGPU applications present an opportunity 
% \changesI{for address
% translation and demand paging optimizations to} work together \changesI{synergistically}, 
\changesI{to support multiple page sizes without costly data migration,}
as \changesI{the applications} perform most of their memory allocation \changesI{\emph{en masse}
(i.e., \changesI{they allocate a large number of base pages at once})}.
% \changesI{We show that} with \changesI{intelligent} memory allocation strategies, 
\changesI{We show that this \emph{en masse} allocation allows us to
create intelligent memory allocation policies which ensure that base pages that are contiguous
in virtual memory are allocated to contiguous physical memory pages.
As a result, coalescing and splintering operations no longer
need to migrate base pages.}
% \changesI{a memory manager
% can effectively} coalesce multiple base pages into a single large page without the need
% to \changesI{perform costly data migration} most of the time.

We introduce \titleShort, a GPU \changesI{memory manager} that
provides \emph{application-transparent} \changesI{support for multiple page sizes}.
\titleShort uses base pages to transfer data over \changesI{the system I/O bus}, and allocates physical
% \titleShort transfers data over I/O bus using small page granularity, and allocates physical
memory in a way that \changesI{(1)~}preserves \changesI{base page contiguity} 
and \changesI{(2)~}ensures that a 
large page \changesIIII{frame} contains \changesI{pages from only} a single memory protection domain.
\changesI{We take advantage of this allocation strategy to design
\changesI{a novel in-place page \changesIII{size selection mechanism} that avoids data migration.}
%\changesI{a novel in-place page \changesIII{size selection mechanism} that avoids data migration.}
%  novel \emph{coalescing} 
% (i.e., merging base pages into a large page) and \emph{splintering} (i.e. splitting a
% large page into base pages) primitives that can be implemented as low-latency
% atomic operations. 
\changesI{This \changesIII{mechanism} allows} the TLB to use large \changesI{pages,} 
reducing address translation overhead.
% while splintering operations allow 
\changesIII{During data transfer, this mechanism enables the GPU}
to transfer \changesI{\emph{only}} the base pages that are needed by the application over the
system I/O bus, \changesI{keeping demand paging overhead low}.}
% significantly increase the TLB
% reach through synchronization-free page coalescing and splintering primitives.
% \changesI{the apparent tension between address translation overheads 
% and demand paging performance by providing \emph{transparent}} huge page
% support for discrete GPUs. \changesI{\titleShort transparently and dynamically
% changes virtual memory mappings during workload execution, by using small 4KB
% pages to perform demand paging when transferring data over PCIe, while
% employing fast address translation based on 2MB large pages to significantly
% reduce the TLB miss rate.}
% % supports fast
% % address translation based on huge pages, with the demand
% % performance enabled by small pages, transparently and dynamically
% % changing virtual memory mappings in response to workloads.
% \titleShort tracks spatial and temporal reference locality
% to inform \changesI{a \emph{contiguity-preserving}} memory management policy,
% which reduces the need for compaction-induced memory 
% to create contiguity.
% \titleShort uses two novel mechanisms, \allocatorName and \policyName, to 
% implement synchronization-free coalesce and splinter primitives
% with the performance cost of a single atomic pointer swap.
Our evaluations show that \titleShort reduces address translation
overheads \changesI{while efficiently achieving the benefits of demand paging},
% near-negligible address translation overheads
% with minimal impact on demand paging performance, 
compared to a contemporary GPU that uses only a 4KB page size.
Relative to \changesI{a} state-of-the-art GPU \changesI{memory manager}, 
\titleShort improves the performance \changesI{of homogeneous and 
heterogeneous multi-application workloads by 55.5\% and 29.7\% on average, 
respectively, coming within 6.8\% and 15.4\% of the performance 
\changesI{of an ideal TLB where all TLB requests are hits}.}
% limiting the performance overhead of address translation to within 5.7\% of an ideal,
% %by 46.7\% on average, bringing address translation costs to within 5.7\% of an ideal,
% infinite TLB.}

%~\cjr{save the homo-hetero business for later. Too confusing here, and
%the 30 percent just waters down the headline anyway.}
%for homogeneous workloads, and by 30.1\% for heterogeneous workloads. \sg{homogeneous/heterogeneous undefined}
%\titleShort  \sg{what is ideal?} for homogeneous 
%workloads, and 14.5\% for heterogeneous workloads, on average.


%  Wide-spread recognition of the need for better GPU virtualization support 
%  has underscored a flurry of recent research interest in memory management
%  features such as TLB-based memory protection and demand paging. 
%  The improved programmability enabled by these features comes at 
%  a cost: address translation and paging put synchronous, high-latency 
%  TLB-misses on the critical path, which can limit parallelism.
%  Uslargelarger pages could help reclaim performance lost to address translation 
%  by increasing TLB reach, but larger pages harm demand paging performance
%  through increased transfer latency and reduced flexibility of the runtime
%  to prefetch or overlap transfer latency with kernel execution.
%  
%  This paper explores the design space for transparent huge page support
%  for GPUs to sidestep the tradeoff between TLB reach and demand paging latency. 
%  We focus on discrete GPUs, whose superior compute density continues to make them
%  the platform of choice in a wide array of settings.
%  We extend the TLB-based design, used in previous work on address translation 
%  and demand paging, to support multiple page sizes. We also explore 
%  designs whose strategy is to back frequently accessed data on the
%  device with contiguous 2MB ``huge'' pages, back infrequently
%  accessed or demand paged data with 4KB ``base'' pages, and transparently
%  move data and changing memory mappings as access profiles change. 
%
%  Our design, \oursystem, tracks temporal 
%  and spatial locality to inform policies for transparent coalescing 
%  of frequently accessed base pages and transparent splintering of huge pages 
%  to reduce fragmentation, increase contiguity, or reduce page 
%  far-fault latencies. \oursystem relies on techniques to preserve 
%  contiguity, allowing it to minimize synchronization and memory copy 
%  in the common case. \oursystem uses RowClone's bulk memory transfer
%  to minimize overheads when copying is required. A novel mechanism called 
%  \remapcache allows application-level updates to virtual pages 
%  to proceed concurrently with coalescing or splintering, 
%  preserving atomicity for page table updates.
%  Evaluation of a \oursystem prototype shows that using huge pages 
%  lowers address translation overhead significantly without harming
%  demand paging performance. \oursystem improves performance over 
%  TLB designs in the literature by X\% and 
%  over demand paging on base or huge pages 
%  alone by Y\%.\cjr{numbers please, when appropriate.}
%
\end{abstract}


==> secs/mosaic/secs/ack.tex <==
\section*{Acknowledgments}

We thank the anonymous reviewers and SAFARI group members for their feedback.
Special thanks to \changesIIIIIII{Nastaran Hajinazar, Juan G\'{o}mez Luna, and Mohammad Sadr for their feedback.}
We acknowledge the support of our industrial partners, \changesIII{especially Google, Intel,
Microsoft, NVIDIA, Samsung, and VMware. This research was
partially supported by the NSF (grants 1409723 and 1618563),}
%(grants 0953246, 1065112, 1147397, 1205618, 1212962,
%1213052, 1302225, 1302557, 1317560, 1320478, 1320531, 1409095, 1409723,
%1423172, 1439021, 1439057, and 1618563), 
the Intel Science and Technology Center for
Cloud Computing, and the Semiconductor Research Corporation.



==> secs/mosaic/secs/design.tex <==
\section{Mosaic}
\label{sec:mechanism-mosaic}

This section describes the design of \titleShortMOSAIC. 
%a mechanism whose key goal
% is to provide a very high performance, high throughput
%and transparent multi-page-size support for GPUs.  
We first enumerate design constraints and the 
basic primitives required, such as coalescing, splintering, and compacting pages,
and subsequently integrate them to form a complete design.

%Transparent large page support requires primitives 
%First, 
%provide all of the design constants and primitives \sg{for what?} of \titleShortMOSAIC} in
%Section~\ref{sec:mosaic-primitive}.  Then, we describe the design of
%\titleShortMOSAIC} in Section~\ref{sec:mosaic-mech}.
%\rachata{We might want to move this part up a Section so that motivation follows directly into the description of MOSAIC.}


\subsection{Design Constraints}
\label{sec:mosaic-primitive}

\paragraphbe{Primitives.}
%\label{sec:design-primitives}
Modulating page sizes backing an application's virtual address space requires 
mechanisms for coalescing and splintering. \emph{Coalescing}
involves collecting a set of 4KB base pages into a single contiguous 2MB page in 
physical memory. This process can involve 1) moving memory
between base pages and large pages and 2) moving and compacting data to create
the required contiguity in the physical address space.
\jl{Not entirely sure what this sentence was trying to say. Did you mean: from/to base/large pages?}
\emph{Splintering}, 
the reverse operation, breaks a single 2MB page into a series of 512 
contiguous 4KB base pages. While splintering
need not involve copy, it is seldom performed without being paired with a
subsequent operation that performs a copy (e.g., compaction, copy-on-write, or data
transfer across PCIe, etc.). Both operations
require updates to page table mappings which must appear atomic to the application.  
In CPU-based large page management,
these operations are performed by the operating system, which can either commandeer an
application's execution context or use background threads to do it.
The atomicity of these operations is achieved using a combination of locking and
inter-processor interrupts (IPIs).

On top of this, our design must contend with limited support for
synchronization along with the GPU's high levels of concurrency. In particular,
memory accesses to virtual pages whose mappings are being updated must \emph{stall}
until the update completes, and stale TLB entries must be flushed. As GPUs are 
incapable of leveraging background threads to perform operations such as compaction,
it argues for a design that proactively minimizes the need to be handled through
background threads. 

\paragraphbe{Concurrency.} Ability to support cross-address-space protection is
a major motivator for implementing address translation, a design that handles
concurrent address translation well is critical.  Depending on allocation
policy, 2MB extents of physical memory may contain 4KB pages from different
address spaces (from different GPGPU applications).  This can force memory copy
to create contiguity under fragmented conditions. Alternatively, a design that
never shares 4KB pages in a 2MB physical extent across protection domains (i.e., all
4KB pages within the 2MB range have the same address space identifier) can
sidestep the need for copying at the cost of increased susceptibility to
fragmentation. \titleShortMOSAIC{}'s design reflects an imperative to allocate
physical memory across applications to proactively conserve contiguity, avoid
copying during coalescing and splintering. While previously-proposed DRAM
techniques that accelerate copy with bulk
primitives~\cite{seshadri2013rowclone, lisa} are available, copying data across
DRAM banks incurs a significant performance impact and should be avoided.


\paragraphbe{Correctness.} 
Atomicity of updates to memory mapping or changes to the physical layout
backing a virtual address space must be preserved from the perspective of the
application. \titleShortMOSAIC{}'s design prohibits memory accesses by
application threads that may use a stale or partially updated address
translation through a combination of TLB shootdowns and blocking all
translation requests at the TLB. Both techniques are costly for performance, so
strategies for minimizing their usage and overhead per operation are necessary.

%\sloppypar{In summary, \titleShortMOSAIC} must be designed to provide transparency, concurrency, and
%correctness.}



%Given a set of primitives with which to implement transparent large page support
%(splintering and coalescing), a design must further exercise them minimally
%according to some policy that preserves performance. To realize the high-level
%design goal described above, \titleShortMOSAIC}{} will:
%
%\begin{compactitem}
%\item Proactively coalesce base pages into large pages when 
%	API-driven transfers of 2MB or more target  
%	virtual address regions already backed by base pages 
%	that map contiguous 2MB-aligned physical regions.  
%\item Coalesce base pages into a large page when spatial and temporal 
%	access frequency indicate that a large page mapping 
%	would be well-utilized, and would not interfere with 
%	demand paging or cause fragmentation. 
%\item Splinter large pages into base pages when they are not 
%	well-utilized, are internally fragmented, 
%	or touched by the demand paging subsystem.
%\end{compactitem}

%Hardware must support some mechanisms for tracking access frequency, while
%fragmentation metrics must be provided by software. 
\subsection{Design of \titleShortMOSAIC} 
\label{sec:mosaic-mech}

\sloppypar{\titleShortMOSAIC{} consists of three components: \allocatorNameLong (\allocatorName),
\policyName, and \compactionNameLong (\compactionName), which work in concert to provide
transparent large page support with minimal common case overhead.}

\cjr{we need to either stick to coalesce or promote, or say somewhere 
that we use them interchangably. I think picking one is best. }

The memory allocator plays an important role in conserving contiguity as well
as eliminating data copies for coalescing. When coalescing a page, data copy 
is necessary only when the underlying contiguity in the physical address space 
is not already present (e.g. because pages must be copied into the physical 
region and any other currently active pages must be moved out of the way). 
%transfer data around if and only if there are pages from \emph{other context}
%that lies within the range of the large page (we define this as a large page
%range) 
Figure~\ref{fig:coalescing-example} shows an example in which there
are three pages under the physical large page range that are mapped from Process~2 while the
remaining pages in the large page range are backing pages in Process~1. To create contiguity 
to enable a large page mapping, 
Process~2's pages need to be \emph{moved, remapped, and replaced} by pages from Process~1,
causing six page-size data movements as well as remapping overhead. To avoid such overheads, \titleShortMOSAIC{}'s
memory allocator, called \allocatorNameLong
(\allocatorName), maintains an important soft-guarantee: memory
allocation from different processes can never fall within the same large page
range. \cjr{not sure this example is working for me. A large page mapping requires 
contiguity in both physical and virtual space, so just moving data around doesn't 
work usually--either process 1 didn't have the contiguity for these pages in the virtual 
space to begin with, and happen to have it afterward, or we have to update 
addresses used by the code (non-starter). The guarantee ensures we generally have 
that contiguity. }
\jl{This may not be the most common case, but sometimes this situation arises from compaction before the entire virtual area was allocated.}

\begin{figure}[h!]
\centering
\includegraphics[width=0.7\columnwidth]{secs/mosaic/figs/coalesce-demote-correct.pdf}%
%  \vm{This figure doesn't stand on its own (is that important?). The caption could do a little more explanation of what is happening so the reader doesn't have to find it in the text. Why do coalesce and splinter look the same? What do dashed lines represent?.}
\caption{Memory allocation in \titleShortMOSAIC aims to avoid sharing large page ranges between multiple processes, reducing the overhead of creating large pages.}
\label{fig:coalescing-example}
\vspace{-0.15in}
\end{figure}



As shown in Figure~\ref{fig:coalescing-example}, \allocatorName forces the
large page range to only contain base pages from Process~1. The clear
advantage of maintaining this guarantee is that, in the common case, 
applications do not share page frames within a large page range, allowing coalesce
operations to proceed without the need for memory copies.

\allocatorName has the disadvantage of risking application-level
fragmentation by reserving multiple large pages while they are only
partially-allocated. Our simulations (Rodinia) do not run long enough to give
rise to the levels of fragmentation that would force the allocator to preempt
some of these reservations to release physical memory, but we can simulate these
conditions by fragmenting the memory before running the simulations.
\sg{this needs to be mentioned earlier}
Compaction is performed by 
\compactionNameLong (\compactionName) when fragmentation reaches a predetermined threshold.
(see Section~\ref{sec:mosaic-motiv-fragmentation}). 
Section~\ref{sec:mosaic-eval-worst-case} provides a thorough analysis of these effects.




%\titleShortMOSAIC}{} proactively conserves contiguity and 
%avoid data copy for coalescing and compaction in the common case
%by careful management of the physical address space in the memory allocator. 
%The memory allocation policy satisfies requests to back virtual 
%memory pages out of per-application pools of 2MB-aligned 2MB contiguous 
%physical frames, or \emph{huge frames}. Consecutive allocations from a single application 
%are satisfied with some number of 4KB physical frames from the current huge frame. 
%When allocations must straddle a 2MB-aligned boundary, the allocator 
%first reserves the next free huge frame for the 
%application, satisfying the allocations with physical frames from it.  
%Under memory pressure, huge frames may be completely reserved, in which 
%case the allocator resorts first to compaction, collecting base pages 
%from partially used huge frames together. Under pathological pressure,
%the allocator satisfies the request from partially used reserved frames, 
%invalidating that reservation and losing the contiguity. 
%

%
%\rachata{This paragraph below and the next section need more work. I think
%the flow should be changed to. The invariance keep pages from different
%apps in a different large page. Then, this benefit coalescing and splintering
%as no copies is needed as shown in the Figure. Then, the actual mechanism
%of how coalescing is done with another Figure and the timeline showing the
%benefit.}


\paragraphbe{Coalescing and Splintering.} 
As we mentioned, \titleShortMOSAIC maintains a soft guarantee where, in the common
case \sg{common case only is not an invariant - rename this to ``soft
guarantee'' instead?}, the allocator will prevent processes from sharing a large page
range. \titleShortMOSAIC{}'s contiguity-aware memory allocator enables common-case coalescing and
splintering to require \emph{no} memory copy operations.  In this case, the
main tasks that the memory manager has to do are 1) ensure all leaf pages
within the large page are in the proper order %new base \sg{what do you mean by base here?} large page range, 
and 2) ensure that all the leaf pages are disabled so nothing can access an invalid small page.
%\sg{Why?  The intuition is lacking here.}
%Figure~\ref{fig:coalescing-mosaic} shows an example of coalescing and
%splintering in \titleShortMOSAIC}{}, which is called \policyName. 
For example, suppose that the page table walking process has four levels of
page table entries.  To create a large page mapping, the memory manager
atomically swaps the 8-byte L3 page table entry, currently pointing to an L4
page table page containing leaf PTEs for all the base pages in the
corresponding large page range, with a single 2MB leaf PTE. The memory manager marks
the L4 page table page as ``disabled'' but retains its entries %but does not free it 
in order to enable a similar fast path for splintering.
~\cjr{unclear--it seems to suggest we're tracking page numbers, and there's an ordering over them, which is not the intent.}
Stale TLB-resident translations for base pages in
the new large page still provide the same virtual-to-physical translation, so TLB
shootdowns can be avoided as an optimization. Hence, the only overhead during
this process is the DRAM writes to update the L3 page table entries.
Splintering performs the inverse operation. As a result, with
\titleShortMOSAIC{}, coalescing and splintering do not trigger TLB flushes or
invalidations. Additionally, the latency of DRAM writes from page table
modifications can be overlapped with the page table walk from the first large
page compulsory miss, leading to a significantly smaller performance overhead,
as shown in Figure~\ref{fig:coalescing-timeline}.
 


\begin{figure*}[h!]
\centering
\includegraphics[width=\columnwidth]{secs/mosaic/figs/coalesce-time.pdf}%
\caption{The benefit of \policyName compares to the state-of-the-art baseline. In the baseline case, virtual-to-physical mapping has to be modified, multiple pages within DRAM has to be moved and GPU cores need to be flushed before the MMU can form a large page.} 
\label{fig:coalescing-timeline}

\vspace{-0.15in}
\end{figure*}



In the case where coalescing requires a TLB shootdown because there are
multiple ongoing page walks to the same large page range, % before \policyName updates the page table entries, 
coalescing triggers the TLB shootdown. In this case, the TLB MSHR entry
responsible for the ongoing page walk triggers the memory management unit,
which then sends flush signals to all the GPU cores to stall all memory
requests. 


~\cjr{We need to
  descibe a baseline design that does TLB shootdown, and if
  we want to talk about the optimization we need to consider a) how to ensure
  concurrent page table walks on other processors either always see a
  consistent view, are are not harmed by inconsistency, b) more detail
  about how to let the TLB know to stall memory requests, and coordination
  of such stalling if it takes place at multiple L1s (conversely, does the
  design require shared L2 TLB? Do we need to coordinate stalls across
  L2 huge vs base TLB? d) what if we leave a stale mapping and then
  metadata on the new mapping changes? Mostly just need to show we're aware
  of the issues.}


Updating the page table entries allows the hardware memory management unit to
keep track of what pages are coalesced\sg{was this mode ever explicitly defined?  it should be...}. As a result, this
enables transparent support as the software side (GPGPU applications) does not
have to be aware of the large pages. However, this comes at a cost, as the
hardware side (i.e., each GPU SM) has to be able to probe into the correct TLB before
it is known whether an address falls under a large or small page. To circumvent
this problem, we 1) invalidate the large page TLB whenever there is a
splintering command so that accesses to small pages never hit in the large page
TLB and 2) probe the large TLB first before proceeding to the small TLB. 
%To reduce the number of TLB accesses to the large shared TLB, we employ a small
%per-SM Bloom filter \sg{cite} in the shared TLB to keep track of what pages are
%coalesced. This Bloom filter reduces the number of shared TLB accesses (which
%take longer than the private TLB access). Upon an L1 TLB miss, the Bloom
%filter is probed, and only addresses that hit in the Bloom filter need to
%access the large page shared TLB.\footnote{We use a 64 byte Bloom filter per
%SM, which in total contributes to a negligible 0.4\% of the L1 cache size.}
%\sg{We need to clearly state earlier that there are two TLBs.  Also, stick to huge
%  page, and avoid using large page.}\cjr{If we can't measure this feature,
%  we should be careful with our claims about it. It invites a bunch of
%  niggly empirical demands like false positive rate, etc. }


%\begin{figure}[h]
%\centering
%\includegraphics[width=\columnwidth]{secs/mosaic/figs/todo.png}%
%\caption{Coalescing and Splintering Process of \titleShortMOSAIC}.} 
%\label{fig:coalescing-mosaic}
%\end{figure}

%--our simulations do not implement it. 
%However, in a case~\cjr{don't assert this if we don't know how rare.} where a large page
%range consist of base pages
%from multiple address spaces, \titleShortMOSAIC}{} does not perform coalescing on these
%pages.~\cjr{obvious...it would break memory protection. Do you mean we don't compact?}
%The reasoning is because with our proposed memory allocator, this
%phenomenon is very rare (we do not ever observe this in our evaluation),
%and the base page TLB should be enough to handle such translations.
%Section~\ref{sec:mosaic-eval-worst-case} provides an analysis on the effect of
%these rare cases on GPU performance.

\paragraphbe{Transparency Support.} Because the software-side is responsible only for performing memory allocation,
both the CUDA and OpenCL runtimes can support \allocatorName without changes to the GPGPU
applications that are running. In the rare case that the GPU hardware is unable
to perform coalescing, the GPU can still translate the same virtual address (i.e.,
there is no change to the virtual-to-physical address mapping of the base page). Lastly, because the
soft guarantee is set, coalescing never triggers any data movement. 
%The hardware does not need to keep track of additional information in the page table entries.

% \rachata{No need to track what is in the large page -- we are not modeling the bloom filter} , except for when the page is a large page.~\cjr{not sure this needs to be said...}

%\rachata{We will want to add a discussion that the software-side only send the trigger
%to perform coalescing/splintering but the hardware side is the one responsible for
%transparently coalesce pages. Because the invariant is set so that coalescing
%never trigger data movement, hardware does not need to really keep track of anything
%as all the information are available in the page table entries. This also provides
%the benefit that the software side can transparently operate without the knowledge
%of whether the page is coalesced or not.}

%\paragraphbe{Fast Bulk Copy using RowClone and LISA.}
%When composing a large page from base pages not already backed by 
%a reserved huge frame, which occurs as the system recovers from fragmentation 
%or high memory pressure, \titleShortMOSAIC}{} must find a new huge frame, and 
%copy data from base physical frames into it, and then update page table mappings. 
%in such cases we use fast in-DRAM bulk copy
%mechanisms to minimize the overhead of copies.  Our coalescing mechanism will
%first try to find a free page within the same DRAM subarray and use RowClone to
%perform a fast bulk-copy of data~\cite{rowclone}, which can perform fast copy
%of data as long as they are from the same DRAM subarray. \rachata{We probably
%need this background somewhere in the text.} If there is no free page within
%the same subarray, our mechanism then searches for a free page within the same
%DRAM bank, and perform bulk-copy using LISA~\cite{lisa}. Because virtual to physical
%mappings are being altered \titleShortMOSAIC}{} must block all translation requests 
%for base pages involved for the duration of the coalesce operations and subsequent 
%TLB shootdown is required. 
%\cjr{URGENT: I don't know enough about RowClone or LISA to know if those 
%systems deal with outstanding writes buffered in upper level caches (or if GPU caches are write-through
%maybe it's not an issue), but since we require blocking at the TLB to enforce atomicity, 
%it seems like we need to shootdown TLBs \emph{before} doing the coalesce.} \rachata{GPU use write-through
%cache. I will cite the paper that evaluate different write policies in GPU.}

%Rachata: I do not think we will run into this?
%\paragraphbe{\remapcache} As an optimization to handle this situation we propose 
%adding a store-buffer-like remap cache, which can buffer writes 
%to pages whose virtual-to-physical mappings are being changed. The \remapcache
%is indexed by the physical frame and entries cache offset, store value pairs.  
%To know when stores should be redirected to the 
%\remapcache, \titleShortMOSAIC}{} adds a bit to TLB-entries indicating that they 
%are ``tentatively invalid''--the system can mark individual entries 
%using mechanisms similar to the INVLPG instruction. Writes to pages 
%translated using entries marked tentatively invalid are redirected to 
%the \remapcache. On completion of the mapping changes, the subsystem 
%notifies the \remapcache that mapping changes are complete, per physical 
%frame. The \remapcache releases those stores to using the offset and 
%the new physical page frame. A full \remapcache causes a memory reference 
%to block. Atomic operations implemented with write-through must similarly 
%stall.~\cjr{While the details could probably be worked out, this is 
%a bit outlandish, and optimizes a case we hope never arises, so probably 
%we cut it.} \rachata{Need to take a look into this design}

%\subsection{Tracking Spatial and Temporal Access Frequency}


\paragraphbe{Determining When to Coalesce Pages.} Coalescing and splintering
decisions are typically based on the hotness of base pages within a large page.
As observed in previous literature~\cite{cong-hpca17}, threads across multiple
warps maintain good spatial locality under multiple adjacent small pages
because these threads typically operate on the same large array or set
of data that are allocated together. We observe similar behavior in our
evaluation. Hence, we simplify the hardware by determining when to coalesce a
page proactively during the allocation phase by using how many base pages are
being mapped within the large page range. 
%Coalescing and splintering decisions
%happens when an application performs any changes to the memory mapping (e.g.,
%memory allocation, memory deallocation).

~\cjr{bring up what we've learned about the need to track locality.}

%This below does not make a lot of sense
%Hence, when the
%MMU probes a memory location under a large page range, the parallelism of the
%GPUs is more than likely forces adjacent memory locations are typically
%accessed, suggesting that as long as the utilization under the huge block range
%is high, the huge block range is likely to be accessed often, and is a good
%candidate for coalescing.

\paragraphbe{Proactively Coalescing Pages.} 
Most of the time, a program can allocate a new region of memory of any size at
any time during its execution. However, in GPGPU applications, we observe that
in order to limit the number of data transfers over PCIe, GPGPU programs groups GPU
memory allocations together. Typically, GPGPU
applications are broken down into phases: data allocation, data preparation,
kernel execution, and data retrieval. As a result, data allocations, which are
managed by the host memory allocator, are typically known before the kernel is
launched to the GPU. Hence, it is possible to modify the GPU memory allocator
to provide software support for multi-page-size TLB design. 

While the MMU can extract the page
utilization information by probing the access bit in the page table entries,\footnote{This can be
done in recent GPU architecture through the Falcon coprocessor.} \titleShortMOSAIC
goes a step further. In this work, we utilize our observation on the memory allocation 
behavior of GPGPU applications.
% from Section~\ref{sec:gpgpu-app-alloc},
%where allocation requests from GPGPU
%applications happen infrequency and in large chunks. 
%Hence, 
Specifically, we observed empirically that the base page mapping information in combination with
an LRU policy can infer the utilization of a page. This means that many coalescing decisions can be
determined at allocation time.\footnote{Note that only the coalescing
decision is determined during allocation and that, while the MMU is aware of these
coalesced commands, the MMU still behaves as if these pages are small pages
until the coalescing command is committed.} When the kernel containing these
coalesced pages is dispatched and the data is copied from the CPU-side memory
to the GPU-side memory, the MMU then performs coalescing right away. This
provides an additional benefit, as preemptively coalescing pages reduces the amount
of thrashing on the small page TLBs. 
\sg{unclear why}~\cjr{as we discussed inferring
  high utilization from malloc, as currently written suggests we don't know the
  difference between \emph{mapped} and \emph{utilized}. Justify these assertions
  empirically. }


%\titleShortMOSAIC}{} coalesces and splinters pages based on hotness, which indicates 
%how likely pages within the large page region are going to be touched again, to determine
%whether to coalesce a page into a large page or not. To track hotness, we add
%a table whose entries are a 2-bit saturating counter. When a TLB is
%accessed, two tags are generated. First, the normal tag is generated to index
%into the TLB tag arrays. Second, another the tag is generated using the huge
%page size, and the tag is used as an index into the saturated counter table,
%and the entry representing this tag is incremented. This hash table represents
%when the page is last touched to each page table entries without tracking every
%single large pages. This saturating counter is decremented periodically, and
%once the number within the saturating counter exceed a threshold, a page is
%coalesced into a large page. 

%\rachata{Update this}


\paragraphbe{Determining When to Splinter a Large Page.} Because the coalescing decision
is made proactively using the base page mapping information, we can further simplify
the hardware by deferring splintering until the page is deallocated. If deallocation
frees up only a part of a large page, \policyName will splinter the remaining pages
back into small pages.
%During the time changes in the
%physical memory structure happen only at a coarse granularity, before a kernel
%launches or when a kernel finishes. 

%\paragraphbe{Determining When to Splinter a Huge Page.} Because changes in the
%physical memory structure happen only at a coarse granularity, before a kernel
%launches or when a kernel finishes. It is possible to defer page splintering
%until the end of a kernel, when old pages are deallocated, leading to data
%fragmentation. In this work, because we observe that GPGPU applications tend to
%deallocate data in huge chunks, we empirically choose always to splinter huge
%pages upon deallocation.~\cjr{since physical region is unmapped, splinter is
%sort of meaningless. What do we really mean here? The region is free.}
%However, further policy changes \sg{policy changes?  is that the right term?}
%can be supported by changing the runtime.

% To determine when a large page
%should be splintered back to a small page we added a bit vector to the huge
%page table entry\cjr{need some way to put it in a side-table as PTEs do not have available bits}
%\rachata{If a table is used, this would require 2MB total, which is pretty big. Will need
%an alternative}, 
%representing occupied pages within the large page region.  If
%a page free up within the large page region, the corresponding bit within this
%bit vector is set. The number of set bits in this vector represents the amount
%of fragmentation in the large page region. Once the number of set bits reach a
%threshold, a large page is demoted.

%\begin{comment}
%
%Potentially difficult issues: 
%\begin{compactitem}
%\item atomic instructions 
%\item read after write dependences that cross SM boundaries. If we had coherence, this would be simple. 
%	If the coalesce is driven by a memory reference from a particular SM (and is therefore synchronous)
%	the weak ordering of the memory model makes this a non-issue. Some reads that would have 
%	seen a new value (being buffered during copy) will observe an old value. Barriers would have been
%	required to enforce any program-level ordering requirements, and those would not be reached because the SM
%	that triggered the coalesce is stalled. However, if coalesce is completely asynchronous, this is a real 
%	problem. Do any of these issues arise in RowClone? \rachata{Coherency is applied in the simulator we use on RowClone.}
%\end{compactitem}
%
%\end{comment}
%
%\rachata{We might want to point out again that this is one of the primary reason
%why GPU should still support small page. I.e., demand paging is costly, but sometimes
%is needed. Managing at 2MB page is too costly.}

\paragraphbe{Demand Paging.} Lastly, to provide support for demand
paging, we restrict the size of the page so that only small pages are allowed
to be demand paged. To enforce this restriction, if a large page is touched 
by a demand paging operation, we first splinter the page so that
demand paging is only performed on a subset of the needed small pages.
\cjr{should go under splinter/coalesce policy. Need to acknowledge additional
  latency incurred for splinter operation on demand paging too.}


%\cjr{from here on out probably goes in meth}

%\rachata{These are new content that motivate/describe our compaction mechanism}

\subsubsection{Dealing with Data Fragmentation}
\label{sec:mosaic-motiv-fragmentation}

As shown in Figure~\ref{fig:coalescing-example}, the combination of \allocatorName{}
and \policyName can increase data fragmentation by coalescing unallocated pages
under a large page. 
%While we observe that GPGPU applications
%are unlikely to have large pages with low utilization~\cjr{achtung!} (see Section~\ref{sec:gpgpu-app-alloc}),
We introduce \compactionNameLong (\compactionName) to \titleShortMOSAIC{} to address any rare cases where
memory compaction is needed to reduce data fragmentation.

%In additional to the TLB invalidation overhead, running applications
%concurrently pose an additional design question for the memory allocator. On
%one hand, mapping allocation requests within a tight region can minimize the
%memory footprint and allows more data to stay in the main memory. However,
%doing so also introduces data fragmentation. This fragmentation comes in two
%forms 1) allocation-fragmentation during the allocation, where applications from different
%address space falls under the same huge frame and 2) post-deallocation-fragmentation after
%a memory region is deallocated, where the utilization of the huge frame
%drop as there are more free pages within the huge frame range.
%Figure~\ref{fig:data-fragmentation} shows data layout when three different
%GPGPU applications are running concurrently. In
%Figure~\ref{fig:data-fragmentation}, we modified the GPGPUsim memory allocator
%to maps each application to be aligned to different page size. We then identify
%1) the number of contiguous 2MB region that belongs exclusively to one
%application, 2) the number of contiguous 2MB region that has a few (less than
%10\%) pages from a different application, and 3) the number of contiguous 2MB
%region that consist of pages from multiple applications. As shown, when trying
%to minimize the number of memory bloat by aligning data to small page size, the
%opportunity of page coalescing significantly decreases.

%\begin{figure}[t!]
%\centering
%  \includegraphics[height=1in]{./secs/mosaic/figs/todo.png}
%  \caption{\footnotesize{A figure showing snapshot of fragmentation when data is allocated in 4KB vs. 2MB region.
%	\assign{Rachata}}}
%  \label{fig:data-fragmentation}
%\end{figure}

%As for post-deallocation fragmentation, regions of memory get deallocated over
%time once they are not needed. This exacerbates the fragmentation problem
%further, increasing memory bloat.

\paragraphbe{Reducing Fragmentation Through Memory Compaction.} 
%While our
%proposed allocation policy can eliminate fragmentation that occurs during
%allocation, it does not reduce fragmentation after deallocation. To solve
%this, we utilize memory compaction, and provide another optimization based on
%the assumption that \titleShortMOSAIC} memory allocation has eliminated pre-allocation
%fragmentation and proposed \compactionName.  \sg{Poor English here makes it hard
%for me to understand what you're saying.  Reword this sentence, please.}
Traditionally, memory compaction is done by rearranging base pages to
form a tight memory region where there is no unallocated memory between base pages.
Figure~\ref{fig:mosaic-compaction} shows an example of the compaction process.  For
the baseline in our example, multiple pages under three different large page ranges
(A, B and C) go through a compaction process. In the baseline, pages under
the large page range C are moved to large page ranges A and B. The resulting
page arrangement prevents coalescing in large page ranges A and B without
requiring additional data movements.\footnote{In the case of contiguous virtual addresses that
span multiple pages, there must be enough contiguous virtual space for compaction
to proceed in both the baseline design and \titleShortMOSAIC.}

\begin{figure}[h!]
\centering
  \includegraphics[width=0.7\columnwidth]{./secs/mosaic/figs/compaction.pdf}
%  \rachata{use an actual address (VA/PA) in the example}
%  \vm{This figure doesn't stand on its own (is that important?). The caption could do a little more explanation of what is happening so the reader doesn't have to find it in the text.}
  \caption{The difference between the baseline compaction mechanism and \compactionName showing that \compactionName always preserve soft-guarantee imposed by \allocatorName.}
  \label{fig:mosaic-compaction}
\end{figure}



In \titleShortMOSAIC{}, \compactionName{} is modified to
maintain our guarantee that large pages only contain pages from the same
process by sorting base pages into new large pages based on
their process ID. This ensures all pages in each large page range (A
and B) belong to a single application, as shown in
Figure~\ref{fig:mosaic-compaction}. Because \compactionName forces compaction
to happen locally (i.e., pages from different applications cannot mix
within the same large page range), \compactionName does not completely eliminate
all fragmentation as shown in ~\ref{fig:mosaic-compaction}. However, in the
worst case, this fragmentation only happens to the last large page of each
application.
% as well as when there is a contiguous virtual blocks that spans multiple pages.
%In the worst case, the remaining fragmentation in \compactionName
%is $HugeBlockSize * numApps$, which is very small.



%However, using such compaction mechanism involves multiple copies, many of
%which occurs across memory partitions. As a result, memory requests to DRAM
%has to be stalled during the whole period when compaction happens.

%\begin{figure}[h!]
%\centering
%  \includegraphics[height=1in]{./secs/mosaic/figs/todo.png}
%  \caption{\footnotesize{A figure showing the overhead of Linux-based compaction mechanism.
%	\assign{Rachata}}}
%  \label{fig:data-fragmentation}
%\end{figure}

\paragraphbe{Bulk Copy.}
% While we do not observe significant data fragmentation
%in our evaluation, 
To further optimize the performance of \compactionName, it is possible
to utilize two in-DRAM bulk copy techniques~\cite{seshadri2013rowclone,lisa}
to reduce the latency of page-level copy. This can be done by
limiting the compaction process to a single memory channel.
%We can use existing techniques that rapidly copy pages in the rare
%cases where \titleShortMOSAIC}{} fragments the main memory.
%Seshadri et al.\ propose
%RowClone~\cite{seshadri2013rowclone}, which is a technique that allows the memory controller
%to send a series of existing DRAM commands to copy an entire row
%within the same DRAM subarray \sg{undefined} to another row. Chang et al.\ propose
%LISA~\cite{lisa}, which requires a minimal modification to the DRAM array, but
%allows low-latency copy of data \emph{across} DRAM subarrays.
%Both of these techniques
%can be used with \titleShortMOSAIC}{} to further reduce the
%overhead of data fragmentation. 
%
% It is possible to employ these two techniques (LISA and RowClone) to
% \titleShortMOSAIC}{}. 
%The compaction process can be done locally in each memory channel.
As a result, a compaction that happens in one memory channel will not stall
memory requests (or shared cache requests) to other memory partitions (and channels). 
%When compaction happens locally, all data movements are
%guaranteed to have very low latency by utilizing either inter-subarray
%bulk-copy with RowClone or inter-bank bulk-copy using LISA.
%\sg{Do we need this kind of detail?  Isn't it enough to say that RowClone and
%LISA provide fast copy mechanisms within and across subarrays?}

\subsection{Overall Design of Mosaic}
\label{sec:mosaic-overall-design}

\sg{How is this different than 4.2?  The subsection names give no clue.}


\begin{figure*}[h!]
\centering
  \includegraphics[width=0.8\columnwidth]{./secs/mosaic/figs/sim-infra-new.pdf}
  \caption{The overall design of \titleShortMOSAIC. (1) \allocatorNameLong provides the soft-guarantee allowing \policyName to coalesce pages transparently. 
(2) coalesce requests are sent to \policyName prior to kernel launch (3). (4) \compactionNameLong provides physical space contiguity and reduces the
amount of fragmentation.}
  \label{fig:mosaic-overall}
\end{figure*}



Figure~\ref{fig:mosaic-overall} shows the overall design of \titleShortMOSAIC.  Upon
reaching a memory allocation call from a GPGPU application, \allocatorName
performs memory allocation while preserving the soft guarantee that a large
page range can only contain pages from the same application (\mycirc{1}).
Then, if the software runtime observes an opportunity to coalesce a page, it
sends a coalescing command to \policyName in order to perform low-overhead
memory coalescing (\mycirc{2}). This allocation process continues until the
GPGPU application reaches its kernel launch (\mycirc{3}). \titleShortMOSAIC maintains
these execution flows until an application wants to deallocate memory. When
there is a deallocation, \titleShortMOSAIC performs page splintering by sending a
splinter command to \policyName (\mycirc{2}). Afterward, the memory allocator
checks for memory fragmentation.  If the fragmentation exceeds  a certain
threshold, \titleShortMOSAIC performs memory compaction, as described in
Section~\ref{sec:mosaic-motiv-fragmentation} (\mycirc{4}).




%\paragraphbe{Fast Bulk Copy.}
%During the compaction, \titleShortMOSAIC}{} must find a new huge frame, and 
%copy data from base physical frames into it, and then update page table mappings. 
%in such cases we use fast in-DRAM bulk copy
%mechanisms to minimize the overhead of copies. Our compaction mechanism works as follow
%First, for each memory partition, the compaction routine calculate the number of huge frames required to hold all
%the base pages using the summing up utilization of each application's huge frame.
%Then, the compaction routine select the huge frame with the most utilization, then
%fill with base page from another huge frame (from the frame with the lowest utilization first) until
%the selected huge frame is fully utilized. During the merge, our mechanism
%first tries to find a free page within the same DRAM subarray and use RowClone to
%perform a fast bulk-copy of data~\cite{rowclone}, which can perform fast copy
%of data as long as they are from the same DRAM subarray. \rachata{We probably
%need this background somewhere in the text.} If there is no free page within
%the same subarray, our mechanism then searches for a free page within the same
%DRAM bank, and perform bulk-copy using LISA~\cite{lisa}. Because this happens
%locally within the same channel, our mechanism is guaranteed to be able to either
%utilize RowClone or LISA, significantly reducing the latency of compaction.
%
%
%Lastly, because virtual to physical mappings are being altered \titleShortMOSAIC}{}
%must block all translation requests to this channel for base pages involved for
%the duration of the coalesce operations and subsequent TLB shootdown is
%required. 
%\cjr{URGENT: I don't know enough about RowClone or LISA to know if those 
%systems deal with outstanding writes buffered in upper level caches (or if GPU caches are write-through
%maybe it's not an issue), but since we require blocking at the TLB to enforce atomicity, 
%it seems like we need to shootdown TLBs \emph{before} doing the coalesce.} \rachata{GPU use write-through
%cache. I will cite the paper that evaluate different write policies in GPU.}




==> secs/mosaic/secs/related.tex <==
% !TEX root=../paper.tex

\section{Related Work}

To our knowledge, \changesIII{this is} the first work to
(1)~analyze the fundamental trade-offs between TLB reach, demand paging 
performance, and internal page fragmentation; and
(2)~propose an application-transparent GPU memory manager that preemptively
coalesces pages at allocation time to improve address translation performance, 
while avoiding the demand paging inefficiencies and memory copy overheads 
typically associated with large page support.
% . Our new application-transparent mechanism manages multiple
% page sizes on GPU in order to effectively increase the TLB reach and
% reduce the performance overhead of address translation in GPUs.}
Reducing performance degradation from address translation overhead is an
active area of work for CPUs, and the performance loss that we observe as a 
result of \changesIII{address} translation is well
corroborated~\cite{direct-segment, jayneel-micro14, bhattacharjee-hpca11,gaud14atc,
merrifield-2016-vee}.  In this section, we discuss previous techniques that aim
to reduce the overhead of address translation. % in CPUs, GPUs and heterogeneous
%CPU-GPU architecture.
%\sg{no statement about our novelty here?}
%Gaud et al. observe that large page sizes can harm performance on NUMA machines with
%increased page migration latency and page-level false sharing~\cite{gaud14atc}.

%\subsection{Multiple Page Sizes}
\subsection{\changesIII{TLB Designs for CPU Systems}}

%\paragraphbe{CPU.}
TLB miss overhead can be reduced by (1)~accelerating page table
walks~\cite{barr-isca10,large-reach} or reducing the walk
frequency~\cite{jayneel-isca16}; or (2)~reducing the number of TLB misses (e.g.,
through prefetching~\cite{bhattacharjee-pact09, kandiraju-isca02,
saulsbury-isca00}, prediction~\cite{prediction-tlb}, or structural changes to
the TLB~\cite{talluri-asplos94, binh-colt, binh-hpca14} or TLB
hierarchy~\cite{bhattacharjee-hpca11, lustig-13, srikantaiah-micro10,
ahn-tocs15, ahn-isca12, rmm, direct-segment, jayneel-micro14}).

\paragraphbe{\changesIII{Support for Multiple Page Sizes.}} \changesIII{Multi-page} mapping 
techniques~\cite{talluri-asplos94, binh-colt, binh-hpca14}
\changesIIIII{use a single TLB entry for multiple page translations,}
% map multiple page translations using a single TLB entry,
improving TLB reach by a small
factor; much greater improvements to TLB reach are needed to
deal with modern memory sizes. 
%Direct segments~\cite{direct-segment,
%jayneel-micro14} extend standard base paging with a large segment to map the
%majority of an address space to a contiguous physical memory region, but these approaches
%require application modifications. %and are limited to workloads able to a single large segment. 
%Redundant memory mappings (RMM)~\cite{rmm} extend TLB
%reach by mapping {\it ranges} of virtually- and physically-contiguous pages in a
%range TLB.
%MIX TLBs~\cite{cox17asplos} enable set-associative TLBs to accommodate entries that translate
\changesIIIII{\changesIIIIII{MIX TLB~\cite{cox17asplos} accommodates} entries that translate
multiple page sizes, eliminating the need for \changesIIIIII{a dedicated set of TLB
large page entries}}. \changesIIIIII{MIX TLB is} orthogonal to our work, and \changesIIIIII{can be used with \titleShortMOSAIC to
further improve TLB reach.}
%benefit further from the improved TLB reach enabled by MIX TLBs.


%The policies and mechanisms used to implement \changesIII{application-transparent large} page
%support in \titleShortMOSAIC{} are influenced by a wealth of previous research
%on OS support for large pages for CPUs. 
Navarro et al.~\cite{superpage} identify
contiguity-awareness and fragmentation reduction as primary concerns for large page management,
proposing reservation-based allocation and deferred promotion (i.e., coalescing) of base pages to large pages.
\changesIII{Similar} ideas are widely used in modern OSes~\cite{thp}.
\changesIIIIII{Instead of the reservation-based scheme, Ingens~\cite{ingens} employs a utilization-based scheme that uses a bit vector to track}
spatial and temporal utilization of base pages.
%Ingens implements promotion \changesIII{(coalescing)}
%and demotion \changesIII{(splintering)} asynchronously, rather than in a page fault handler. 
%These basic ideas \changesIII{of coalescing and splintering pages asynchronously} heavily influence \titleShort{}'s design. % which attempts to emulate these same policies in hardware. 

%In contrast to Ingens, \titleShortMOSAIC{} can take advantage of the memory allocation
%behavior of GPGPU applications to avoid the need to sample access bits
%when making coalescing decisions.

% reon dedicated hardware to provide
% access frequency and distribution, and need not infer it by sampling
% access bits whose granularity may be a poor fit for the page size.

\paragraphbe{\changesIII{Techniques to Increase Memory Contiguity.}} 
%A number of related works propose hardware support to recover and expose memory
%contiguity. 
\changesIIIII{GLUE~\cite{binh-micro15} groups contiguous, aligned base page
translations under a single speculative large page translation in the TLB.
%Speculative translations (similar to SpecTLB~\cite{spectlb}) can be verified
%by \changesIII{off-the-critical-path} page-table walks, reducing the effective page-table walk
%latency.  
GTSM~\cite{du15hpca} provides hardware support to leverage the contiguity of
physical memory \changesIIIIII{region} even when pages have been retired due to bit errors.
These mechanisms for preserving or recovering contiguity are orthogonal to 
the contiguity-conserving allocation we propose for \titleShort, and \changesIII{they} can
help \titleShortMOSAIC by avoiding the need for compaction.}


Gorman et al.~\cite{gorman-ismm08} propose a placement policy for an OS's 
physical page allocator that mitigates fragmentation and promotes contiguity 
by grouping pages according to \changesIIIIII{the amount of migration required
to achieve contiguity}. Subsequent work~\cite{gorman-wiosca10}
proposes a software-exposed interface for applications to explicitly
request large pages like {\tt libhugetlbfs}~\cite{libhugetlbfs}.
These ideas are complementary to our work.
\titleShortMOSAIC can potentially benefit from similar policies if they can be simplified
enough to be \changesIIIII{implementable} in hardware. 
%We leave the exploration of these policies as future work.

% \paragraphbe{\changesIII{Page Walk Cache Designs.}} 
\paragraphbe{\changesIIIII{Alternative TLB Designs}.} 
Research on shared last-level TLB
designs~\cite{inter-core-tlb, bhattacharjee-hpca11, lustig-13} and page walk cache
designs~\cite{large-reach} has yielded mechanisms that accelerate
multithreaded CPU applications by sharing translations between cores. 
%Barr et al.~\cite{spectlb} propose a technique that predicts address
\changesIIIII{SpecTLB~\cite{spectlb} provides a technique that predicts address
\changesIII{translations}. While speculation works on CPU applications,
speculation for highly-parallel GPUs is more complicated, and can eventually
waste \changesIII{off-chip DRAM} bandwidth, which is a highly-contended resource in GPUs.}
%This proposal mainly target system with small pages, which generally increases
%the cost of translation upon a TLB miss, which can be common in GPUs.
%\cjr{Smaller than 4k?}
%
%
%\paragraphbe{Alternative Designs to Improve TLB Reach.} Direct segments~\cite{direct-segment}
\changesIIIII{Direct segments~\cite{direct-segment}
and redundant memory mappings~\cite{rmm} provide virtual memory support
for server workloads that reduce the overhead of address translation. 
%Both are active areas of research. 
These proposals map large contiguous chunks of virtual memory
to the physical address space in order to reduce the address translation
overhead. While these techniques improve the TLB reach, % in a similar manner as large pages, 
they increase the transfer latency depending on the size of the
virtual chunks \changesIIIIII{they} map.}




%\paragraphbe{GPU.}
%
%\begin{itemize}
%\item envytools documentation showing NVIDIA GPUs have 4,16,64KB pages, using segments + 2-level page table
%\item documentation of AMD architecture. Anecdotally, I know new GPU has L1/L2 TLB, 64 contexts per core, and a similar
%  range of page sizes to NVIDIA.
%\item revisit kecker page placement paper, which he asserts (perhaps inaccurately) says something about this.
%\end{itemize}

  %\sg{Can we say that they do not provide practical support for multiple page sizes?}


\subsection{\changesIII{TLB Designs for GPU Systems}}

\paragraphbe{TLB Designs for Heterogeneous Systems.} 
%A number of previous works on enabling 2MB large page support for GPUs report initial
%findings that a larger page size can improve TLB reach~\cite{pichai-asplos14,
%powers-hpca14} and prefetch locality~\cite{tianhao-hpca16}. 
%Gaud et al. observe that large page sizes can harm performance on NUMA machines with
%increased page migration latency and page-level false sharing~\cite{gaud14atc}.
%Their findings are analogous to the findings that we make, and \changesIII{preventing} page migration to avoid performance loss is a key goal for \titleShort.
Previous works provide several TLB designs for
heterogeneous systems with
GPUs~\cite{powers-hpca14,pichai-asplos14,abhishek-ispass16} and with 
accelerators~\cite{cong-hpca17}. 
\changesIIIII{\titleShort{}} improves upon a state-of-the-art TLB
design~\cite{powers-hpca14} by providing application-transparent,
high-performance support for multiple page sizes in GPUs.
\changesIII{No prior work provides such support.}
% In this
% work, \titleShortMOSAIC{} improves on the best performing configuration out of these
% designs by providing transparent and high-performance multi-page-size support.

%Rachata This is a repeat of up there
%Cox et al.~\cite{cox17asplos} propose a low-cost centralized TLB design that allows entries of
%different page sizes to share a centralized structure.  This
%TLB design is orthogonal to our work, and solves a completely different problem
%(a consolidated TLB for multiple page sizes, as opposed to reducing address translation
%and demand paging overheads).

%It can be combined with \titleShortMOSAIC to reduce the overhead of supporting
%multiple-page size. 

\paragraphbe{TLB-Aware Warp Scheduler.} Pichai et al.~\cite{pichai-asplos14}
%perform a design exploration of heterogeneous CPU-GPU systems, and 
\changesIIIIII{extend the cache-conscious warp scheduler~\cite{ccws} to be} aware of the 
TLB \changesIIIIII{in heterogeneous CPU-GPU systems}. 
%This design also provides parallel TLB accesses at the L1 cache level.
These techniques are orthogonal to the problem we focus on, and can be applied
in conjunction with \titleShortMOSAIC{} to further improve performance.

\paragraphbe{Analysis of Address Translation in GPUs.}
Vesely et al.~\cite{abhishek-ispass16} analyze support for virtual memory in
heterogeneous systems, finding 
that the cost of address translation in GPUs is an order of magnitude
higher than \changesIII{that} in CPUs. They observe that \changesIIIII{high-latency} address translations limit the GPU's
latency hiding capability and hurt performance, which is
in line with the observations we make in
Section~\ref{sec:motivation-mosaic}.
Mei et al.~\cite{gpu-arch-microbenchmarking} use a set of microbenchmarks to evaluate the address
translation process in commercial GPUs.
Their work concludes that previous NVIDIA architectures~\cite{kepler,maxwell}
have \emph{off-chip} L1 and L2 TLBs, which lead
% ; however, these TLBs are off-chip, which leads
to poor performance. 
%We find this observation to be in line with our evaluation,
%as well as with previous works~\cite{abhishek-ispass16,powers-hpca14,cong-hpca17}

%\cjr{need to cite ``Dissecting GPU Memory Hierarchy through Microbenchmarking''~\cite{gpu-arch-microbenchmarking} 2016 paper 
%that microbenchmarks to find microarchitecture parameters. In particular, they prove that 
%while previous NVIDIA architectures do have L1 and L2 TLBs, they are off chip. Which is 
%what we've been saying.}


\sloppypar{\paragraphbe{\changesIII{Other Ways to Manage Virtual Memory.}} 
VAST~\cite{vast} is a software-managed virtual memory space for
GPUs. In that work, the authors observe that the limited size of physical
memory typically prevents data-parallel programs from utilizing GPUs. To
address this, VAST automatically partitions GPU programs into chunks that fit \changesIIIIII{within} the
physical memory space to create an illusion of \changesIIIIII{virtual memory.} 
Unlike \titleShort{}, VAST is \changesIIIIII{unable} to provide memory protection from 
concurrently-\changesIIIII{executing} GPGPU applications.
Zorua~\cite{zorua} is a holistic mechanism to virtualize
multiple hardware resources within the GPU. Zorua does not virtualize the
main memory, and is thus orthogonal to our work. \changesIII{CABA~\cite{caba}
introduces assist warps, which act as background helper threads for GPU SMs. These assist
warps can be adapted to perform various memory virtualization functions, such as
page walks and base page utilization analysis.}}

%% However, this proposal does not work on GPU workloads as memory
%% allocations in GPU applications are more dynamic. 
%% CJR: the real thing here is that you don't need this stuff on
%% a card that can only address 5-10GB of memory. However, there's no 
%% reason our work can't use these ideas. 


%\cjr{related work for RowClone and LISA please.}





\subsection{Demand Paging for GPUs}

%In a program running on CPU-GPU systems, performing demand paging can be done
%through the OS on the CPU side. However, this is no longer possible when demand
%paging is done to support concurrent GPU applications. 

Demand paging is a challenge for GPUs~\cite{abhishek-ispass16}.  Recent
works~\cite{tianhao-hpca16, cc-numa-gpu-hpca15}, and the
AMD hUMA~\cite{huma} and NVIDIA PASCAL
architectures~\cite{tianhao-hpca16,pascal}
% , and recent work on CC-NUMA~\cite{cc-numa-gpu-hpca15} 
provide various levels of support for demand paging in GPUs.
%These techniques are orthogonal to \titleShort, and, 
These techniques do not tackle the existing trade-off in GPUs
between using large pages to improve address translation and
using base pages to minimize demand paging overhead, which
we relax with \titleShort.
As we discuss in
Section~\ref{sec:motivation-mosaic}, support for multiple page sizes can be
adapted to minimize the overhead of demand paging by limiting demand paging to
\changesIIIII{base} pages only.
% to support paging.


%Lastly, when there is an interrupt or an exception, the GPU will have to be
%able to handle the long latency of the interrupt to resolve. These latency
%generally range in hundred thousand to million cycles. Generally, when these
%interrupt occurs in other systems, an interrupt handler from the Operating
%system will handle the interrupt while the processor perform a context switch
%and run other processes during this event in order to utilize the stalling
%cores. However, in GPU, two major components are missing.  First, preemption
%does not exist and the application current running on the GPU will stall.
%Second, there is no operating system to handle the interrupt. In this work, we
%address both problems by first introducing cross-cores task migration, which
%allows other concurrent applications from other cores to migrate, acting
%similar to a context switch. Second, we introduce [TODO: Continue]





==> secs/motivation.tex <==



==> secs/prelim.tex <==

\section{Preliminary Work}

\subsection{Reducing Interference of a GPGPU Application through Memory Divergence Correction}
\label{sec:prelim-medic}

In the past, GPUs strictly executed Graphics applications, which naturally
exhibit large amounts of concurrency.  In recent years, with tools such as
CUDA~\cite{programmingguide} and OpenCL~\cite{khronos2008opencl}, programmers
have been able to adapt non-Graphics applications to GPUs, writing these
applications to have thousands of threads that can be run on a SIMD computation
engine. Such adapted non-Graphics programs are known as general-purpose GPU
(GPGPU) applications. Prior work has demonstrated that many scientific and data
analysis applications can be executed significantly faster when programmed to
run on GPUs~\cite{rodinia,parboil,mars,lonestar}.

While many GPGPU applications can tolerate a significant amount of memory
latency due to their parallelism and the use of fine-grained multithreading,
many previous works (e.g.,~\cite{caba,owl-asplos13,largewarps,osp-isca13})
observe that GPU cores still stall for a significant fraction of time when
running many other GPGPU applications.  One significant source of these stalls
is \emph{memory divergence}, where the threads of a warp reach a memory
instruction, and some of the threads' memory requests take longer to service
than the requests from other threads~\cite{largewarps,warpsub,chatterjee-sc14}.
Since all threads within a warp operate in lockstep due to the SIMD execution
model, the warp cannot proceed to the next instruction until the \emph{slowest}
request within the warp completes, and \emph{all} threads are ready to continue
execution. 

%\begin{itemize}
%    \item Figure~\ref{fig:mem-div}a shows a \emph{mostly-hit warp}, where most
%        of the warp's memory accesses hit in the cache (\mycirc{1}). However, a
%        single access misses in the cache and must go to main memory
%        (\mycirc{2}). As a result, the \emph{entire warp} is stalled until the
%        much longer cache miss completes. 
%    \item Figure~\ref{fig:mem-div}b shows a \emph{mostly-miss warp}, where 
%        most of the warp's memory requests miss in the cache (\mycirc{3}), resulting in many
%        accesses to main memory. Even though some requests are cache hits (\mycirc{4}),
%        these do not benefit the execution time of the warp.
%\end{itemize}


%\subsection{Mitigating Inter-warp Interference in GPUs}
%
%In this work, we make three key observations: (1) across warps, there is heterogeneity
%in the degree of memory divergence experienced at the shared L2 cache, (2) a warp tends
%to retain its memory divergence behavior for long periods of execution, and (3) significant
%queuing delays occur at the L2 cache due to the high amount of memory request parallelism.
%We use these three observations to develop \emph{Memory Divergence Correction} (MeDiC),
%a GPU-specific mechanism that exploits memory divergence heterogeneity to improve
%GPGPU application performance.  MeDiC classifies warps based on their degree of divergence
%(i.e., how many threads within a warp are shared cache hits, and how many are cache misses),
%and uses this classification to drive three components: (1) warp-type-aware cache
%bypassing logic, (2) warp-type-aware cache insertion, and (3) warp-type-aware memory
%scheduling.

\subsubsection{Memory Divergence Heterogeneity}
%\vspace{3pt}

Figures~\ref{fig:mem-div}a and~\ref{fig:mem-div}b show examples of memory
divergence within a warp. As shown in Figure~\ref{fig:mem-div}, there is
\emph{heterogeneity across warps} in the degree of memory divergence
experienced by each warp at the shared L2 cache.  
%Figure~\ref{fig:mem-div} shows examples of two different \emph{types of warps}
%that exhibit different degrees of memory divergence.
Figure~\ref{fig:mem-div}a shows a \emph{mostly-hit warp}, where most of the
warp's memory accesses hit in the cache (\mycirc{1}). However, a single access
misses in the cache and must go to main memory (\mycirc{2}) and the
\emph{entire warp} is stalled until the much longer cache miss completes.
Figure~\ref{fig:mem-div}b shows a \emph{mostly-miss warp}, where most of the
warp's memory requests miss in the cache (\mycirc{3}), resulting in many
accesses to main memory.  Even though some requests are cache hits
(\mycirc{4}), these do not benefit the execution time of the warp.

\begin{figure}[h]
	\centering
        \vspace{3pt}
	\includegraphics[width=0.6\columnwidth]{fig/mem-divergence.pdf}	
    \caption{Memory divergence within a warp. (a) and (b) show the heterogeneity between
    \emph{mostly-hit} and \emph{mostly-miss} warps, respectively.  (c) and (d) show the change in stall time from 
    converting \emph{mostly-hit warps into all-hit warps}, and \emph{mostly-miss warps into all-miss
    warps}, respectively.}
	\label{fig:mem-div}
\end{figure}

Our preliminary work, \titleShortMeDiC, provides two mechanisms,
warp-type-aware cache bypassing and warp-type-aware cache insertion policy, to
convert \emph{mostly-hit} warps into \emph{all-hit} warps, where all requests
in the warp hit in the cache, reducing the stall time of mostly-hit warp
significantly. This is done at the cost of converting the \emph{mostly-miss}
warps into \emph{all-miss} warps without increasing their stall time.  To speed
up uncacheable cache misses from mostly-hit warps, the warp-type-aware memory
scheduling policy in \titleShortMeDiC prioritize memory requests from
mostly-hit warps over memory requests from mostly-miss warps.



\subsubsection{Memory Divergence Stability Over Time}
\emph{A warp tends to retain its memory divergence behavior} (e.g., whether or
not it is mostly-hit or mostly-miss) \emph{for long periods of execution}, and
is thus predictable.  This is due to the spatial and temporal locality of each
thread within the warp. Figure~\ref{fig:warp-ratio-trend} shows a sample of
warps from a selected application that shows this predictability. This
predictability enables us to perform history-based warp divergence
characterization. 

In MeDiC, we include  warp type identification logic, which profiles and
categorize warps into one of the five categories: \emph{all-hit},
\emph{mostly-hit}, \emph{balanced}, \emph{mostly-miss} and \emph{all-miss}. To
cope with long-term shifts in warp divergence behavior, he hit ratio is
periodically resampled, and the warp type is adjusted if need be.

        \begin{figure}[h]
        \centering
	\includegraphics[width=0.75\columnwidth]{results/hit_ratio_bfs.pdf}%	
	\caption{Hit ratio of randomly selected warps over time.} 
	\label{fig:warp-ratio-trend}
        \end{figure}


% We also show that a warp tends to retain their memory divergence behavior
% throughout its lifetime. This predictability enables us to perform history-based warp
% characterization as we will show in Section~\ref{sec:mech}.


%Second, we observed that the same warp tends to exhibit the similar memory
%divergence pattern. In particular, we observe that warps that have most of its
%threads miss at the cache tend to retain its divergence characteristics. This
%allows an easy method to keep track of the divergence in each warp. In this
%paper, we take advantage of this observation and use a simple per-warp counter
%to keep track of the divergence information. Additionally, we proposed several
%improvements to how memory requests is handled at the cache and main memory
%in order to take advantage of this divergence information.

\subsubsection{High Queuing Latencies at the Shared Cache due to Interference}

Due to the amount of thread parallelism within a GPU, \emph{a large number of
memory requests can arrive at the L2 cache in a small window of execution time,
leading to significant queuing delays}.  Prior work observes high access
latencies for the shared L2 cache within a GPU~\cite{sisoftware,
coherence-hpca13,demystify}, but does not identify \emph{why} these latencies
are so high.  We show that when a large number of requests arrive at the L2
cache, both the limited number of read/write ports and backpressure from cache
bank conflicts force many of these requests to queue up for long periods of
time. We observe that this queuing latency can sometimes add \emph{hundreds} of
cycles to the cache access latency, and that non-uniform queuing across the
different cache banks exacerbates memory divergence.
Figure~\ref{fig:l2-queue-latency} quantify the magnitude of this queue
contention when setting the cache lookup latency at one cycle. As shown, a
significant number of requests experience tens to hundreds of cycles of queuing
delay.

The warp-type-aware bypassing logic in MeDiC helps to alleviate these L2
queuing latencies.  By preventing mostly-miss and all-miss warps from
accessing the cache, which yields little benefits to them, we reduce
the access latencies for requests from mostly-hit and all-hit warps.

\begin{figure}[h]
	\centering
	\includegraphics[width=2.5in,angle=270]{results/queuing_lat.pdf}	
        \caption{Distribution of per-request queuing latencies for L2 cache requests from BFS.}
	\label{fig:l2-queue-latency}
\end{figure}


%
%\begin{figure}[h]
%	\center
%        \begin{subfigure}[h]{3in}
%	\includegraphics[width=3in]{results/hit_ratio_bfs.pdf}%	
%	\subcaption{Hit ratio of randomly selected warps over time.} 
%	\label{fig:warp-ratio-trend}
%        \end{subfigure}
%
%	\hspace{0.2in}
%
%        \begin{subfigure}[h]{3in}
%	\centering
%	\includegraphics[width=3in,angle=270]{results/queuing_lat.pdf}	
%        \subcaption{Distribution of per-request queuing latencies for L2 cache requests from BFS.}
%	\label{fig:l2-queue-latency}
%        \end{subfigure}
%\end{figure}
%
\subsubsection{Memory Divergence Correction (MeDiC)}

Based on these three observations and the key ideas of \titleShortMeDiC, there are
three major goals: (1)~convert mostly-hit warps into \emph{all-hit warps}
(warps where \emph{all} requests hit in the cache, as shown in
Figure~\ref{fig:mem-div}c), (2)~convert mostly-miss warps into \emph{all-miss
warps} (warps where \emph{none} of the requests hit in the cache, as shown in
Figure~\ref{fig:mem-div}d) and (3)~reduce L2 cache queuing delay for all warp
types. As we can see in Figure~\ref{fig:mem-div}a, the stall time due to memory
divergence for the mostly-hit warp can be eliminated by converting only the
single cache miss (Figure~\ref{fig:mem-div}a, \mycirc{2}) into a hit. Doing so
requires additional cache space. With the warp-type-aware cache bypassing and
warp-type-aware cache insertion policy of \titleShortMeDiC. We can convert the two
cache hits of the mostly-miss warp (Figure~\ref{fig:mem-div}b, \mycirc{4}) into
cache misses, we can cede the cache space previously used by these hits to the
mostly-hit warp, thus converting the mostly-hit warp into an all-hit warp.
Though the mostly-miss warp is now an all-miss warp
(Figure~\ref{fig:mem-div}d), it incurs no extra stall penalty, as the warp was
already waiting on the other six cache misses to complete. 

% Additionally, now
% that it is an all-miss warp, we predict that its future memory requests will
% also not be in the L2 cache, so we can simply have these requests \emph{bypass
% the cache}. In doing so, the requests from the all-miss warp can completely
% avoid unnecessary L2 access and queuing delays. This decreases the total number
% of requests going to the L2 cache, thus reducing the queuing latencies for
% requests from mostly-hit and all-hit warps, as there is less contention.

As depicted in Figure~\ref{fig:main-mechanism}, \titleShortMeDiC{} uses \mycirc{1}
warp type identification to drive three different components: \mycirc{2} a
\emph{warp-type-aware cache bypass mechanism}, which bypasses requests from
all-miss and mostly-miss warps to reduce the L2 queuing delay; \mycirc{3} a
\emph{warp-type-aware cache insertion policy}, which works to keep cache lines
from mostly-hit warps while demoting lines from mostly-miss warps; and
\mycirc{4} a \emph{warp-type-aware memory scheduler}, which prioritizes DRAM
requests from mostly-hit warps as they are highly latency sensitive.

\begin{figure}[h]
        \vspace{3pt}
	\centering
	\includegraphics[width=\textwidth]{fig/overall-design.pdf}	
	\vspace{-7pt}
	\caption{Overview of \titleShortMeDiC{}: \protect\mycirc{1} warp type identification logic, \protect\mycirc{2} warp-type-aware cache bypassing, \protect\mycirc{3} warp-type-aware cache insertion policy, \protect\mycirc{4} warp-type-aware memory scheduler.} 
	\label{fig:main-mechanism}
	\vspace{6pt}
\end{figure}


To evaluate the effectiveness of \titleShortMeDiC, we compare \titleShortMeDiC{} to four
GPU cache management mechanisms: the Evicted Address Filter insertion
policy~\cite{eaf-vivek}, PCAL bypassing policy~\cite{donglihpca15}, PC-based
cache bypassing policy and a random bypassing policy over 15 different GPGPU
applications from 4 benchmark suites. We find that \titleShortMeDiC delivers an
average speedup of 21.8\%, and 20.1\% higher energy efficiency, We conclude
that each component of \titleShortMeDiC{}, and the full \titleShortMeDiC{} framework, are
effective. Each component of \titleShortMeDiC{} addresses the same problem (i.e.,
memory divergence of threads within a warp) using different techniques on
different parts of the memory hierarchy. For the majority of workloads, one
optimization is enough.  However, we see that for certain high-intensity
workloads (BFS and SSSP), the congestion is so high that we need to attack
divergence on multiple fronts. Thus, \titleShortMeDiC{} provides better average
performance than all of its individual components, especially for such
memory-intensive workloads.

\subsubsection{Proposed Works on Warp-Aware Shared Cache/Memory Management}
\label{sec:medic-plus}

While \titleShortMeDiC provides a shared cache management scheme that can
provide better cache utilization to GPGPU applications, several questions still
remains to be answered. As the extension of this work, we plan to improve the
design of \titleShortMeDiC and answer the following questions:

\begin{enumerate}

\item Is the memory divergence heterogeneity trend the same for different input
sets for each workload? 

\item Is it possible to design a mechanism that provides load balancing between
different memory partitions to reduce cache contention and queuing delay further
while still maintain good locality?

\item What is the reason behind memory divergence heterogeneity? Our extension to
\titleShortMeDiC should provide further analysis on what the cause of
memory divergence heterogeneity is.

\item How to modify \titleShortMeDiC for multi-core and heterogeneous architecture?

\end{enumerate}




\subsection{Interference from GPU Application to CPUs in a CPU-GPU Heterogeneous Systems}
\label{prelim-sms}

In addition to interference between each warp in GPU, GPUs in a CPU-GPU
heterogeneous systems can also become a major source of interference. A typical
CPU application only has a relatively small number of outstanding memory
requests at any time. The size of a processor's instruction window bounds the
number of misses that can be simultaneously exposed to the memory system.
Branch prediction accuracy limits how large the instruction window can be
usefully increased. In contrast, GPU applications have very different access
characteristics, generating many more memory requests than CPU applications. A
GPU application can consist of many thousands of parallel threads, where memory
stalls on one group of threads can be hidden by switching execution to one of
the many other groups of threads.

Figure~\ref{fig:intensity} (a) shows the memory request rates for a
representative subset of our GPU applications and the most memory-intensive
SPEC2006 (CPU) applications, as measured by memory requests per thousand cycles
when each application runs alone on the system. The raw bandwidth demands of
the GPU applications are often multiple times higher than the SPEC benchmarks.
Figure~\ref{fig:intensity} (b) shows the row-buffer hit rates (also called
row-buffer locality or RBL). The GPU applications show consistently high levels
of RBL, whereas the SPEC benchmarks exhibit more variability. The GPU programs
have high levels of spatial locality, often due to access patterns related to
large sequential memory accesses (e.g., frame buffer updates).
Figure~\ref{fig:intensity}(c) shows the BLP for each application, with the GPU
programs consistently making use of far banks at the same time.

\begin{figure}[h]
\centering
\includegraphics[width=0.95\columnwidth]{./fig/intensity.pdf}
\caption{GPU memory characteristic. (a) Memory-intensity, measured by memory requests
per thousand cycles, (b) Row buffer locality, measured by the fraction
of accesses that hit in the row buffer, and (c) Bank-level parallelism.}
\label{fig:intensity}
\end{figure}



In addition to the high-intensity memory traffic of GPU applications, there are
other properties that distinguish GPU applications from CPU applications.  The
TCM~\cite{tcm} study observed that CPU applications with streaming access
patterns typically exhibit high RBL but low BLP, while applications with less
uniform access patterns typically have low RBL but high BLP.

In contrast, GPU applications have {\em both} high RBL and
high BLP. The combination of high memory intensity, high RBL and high BLP means
that the GPU will cause significant interference to other applications
across all banks, especially when using a memory scheduling algorithm
that preferentially favors requests that result in row-buffer hits.

The main memory system has become a critical shared resource in many modern
chip multiprocessor (CMP) systems. Memory requests from multiple cores
interfere with each other and degrade overall system performance. The memory
controller is designed to appropriately prioritize memory requests in order
to reduce interference and improve system performance. 

Recent systems present an additional challenge by introducing an integrated
Graphics Processing Unit (GPU) on the same die with the CPU cores. Due to the
GPU's ability to execute a large number of parallel threads, GPU applications
typically demand significantly more memory bandwidth than CPU applications.
Previous proposals on memory scheduling have either focused on memory
interference between applications in CPU-only scenarios~\cite{atlas,
tcm, fr-fcfs} or maximizing bandwidth in GPU-only
scenarios~\cite{fr-fcfs,complexity}. While application-aware memory
scheduling policies designed for CPU-only scenarios can be applied on a CPU-GPU
heterogeneous system, the GPU requests occupy a significant portion of request
buffer space and reduce the visibility of CPU cores' requests, lowering system
performance. Increasing the request buffer space requires complex logic to
analyze applications' characteristics, assign priorities for each memory
request and enforce these priorities when the GPU is present. As a result,
these past proposals \emph{perform poorly on a CPU-GPU heterogeneous system at low
complexity.}

\textbf{Our goal} in this preliminary work is to design a low-complexity memory
scheduler that provides high performance and fairness in a heterogeneous
CPU-GPU system. 

\subsubsection{The \titleLongSMS}
\label{sec:prelim-sms}

\noindent{\bf Overview:} Our proposed \titleLongSMS~\cite{sms} architecture
introduces a new memory controller (MC) design that provides 1) scalability and
simpler implementation by decoupling the primary functions of an
application-aware MC into a simpler multi-stage MC, and 2) performance and
fairness improvement by reducing the interference from bandwidth-intensive
applications. \titleShortSMS provides these benefits by introducing
a three-stage design. The first stage is the \emph{\batch formation} stage that
groups requests from the same application that access the same row to improve
\mbox{row-buffer} locality. The second stage is the \emph{\batch scheduler}
that schedules batches of requests across different applications. The last
stage is the \emph{DRAM command scheduler} that schedules requests while
satisfying all DRAM constraints.

The staged organization of \titleShortSMS lends directly to a \mbox{low-complexity}
hardware implementation. Figure~\ref{fig:overall} illustrates the overall
hardware organization of the \titleShortSMS.\\[-0.1in]

\begin{figure}[h]
\centering
\includegraphics[width=\columnwidth]{./fig/main_imporved.pdf}
\caption{Organization of the \titleShortSMS~\cite{sms}.}
\label{fig:overall}
\end{figure}

\subsubsection{The \titleShortSMS Algorithm}
\label{sec:algoSMS}
%\vspace{-0.1in}
\noindent {\bf Stage 1 - \Batch Formation.}
The goal of this stage is to combine individual memory requests from each source
into batches of row-buffer hitting requests.
It consists of several simple FIFO structures, one
per {\em source} (i.e., a CPU core or the GPU). Each request from a given
source is initially inserted into its respective FIFO upon arrival at the
MC. A {\em\batch} is simply one or more memory requests from
the same source that access the same DRAM row. That is, all requests within a
\batch, except perhaps for the first one, would be row-buffer hits if scheduled
consecutively. A \batch is deemed complete or {\em ready} when an incoming request
accesses a different row, when the oldest request in the \batch has exceeded a
threshold age, or when the FIFO is full. Only ready batches are considered
by the second stage of \titleShortSMS.

\ignore{
\begin{figure*}[ht]
\centering
\includegraphics[width=\columnwidth]{./fig/reqBatch.pdf}
\caption{A timeline showing how a batch of requests is formed for an application}
\label{fig:batcher}
\end{figure*}
}

\noindent{\bf Stage 2 - \Batch Scheduler.}
\ignore{
The \batch formation stage has combined individual memory requests into \batches of
row-buffer hitting requests.}
The \batch scheduler deals directly with \batches, and therefore need not worry
about scheduling to optimize for \mbox{row-buffer} locality. Instead, the
\batch scheduler focuses on higher-level policies regarding inter-application
interference and fairness. The goal of this stage is to prioritize \batches from applications
that are latency critical, while making sure that bandwidth-intensive
applications (e.g., the GPU) still make reasonable progress.

The \batch scheduler considers every source FIFO (from stage 1) that
contains a ready batch. It picks one ready batch based on either a shortest job
first (SJF) or a round-robin policy.  Using the SJF policy, the \batch
scheduler chooses the oldest ready batch from the source with the fewest total
in-flight memory requests across all three stages of the \titleShortSMS. 
SJF prioritization reduces average request service latency, and it tends to favor
latency-sensitive applications, which tend to have fewer total requests. 
Using the round-robin policy, the \batch scheduler simply picks the next ready batch
in a \mbox{round-robin} manner across the source FIFOs. This ensures that
memory-intensity applications receive adequate service. The \batch
scheduler uses the SJF policy with probability $p$ and the round-robin policy
with probability $1-p$. The value of $p$ determines whether the CPU or the GPU
receives higher priority. When $p$ is high, the SJF policy is applied more
often and applications with fewer outstanding requests are prioritized. Hence,
the batches of the likely less memory-intensive CPU applications are
prioritized over the batches of the GPU application. On the other hand, when
$p$ is low, request batches are scheduled in a round-robin fashion more often.
Hence, the memory-intensive GPU application's request batches are likely
scheduled more frequently, and the GPU is prioritized over the CPU.

% Overall, the batch
%scheduler uses the SJF policy with a probability $p$ and the round-robin policy
%otherwise. $p$ is a configurable parameter.
%
After picking a \batch, the \batch scheduler enters a drain state where it
forwards the requests from the selected \batch to the final stage of the
\titleShortSMS. The \batch scheduler dequeues one request per cycle until
all requests from the \batch have been removed from the selected FIFO. 

\noindent{\bf Stage 3 - DRAM Command Scheduler (DCS).} The DCS consists of one
FIFO queue per DRAM bank. The drain state of the \batch scheduler places the
memory requests directly into these FIFOs. Note that because \batches are moved
into the DCS FIFOs one \batch at a time, \mbox{row-buffer} locality within a
\batch is preserved within a DCS FIFO. At this point, higher-level policy
decisions have already been made by the \batch scheduler. Therefore, the DCS
simply issues low-level DRAM commands, ensuring DRAM protocol compliance.

In any given cycle, the DCS considers only the requests at the {\em head} of
each of the per-bank FIFOs. For each request, the DCS determines whether that
request can issue a command based on the request's current row-buffer state
(e.g., is the row-buffer already open with the requested row?) and the current
DRAM state (e.g., time elapsed since a row was opened in a bank, and data bus
availability). If more than one request is eligible to issue a command in any
given cycle, the DCS arbitrates between DRAM banks in a round-robin fashion.

We evaluated the design trade-offs involved in our \titleLongSMS
(\titleShortSMS) and compared it against four state-of-the-art memory
controller designs. Our evaluation shows that \titleShortSMS gains 41.2\%
performance improvement and 4.8$\times$ improvement in fairness compared to the
best previous state-of-the-art techniques, while providing a design that is
significantly less complex to implement. 


\subsubsection{Proposed works on CPU-GPU Memory Scheduling}
\label{sec:sms-plusplus}

In addition to the throttling mechanism we propose (See
Section~\ref{sec:sms-plus} to reduce the interference of GPU in heterogeneous
systems, we propose to continue investigating 


\begin{enumerate}

\item What is the performance affect of writes? Would it be possible to mitigate GPU interference
even further by isolating read from write requests?

\item Can we take advantage of the sub-array level parallelism~\cite{salp,dsarp} to further improve the performance
and QoS of heterogeneous CPU-GPU systems? 

\item How would SMS performs against recent memory scheduling mechanisms~\cite{bliss}.

\end{enumerate}





==> secs/sms/secs/0_abstract.tex <==
\begin{abstract}
When multiple processor cores (CPUs) and a GPU integrated together on the same
chip share the off-chip DRAM, requests from the GPU can heavily interfere with
requests from the CPUs, leading to low system performance and starvation of
cores. Unfortunately, state-of-the-art memory scheduling algorithms are
ineffective at solving this problem due to the very large amount of GPU traffic,
unless a very large and costly request buffer is employed to provide these
algorithms with enough visibility across the global request stream.

Previously proposed memory controller (MC) designs use a single monolithic
structure to perform three main tasks. First, the MC attempts to schedule
together requests to the same DRAM row to increase row-buffer hit rates.
Second, the MC arbitrates among the requesters (CPUs and GPU) to optimize for
overall system throughput, average response time, fairness and quality of
service. Last, the MC manages the low-level DRAM command sequencing to ensure
compliance with all DRAM timing and power constraints.

%%% ONUR-11-19: The first sentence below needs work... It was broken before.
This paper proposes a fundamentally new approach that decouples the three
primary MC tasks into three significantly simpler structures that together
improve system performance and fairness. Our three-stage MC first groups
requests based on row-buffer locality. This grouping allows the second stage to
focus only on inter-application scheduling decisions. These two stages enforce
high-level policies regarding performance and fairness, and therefore the last
stage can get away with using simple per-bank FIFO queues (no further command
reordering within each bank) and straight-forward logic that only deals with
the low-level DRAM commands and timing.

%%% ONUR-11-19: Is the last stage dealing only with correctness and
%%% power issues? If so, let's say it. I assume it is doing command
%%% reordering, too, so saying this may not be correct. But, please
%%% let me know.
We evaluated the design trade-offs involved in our \titleLongSMS (\titleShortSMS) and
compared it against four state-of-the-art MC designs. Our evaluation shows that
\titleShortSMS gains 41.2\% performance improvement and 4.8$\times$ improvement in
fairness compared to the best previous state-of-the-art techniques, while
providing a design that is significantly less complex to implement. 

\ignore{
In addition, only
the last stage of \titleShortSMS needs to deal with correctness and power issues,
the design of \titleShortSMS is significantly less complex to implement.
}
\end{abstract}


==> secs/sms/secs/7_related.tex <==
\subsection{Related Work}
\label{sec:related}

%%GL: we need to be careful about this claim.  Some of the GPU schedulers
%%GL: (for example the Nvidia patent in the citations) are arguably scalable
%%GL: (while they have significant area and power cost, they still decided
%%GL: that it was acceptable to implement).
%\noindent To our knowledge, we are the first to propose a multi-staged memory
%scheduler to address the scalability problem of conventional schedulers that
%are limited to a monolithic memory request buffer, in a system with high
%inter-application interference.

\noindent\textbf{Memory Schedulers:}
We have compared \titleShortSMS to recent state-of-the-art memory schedulers
(FR-FCFS~\cite{fr-fcfs}, ATLAS~\cite{atlas}, PAR-BS~\cite{parbs},
and TCM~\cite{tcm}) both quantitatively and qualitatively in previous sections.
\titleShortSMS outperforms these schedulers in terms of both system performance and
fairness. Other memory schedulers
~\cite{stfm,memattack,csfq,dram_man,dram_smt,mem_study,complexityeffscheduling}
that are either aware or unaware of applications have been proposed.
However, none of these works have been shown to provide better performance/fairness than TCM, which
\titleShortSMS outperforms across a wide range of workloads.
In particular, Yuan et al.~\cite{complexityeffscheduling} propose a mechanism to
preserve row-buffer locality with modifications to the interconnection
network, while keeping the memory scheduler simple and in-order. Our \titleShortSMS
proposal, on the other hand, not only preserves row-buffer locality by using a
simple distributed FIFO design, but also provides application-awareness
with simple \batch scheduling logic. Furthermore, our results show that
\titleShortSMS provides 2$\times$ better system performance and 9$\times$ better
fairness as compared to an application-unaware FR-FCFS scheduler.

\ignore{
Although the goals on
preserving the row-buffer locality and keeping the simplicity of request
buffer are the same, they do not address the problem of inter-application
interference that can significantly destroy row-buffer localities of all the
applications. 
}

\ignore{In addition, they all use a
single memory request buffer to observe memory traffic characteristics from
different applications.}

\noindent\textbf{Memory Channel Partitioning:}
Instead of mitigating the interference problem between applications by
scheduling requests at the memory controller, Muralidhara et al.~\cite{mcp}
propose memory channel partitioning (MCP) to map applications
to different memory channels based on their memory-intensities and row-buffer
locality to reduce inter-application interference. Our \titleShortSMS approach is
complementary to MCP. Furthermore, as shown in~\cite{mcp}, MCP can be integrated
with different memory schedulers to further improve system throughput and
fairness. 

\ignore{
Although MCP has the same
goal as our work, our approach is to design a new memory request scheduler,
which is complementary to MCP. As shown in~\cite{mcp}, MCP can be integrated
with different memory schedulers to further improve the system throughput and
fairness.
}

\noindent\textbf{Source Throttling:}
Ebrahimi et al.~\cite{fst} propose fairness via source throttling (FST) to
mitigate inter-application interference in a shared-memory system by throttling
the request injection rate of interfering applications
at the source. However, this approach is orthogonal to \titleShortSMS which
reduces inter-application interference via memory scheduling. Therefore,
\titleShortSMS and FST can be applied synergistically to achieve better
inter-application interference reduction and further improvements in fairness and
system performance.

\ignore{
\noindent\textbf{Application-Aware Memory Scheduling:} We briefly describe
recently proposed application-aware memory schedulers~\cite{atlas,parbs,tcm}
that attempt to reduce inter-application interference at the memory system. 
In section X, we will compare \titleShortSMS quantitatively with these three
state-of-the-art memory schedulers.

Kim et al. propose ATLAS~\cite{atlas} with the goal of maximizing system
throughput. It achieves improved system throughput by prioritizing
applications with least attained memory service because low memory intensity
applications experience more slowdown than high memory intensity applications
from request stalling. However, ATLAS has the disadvantage of not preserving
fairness.  Simply prioritizing low memory intensity applications lead to high
slowdown of memory-intensive applications.

Mutlu et al. propose parallelism-aware batch scheduling (PAR-BS)~\cite{parbs}
to achieve fairness and high system throughput. In order to
prevent unfairness, it forms batches of outstanding memory requests and
prioritizes the oldest batch, so that it avoids starvation of any request. To
improve system throughput, it ranks applications based on their number of
outstanding memory requests to any bank and prioritizes applications with the
shortest job first principle. Hence, applications with low memory intensity
or high bank-level parallelism are prioritized over others to reduce average
stall time to achieve a high system throughput.

Thread cluster memory scheduling (TCM)~\cite{tcm} is the best state-of-the-art
memory scheduler in providing both fairness and system throughput. It groups
applications based on their memory intensity into either latency- or
bandwidth-sensitive clusters. In order to achieve high system throughput and
low unfairness, TCM employs different prioritization policy for each cluster. To
improve system throughput, a fraction of total memory bandwidth is dedicated
to latency-sensitive cluster and applications within the cluster are then
ranked based on memory intensity with least memory-intensive application
receiving the highest priority. On the other hand, TCM minimizes unfairness by
periodically shuffling applications within a bandwidth-sensitive cluster to
prevent starvation of any application.

These and other additional~\cite{stfm,memattack,csfq,dram_man}
application-aware memory schedulers observe the characteristics of different
applications from a single memory request buffer to make ranking decisions to
mitigate inter-application interference. However, simply using a single memory
request buffer becomes problematic in a CPU-GPU system that generates
extremely large amount of memory requests from the GPU. In order to make a
good decision on which requests to prioritize requires a significantly
large memory request buffer to observe memory traffic characteristics of the GPU
and CPUs. This buffer scalability issue will only exacerbate as the number of
cores continues to grow in the future. In contrast to these schedulers with a
centralized memory request buffer and scheduling algorithm, we propose a new
approach that performs two levels of scheduling with decoupled memory request
buffers to improve system performance at a lower cost.

\noindent\textbf{Application-Unaware Memory Scheduling:}
Prior work~\cite{fr-fcfs,dram_smt,mem_study} have proposed memory
schedulers that are oblivious to different applications' memory access
behaviors. The most widely adapted FR-FCFS memory scheduler~\cite{frfcfs}
prioritizes row-buffer hit over row-buffer miss requests and then schedules
the rest based on a first-come, first-served policy. Since these memory
schedulers aim to maximize DRAM throughput, they have been shown to have low
system performance and high unfairness in previous
work~\cite{atlas,parbs,tcm,stfm,memattack}.
}

\ignore{
\noindent\textbf{Source Throttling:}
}



==> secs/sms/secs/my_eval.tex <==
\section{Experimental Evaluation}
\label{sec:eval}

\subsection{Main Results}



We first present the performance of \titleShort in comparison with four
previously proposed scheduling policies (FR-FCFS, PAR-BS, ATLAS, TCM) each with
a 300-entry request buffer and TCM with a 2048-entry request buffer, on a
baseline with 16 CPU cores, 1 GPU core and 4 memory controllers (as described in
Sec~\ref{sec:meth}).


Figure~\ref{fig:mainres} shows CPU system performance, fairness and GPU memory
throughput provided by previously proposed algorithms and \titleShort, averaged
across 15 workloads of 7 categories (105 workloads in all). Four major
conclusions are in order. First, TCM (TCM 300) provides higher CPU system
performance and lower unfairness, while degrading the GPU memory throughput by
less than 10\% as compared to previously proposed scheduling policies with the
same number (300) of request buffer entries. Second, TCM with 2048 request
buffer entries (TCM 2048) provides significantly better performance and fairness
than TCM with 300 request buffer entries (TCM 300), due to improved visibility
from increasing the number of entries in the request buffer. However, this
incurs the storage cost of 6x extra request buffer entries and the complexity of
associative logic for looking into a large request buffer. Third, our proposed
\titleShort approach provides 2x better CPU system performance, 5x lower
unfairness while degrading the GPU memory throughput by only 30\% as compared to
TCM 300 - a TCM design with the same number (300) of request buffers. Finally,
an \titleShort design provides 4\% better CPU system performance, on par
fairness and GPU memory throughput as a TCM design with 6x the number of request
buffer entries (TCM 2048). We conclude that \titleShort provides better
performance and fairness than all previously proposed scheduling policies while
incurring much lower hardware cost and complexity.


\begin{figure}
\centering
\includegraphics[width=6.5in,height=2.5in]{./fig/main_results2.pdf}
\vspace{-0.1in}
\caption{\titleShort vs other algorithms on a 16 CPU/1 GPU system with 4 memory
controllers (averaged across 105 workloads - 15 workloads in each category)}
\vspace{-0.2in}
\label{fig:mainres}
\end{figure}

\subsection{Effect of Workload Memory Intensity}

Figure~\ref{fig:mainres} shows CPU system performance, fairness and GPU memory
throughput for workloads composed of applications with different memory
intensities. L, M and H stand for low, high and medium memory-intensity (as
described in Sec~\ref{sec:meth} and indicate the composition of workloads in
a category. Three major conclusions can be made from the results. First,
\titleShort provides consistently better CPU/GPU performance and fairness than
TCM 300, across all workload categories. Second, TCM 2048, provides on par system
performance as \titleShort in most workload categories. However, when all
applications in a workload have high memory-intensity (the H category), TCM 2048
provides better system performance at the cost of severe degradation in
fairness. We observe that that when TCM attempts to rank between and cluster all
applications of high memory-intensity, some applications get mis-classified into
the low memory-intensity cluster starving requests of other applications that
were classified into the high memory-intensity cluster. \titleShort on the
other hand employs a probabilistic round-robin mechanism that ensures that each
application's requests will eventually get served, reducing unfairness
significantly.

\subsection{Scalability with Cores and Memory Controllers}

Figure~\ref{fig:coreSweep} compares the performance and unfairness of
\titleShort against TCM with the same number (300) of request buffers. As the
number of cores and memory controllers is varied, we make several major
conclusions. First, \titleShort consistently provides better system performance
and fairness than TCM. Second, the system performance (from 30\% to 115\%) and
fairness gains (194\% to 379\%) increase as the number of cores is increased.
This performance gain widens because \titleShort is capable of throttling GPU
requests while allowing latency sensitive applications to progress faster.  As
a result, there is a cost of minor GPU bandwidth reduction (from 14.7\% to
39.5\%)

\begin{figure}
\centering
\begin{minipage}{3.25in}
\includegraphics[scale=0.75]{./fig/coreSweep.pdf}
\caption{\titleShort vs TCM on a 16 CPU/1 GPU, 4 memory controller system with varying the number of cores}
\label{fig:coreSweep}
\end{minipage}
\begin{minipage}{3.25in}
\includegraphics[scale=0.75]{./fig/batchTize.pdf}
\caption{\titleShort sensitivity to \batch-age threshold}
\label{fig:batch-age}
\end{minipage}
\end{figure}

\begin{figure}
\centering
\end{figure}

\subsection{Sensitivity to \titleShort Design Parameters}

We present sensitivity of \titleShort to its different design parameters. These
results are averaged across 75 of our workloads.

\textbf{\Batch-age Threshold:}
Figure~\ref{fig:batch-age} shows the sensitivity of \titleShort to the
\batch-age threshold (across three different categories of applications), which
determines how long \titleShort batches requests. This result shows how
sensitive each type of applications is to \batch-age threshold. For both low
and medium intensity applications, the performance degrades as the \batch-age
threshold increases. However, for the high intensity applications, they do not
lose performance when the \batch-age is less than 200 cycles.

\textbf{\Batch Size:} 
Figure~\ref{fig:batchsize} shows the sensitivity of \titleShort to \batch size.
\titleShort provides good performance and fairness except with very small \batch
sizes. This is because when the \batch size is zero or very small, both CPU and
GPU intra-application row-buffer locality is not preserved and requests of
multiple CPU applications and the GPU application interfere with each other in
the row-buffer. With reasonably large \batch sizes (starting from 10
onwards), row-buffer locality is well-preserved enough to provide good
performance and fairness. 

\begin{figure}
\centering
\begin{minipage}{3.25in}
\includegraphics[scale=0.75]{./fig/batchSize.pdf}
\caption{\titleShort sensitivity to \batch Size}
\label{fig:batchsize}
\end{minipage}
\begin{minipage}{3.25in}
\includegraphics[scale=0.75]{./fig/FIFOSize.pdf}
\caption{\titleShort sensitivity to DCS FIFO Size}
\label{fig:fifosize}
\end{minipage}
\end{figure}

\textbf{DCS FIFO Size:}
Figure~\ref{fig:fifosize} shows the sensitivity of \titleShort to the size of
per-bank FIFOs in the DRAM Command Scheduler (DCS). We make the following
observation: As the size of the per-bank FIFOs increases, the \batch scheduler
tends to move more batches from the \Batch formation stage to the FIFOs. Once
\batches are moved to the FIFOs, they cannot be reordered anymore. Therefore,
employing larger per-bank FIFOs in the DCS stage can prevent the \batch
scheduler from seeing more \batches and making better \batch scheduling
decisions.

%% BELOW EXPLANATION NEEDS A LOT OF WORK.
\textbf{\Batch Formation FIFO Size}
We observe that our current design of 10-entry FIFOs for each CPU core
and a 20-entry FIFO for the GPU provides good performance and fairness.
Because \batch formation only allows each individual request to progress
downstream in-order. Increasing the \batch Formation FIFO size has no effect
on the order of which each request within an application will be serviced.
As a result, the size of \batch formation FIFO only need to be large enough
to contain a few \batches.
 

\subsection{Case Studies}

In this section, we present a sensitivity analysis against other interesting
workload setups, and also the sensitivity to other design and system
parameters. Due to simulation bandwidth, we reduce the simulation time of all
sensitivity analysis study to 200M cycles.

\ignore{
\subsubsection{Case study 1: Random and stream applications}

In this section, we evaluate the performance of \titleShort and other previously proposed
mechanisms on a synthetically generated stream and random applications. Table [cite]
shows the characteristic of each application. We generated 2 sets of workload categories.
The first category consists of several streaming applications along with randomly selected 
SPEC2006 applications from L/M/H group, and a GPU. The second category consists of a synthetic
application with random memory access pattern along with randomly selected SPEC2006
applications from L/M/H group, and a GPU. Figure~\ref{fig:stream} shows the performance of
SMS on these two workloads categories.

[TODO: fix the WS number after all corrected alone results are out]
\begin{figure}
\centering
\includegraphics[width=6.5in,height=2.5in]{./fig/stream.pdf}
\vspace{-0.1in}
\caption{Performance on a streaming and random applications}
\vspace{-0.2in}
\label{fig:stream}
\end{figure}

}

\subsubsection{Case study 1: CPU only results}

We evaluate the performance of \titleShort on a CPU-only workloads. We use the
four categories of workloads discussed in ~\ref{sec:meth} that contains high
intensity applications; however, we take out the GPU applications and measure
the performance of FRFCFS, TCM and \titleShort. Figure ~\ref{fig:cpu} shows how
\titleShort performs on a CPU-only workloads. In this experiment, the
parameters for both TCM and \titleShort are not fine tuned to acheive the
maximum performance. In this case study, TCM performs 4\% better than
\titleShort while \titleShort gain 25.7\% improvement in fairness. The
majority of the performance difference come from the all-high workload
category. As discessed in ~\ref{sec:qualComp}, TCM will cluster a few
lowest intensity applications among the high intensity workload, and
prioritize those applications over the other. This will cause those
few lucky applications progress faster at a cost of higher unfairness.
In \titleShort, we mitigate this problem by probabilistically performing 
a round-robin prioritization in order to ensure forward progress to
all applicaitons.

\begin{figure}
\centering
\includegraphics[scale = 1.5]{./fig/cpuOnly.pdf}
\vspace{-0.1in}
\caption{Performance on a 16 cores CPU-only workloads}
\vspace{-0.2in}
\label{fig:cpu}
\end{figure}


\subsubsection{Case study 2: do not coalesce GPU requests}

In the final result, we coalesce GPU request as discussed in Section
~\ref{sec:meth}.  This coalescing unit require some amount of buffering as well
as additional logic. In this section, we perform a study of what is the
performance impact if we do not coalesce GPU requests. Figure ~\ref{fig:gmc}
shows the performance difference between coalescing and not coalescing GPU
requests, which shows that coalescing can provide significant performance and
fairness improvements. In addition, Figure~\ref{fig:gmc} also shows that
\titleShort performs better than TCM on both with and without GPU request
coalescing. In order to further minimize the design cost of \titleShort over
other scheduling mechanisms, one possible improvement we can perform on
\titleShort is to performs request coalescing at the \batcher formation FIFO.
However, due to space limitation we will leave this to future work.


\begin{figure}
\centering
\includegraphics[scale =1.5]{./fig/gmc.pdf}
\vspace{-0.1in}
\caption{Result with and without GPU requests coalescing}
\vspace{-0.2in}
\label{fig:gmc}
\end{figure}

\ignore{
\subsection{Main Results}

We first analyze the result on a 17 cores CPU-GPU system discussed on Seciton
~\ref{sec:meth}.  Figure ~\ref{fig:mainres} shows the weighted speedup,
GPU memory throughput, unfairness and average latency per memory instruction
for CPUs and a GPU application across 7 categories of workloads. We compare the
results against five different previously proposed mechanism.

\begin{figure}
\centering
\includegraphics[width=6.5in,height=2.5in]{./fig/main_results.pdf}
\vspace{-0.1in}
\caption{Final Results}
\vspace{-0.2in}
\label{fig:mainres}
\end{figure}

\squishlist
\item\textbf{FRFCFS:} The commonly-used FRFCFS scheduling policy is both performs
poorly and very unfair toward GPU application. Given that GPU applications has
high row buffer locality, most of the time FRFCFS will give priority to GPU applications,
while CPU applications will starve. This results in unfairness, and also worse
system throughput.

\item \textbf{PAR-BS:} Even though batching in PAR-BS helps prevent starvation.
The mechanism itself is not designed to handle an extreme case of the GPU. In
this case, GPU has issue too many requests per cycles. Batching allows older
GPU requests to have more priority than other latency sensitive CPU
applications. This will result in significant slowdown across all CPU
application including high intensity CPU applications, leading to severe
unfairness and low system throughput.

\item \textbf{ATLAS:} In the case of ATLAS, we observed that there are two
affects in the mechanisms that reduce the system throughput. In ATLAS, there is
a timeout threshold for each requests.  Once a request waits in the request
buffer for too long, it will be marked. All marked requests will be prioritized
over unmarked requests. Once a GPU application issue lots of memory requests,
the system will be heavily congested. This will result in most requests, CPU
and GPU, become marked. As a result, most GPU request eventually will be
masked. When a new CPU requests arrive, it will need to wait either all marked
GPU requests are serviced, or wait until it is marked. We have observed that
CPU generally need to waited until they are marked, leading to starvation of
latency sensitive CPU applications.  One possible way to fix this is to
increase the timeout threshold. However, we observe that increase the timeout
will starve the GPU application.

\item \textbf{TCM:} We have observed that when facing limited number of request
buffers, TCM more high intensity applications in the low intensity cluster.
This has two effects to the system performance.  Because TCM will prioritize
applications in the low intensity clusters over applications in the high
intensity cluster. TCM ends up strictly prioritizing a lucky high intensity
applications in the low intensity cluster over other unlucky high intensity
applications in the high intensity cluster, leading to more interference among
high intensity applications. In addition, when there are fewer applications in
the high intensity cluster for shuffling, a GPU application has more chance to
be prioritized. As a result, high intensity applications that are grouped in
the high intensity cluster experience severe slowdown, which can be seen by the
unfairness result. Still, TCM still performs better than other previously
proposed scheduling mechanisms.
 
\item \textbf{\titleShort:} As the main goal for \titleShort
is similar to that of TCM, which is prioritizing low intensity application over
high intensity application, but preserve the row buffer locality with the
batcher.  We are able to achieve much better performance compared to 300-entry
TCM. In fact, we are able to perform almost as good as 2048-entry TCM. By
decoupling the functionality of the memory controller, batcher is able to
preserve the row buffer locality of intensive applications while the batch
scheduler allow low intensity applications, which is latency sensitive, to
progress. This prevent starvation as can be seen by the unfairness plot. We are
able to achieve xx\% increase in weighted speedup compared to 300-entry TCM,
which is the best previously proposed mechanism, while able to be yy\% fairer.
Figure~\ref{fig:mainres} also shows the improvement in term of average memory latency of
CPU applications while trading off with higher GPU memory latency. However,
this trade-off is not costly as GPU applications have an extremely high MLP,
and is able to hide the memory latency much better than CPU applications.

\item \textbf{Effects on each workload group:} In Figure~\ref{mainres}, \titleShort typically
provide better performance if the workload is heterogeneous. However, when each
CPU application in the workload has the similar intensity. TCM have better
weighted speed, with a cost of severe fairness issue. We observed that TCM
cluster a few lowest intensity applications into the low intensity cluster,
starving other applications in the high intensity clusters. In \titleShort,
probabilistic round-robin will make sure that every application will eventually
get serviced, reducing unfairness significantly at the cost of weighted
speedup.

\squishend

\subsection{Sensitivity Analysis}

In this section, we present a sensitivity analysis against other interesting
workload setups, and also the sensitivity to other design and system
parameters. Due to simulation bandwidth, we reduce the simulation time of all
sensitivity analysis study to 200M cycles.

\subsubsection{Case study 1: Random and stream applications}

In this section, we evaluate the performance of \titleShort and other previously proposed
mechanisms on a synthetically generated stream and random applications. Table [cite]
shows the characteristic of each application. We generated 2 sets of workload categories.
The first category consists of several streaming applications along with randomly selected 
SPEC2006 applications from L/M/H group, and a GPU. The second category consists of a synthetic
application with random memory access pattern along with randomly selected SPEC2006
applications from L/M/H group, and a GPU. Figure~\ref{fig:stream} shows the performance of
SMS on these two workloads categories.

[TODO: fix the WS number after all corrected alone results are out]
\begin{figure}
\centering
\includegraphics[width=6.5in,height=2.5in]{./fig/stream.pdf}
\vspace{-0.1in}
\caption{Performance on a streaming and random applications}
\vspace{-0.2in}
\label{fig:stream}
\end{figure}


\subsubsection{Case study 2: CPU only results}

We evaluate the performance of \titleShort on a CPU-only workloads. We use the same set
of workloads discussed in ~\ref{sec:meth}; however, we take out the GPU
applications and measure the performance of \titleShort. Figure [cite] shows how \titleShort
performs on a CPU-only workloads.

\subsubsection{Case study 3: do not coalesce GPU requests}

In the final result, we coalesce GPU request as discussed in Section ~\ref{sec:meth}.
This coalescing unit require some amount of buffering as well as additional
logic. In this section, we perform a study of what is the performance impact
if we do not coalesce GPU requests. Figure ~\ref{fig:gmc} shows the performance impact
when we do not coalesce GPU requests.

\begin{figure}
\centering
\includegraphics[width=6.5in,height=2.5in]{./fig/gmc.pdf}
\vspace{-0.1in}
\caption{Result with and without GPU requests coalescing}
\vspace{-0.2in}
\label{fig:gmc}
\end{figure}

\subsubsection{Sensitivity to design and system parameters}

Several design and system parameters can affect the performance of the system.
Figure [cite] shows the effect of different number of memory channels in the
system. 

How long we batch and the maximum batch size can also generate some side
effects to \titleShort. Figure [cite] shows the sensitivity analysis of how long we
batch each requests across different types of workloads.  The result shows that
the time spend batching should be inversely proportional to the intensity of an
application, as we have discussed in Section ~\ref{sec:mechanism}. 

Figure~\ref{fig:batchsize} shows the sensitivity analysis of \titleShort to the
size of the batch across 4 different workloads categories that contain memory
intensive CPU applications.  This shows that breaking the row buffer hitting
stream of requests does not hurt the performance as long as they are reasonably
sized. However, when requests are never batched, the performance drops
significantly because 1) a CPU request can interfere anywhere in the GPU
request stream, decreasing the row buffer locality of GPU request and 2) it
allow each individual GPU requests to be service separately, leading to more
interference to CPU application.

\begin{figure}
\centering
\begin{minipage}{3.25in}
\includegraphics[width=3.25in,height=1.3in]{./fig/batchSize.pdf}
\caption{Performance at different batch size limit}
\label{fig:batchsize}
\end{minipage}
\begin{minipage}{3.25in}
\includegraphics[width=3.25in,height=1.3in]{./fig/FIFOSize.pdf}
\caption{Performance at different size of FIFO}
\label{fig:fifosize}
\end{minipage}
\end{figure}


\subsubsection{Scalability}

Figure ~\ref{fig:fifosize} shows the performance of \titleShort scale with
different size of FIFO request queue. We observed that smaller FIFO request
queue can gain more performance. This happens because once a batch is
scheduled, it will be serviced in order. When the size of FIFO is large, more
requests will wait in the FIFO request scheduler, where no further scheduling
decision can be mode. When the FIFO request queue is small, most requests are
in the batcher. Leaving most of memory requests in the batcher allows the batch
scheduler to observe the state of each application more accurately.

\begin{figure}
\centering
\includegraphics[width=6.5in,height=2.5in]{./fig/coreSweep.pdf}
\vspace{-0.1in}
\caption{Result with and without GPU requests coalescing}
\vspace{-0.2in}
\label{fig:coreSweep}
\end{figure}

Figure~\ref{fig:coreSweep} shows the performance of FRFCFS, TCM and \titleShort on different number
of CPU cores.


}

